Towards Urban General Intelligence: A Review and Outlook of Urban Foundation Models

The integration of machine learning techniques has become a cornerstone in the development of intelligent urban services, significantly contributing to the enhancement of urban efficiency, sustainability, and overall livability. Recent advancements in foundational models, such as ChatGPT, have introduced a paradigm shift within the fields of machine learning and artificial intelligence. These models, with their exceptional capacity for contextual comprehension, problem-solving, and task adaptability, present a transformative opportunity to reshape the future of smart cities and drive progress toward Urban General Intelligence (UGI). Despite increasing attention to Urban Foundation Models (UFMs), this rapidly evolving field faces critical challenges, including the lack of clear definitions, systematic reviews, and universalizable solutions. To address these issues, this paper first introduces the definition and concept of UFMs and highlights the distinctive challenges involved in their development. Furthermore, we present a data-centric taxonomy that classifies existing research on UFMs according to the various urban data modalities and types. In addition, we propose a prospective framework designed to facilitate the realization of versatile UFMs, aimed at overcoming the identified challenges and driving further progress in this field. Finally, this paper systematically summarizes and discusses existing benchmarks and datasets related to UFMs, and explores the wide-ranging applications of UFMs within urban contexts, illustrating their potential to significantly impact and transform urban systems. A comprehensive collection of relevant research papers and open-source resources have been collated and are continuously updated at: https://github.com/usail-hkust/Awesome-Urban-Foundation-Models.

==> sections/basics.tex <==
\section{Basics of Urban Foundation Models} \label{basic}

% \begin{figure*}[tb]
% \centering
% \includegraphics[width=1.95\columnwidth]{figs/basic1.pdf}
% \caption{Urban Foundation Models (UFMs) are pre-trained on multi-source, multimodal urban data and can be adapted for a variety of downstream applications.}
% \label{fig:basic}
% \end{figure*}

\begin{figure*}[tb]
\centering
\includegraphics[width=1.95\columnwidth]{figs/basic2.pdf}
\caption{Urban Foundation Models (UFMs) are pre-trained on multi-source, multimodal urban data and can be adapted for a variety of downstream applications.}
\label{fig:basic}
\end{figure*}

\subsection{Concepts of Urban Foundation Models}

\begin{defi}[\textbf{Urban Foundation Models}]
Urban Foundation Models (UFMs) are large-scale models pre-trained on massive multi-source and multimodal urban datasets. It benefits significantly from its pre-training phase, exhibiting emergent capabilities and remarkable adaptability to a broader range of multiple downstream tasks in urban contexts. 
\end{defi}

UFMs, similar to foundation models in other fields, rely primarily on two key techniques: pre-training and adaptation.


\subsubsection{Pre-training}
UFMs typically undergo pre-training on extensive, varied datasets comprising geo-text data, social media content, street view images, trajectories, spatiotemporal time series data, point of interests, \etc The primary goal of pre-training is to enable these models to obtain as much general knowledge and patterns as possible, thereby capturing the overarching characteristics and structures inherent in the data. Pre-training methods for UFMs are principally divided into four categories: supervised pre-training, generative pre-training, and contrastive pre-training \cite{sslsurvey2021}:

\subsec{Supervised pre-training.} This method involves training models on datasets with a substantial volume of labeled data, pairing an input with its corresponding output. This approach allows models to learn the relationship between inputs and outputs in a supervised manner.

\subsec{Generative pre-training.} This approach trains models to generate or reconstruct input data in the absence of labeled data. It necessitates the model's ability to autonomously discern patterns and regularities, thereby producing outputs that closely mimic real data.

\subsec{Contrastive pre-training.} This method trains models to distinguish between data instances and learn robust data representations by evaluating similarities and differences among data samples, all without needing externally provided labels.

\subsec{Hybrid pre-training.} This approach is a versatile approach that integrates multiple pre-training methods, including supervised, generative, and contrastive techniques. This strategy aims to tailor the training process to specific problem demands, leveraging the strengths of each method. 

Since obtaining a large amount of high-quality human-labeled data can be expensive or impractical in many domains, generative and contrastive pre-training are frequently employed to fully leverage various dataset types. These methods optimize the model's performance and adaptability. Supervised pre-training may be used in specific application scenarios, particularly with abundant high-quality labeled data.

\subsubsection{Adaptation}
After pre-training, models can be tailored to specific tasks or domains through several methods like fine-tuning. During this phase, the model is trained on smaller, task-specific datasets to adjust and optimize its parameters, enhancing its performance for the particular task. Below are several prevalent adaptation methods.

\subsec{Vanilla fine-tuning.} This approach entails additional training of the pre-trained model using a task-specific dataset. It typically involves adjusting most or all of the model's parameters. Although direct and effective for task-specific adaptation, this method may demand significant amounts of training data and computational resources.

\subsec{Parameter-efficient Fine-tuning.} This technique minimizes the number of parameters that require adjustment during adaptation. It involves training only a subset of the model, thereby reducing training costs. This method maintains a balance between model adaptation performance and resource consumption~\cite{hu2021lora}

\subsec{Prompt-tuning.} In contrast to the conventional ``pre-train, fine-tune'' approach, prompt-tuning employs lightweight prompt tokens containing relevant information about the target task. This method has proven effective in leveraging the inherent knowledge embedded in the pre-trained backbone. This ``Pre-train, Prompt and Predict'' paradigm \cite{promptsurvey2023} is more efficient, as it necessitates training only a minimal set of prompt parameters, thereby avoiding the need for extensive alterations to the model's existing parameters.

These adaptation methods enhance the flexibility and power of UFMs across diverse application contexts. Selecting suitable adaptation strategies is crucial for maximizing the performance of pre-trained models on specific tasks and datasets while reducing resource costs.

\subsection{Difference to Existing Foundation Model}
\subsubsection{Difference to Existing Foundation Model}
While existing foundation models, such as LLMs and VFMs, demonstrate consistent versatility across various fields, UFMs exhibit distinct characteristics in several crucial aspects.

\subsec{Multi-source multimodal urban data integration.}
UFMs integrate diverse urban data from multiple sources, such as geo-text data, social media contents, street view images, trajectories, spatiotemporal time series data, point of interests. This integration contrasts with other foundation models, which often concentrate on a single data type, such as text or images.

\subsec{Multi-granularity.}
UFMs possess the ability to process and analyze data at varying levels of granularity. They can manage both macro-level data encompassing entire cities and micro-level data pertaining to specific locations, such as neighborhoods or streets. This capability of handling multi-granular data enables these models to interpret and forecast urban phenomena across different scales, a trait less prevalent in other foundation models.

\subsec{Domain specificity.}
UFMs are specifically tailored to tackle the unique challenges presented by urban-centric applications, offering advanced capabilities in handling the complexity, dynamism, and multidisciplinary nature of urban environments, distinguishing them from the more generalized scope of typical foundation models. This specialization enables them to provide more effective solutions in areas such as urban planning, traffic management, and public safety, compared to general foundation models.

\subsec{Spatio-temporal reasoning ability.}
UFMs excel in spatio-temporal reasoning, a capability crucial for analyzing and predicting the complex, ever-changing patterns of urban environments. This involves not just understanding data at a specific point in time but also how it evolves and interacts over both time and space. This spatio-temporal reasoning skill is particularly vital in urban contexts and is often less emphasized or absent in other foundation model types.

==> sections/dataset_old.tex <==
\section{Benchmarks and Datasets} 
\label{dataset}

\begin{table*}[th]
\centering
\tiny
\setlength{\tabcolsep}{4.0pt}
\renewcommand{\arraystretch}{1.15}
\begin{tabular}{p{1.5cm} p{1.9cm} p{3.0cm} p{3.0cm} p{3.0cm}}
\hline
\textbf{Benchmark} & \textbf{Data Modalities} & \textbf{Evaluated Abilities} & \textbf{Tasks} & \textbf{Metrics} \\
\hline

\textbf{USTBench} &
language + time series + trajectory + geovector &
spatiotemporal understanding; forecasting; planning; reflection-with-feedback; downstream applications &
4 prediction tasks: next-POI prediction; traffic congestion forecasting; socio-economic indicator prediction; OD prediction.
5 decision-making tasks: traffic-signal control; POI placement; route planning; road planning; urban planning &
process-level structured QA evaluation + task-specific quantitative metrics (e.g., MAPE/RMSE/Accuracy depending on task) \\
\hline

\textbf{CityBench} &
vision + language + trajectory + geovector &
urban perception \& understanding; planning \& decision-making &
8 tasks: image geo-localization; geospatial prediction; infrastructure inference; GeoQA for city elements; mobility prediction; urban exploration; outdoor navigation; traffic signal control &
task-specific quantitative metrics (e.g., Acc@1km/25km; $R^2$/RMSE; Recall@K/Top-1; success rate/avg steps/queue length) \\
\hline

\textbf{STBench} &
language + time series + trajectory + geovector &
knowledge comprehension; spatiotemporal reasoning; accurate computation; downstream applications &
15 tasks (4 dimensions): POI tasks; point tasks; trajectory tasks; region tasks (e.g., recognition/identification; relation reasoning; trajectory analysis/direction; anomaly detection/prediction/classification; flow prediction; navigation) &
QA accuracy + task-specific quantitative metrics (e.g., absolute error for trajectory prediction; MAE/RMSE for flow prediction) \\
\hline

\textbf{STARK} &
language + time series + trajectory &
state estimation; spatiotemporal reasoning; world-knowledge-aware reasoning &
field-variable prediction; localization/tracking; spatiotemporal relationship inference; landmark-/intent-aware navigation-style tasks &
challenge-level success/accuracy \\
\hline


\textbf{UrBench} &
vision + language &
geo-localization; scene understanding \& reasoning; object understanding; cross-view consistency &
14 QA tasks across 4 dimensions: geo-localization, scene understanding, scene reasoning, object understanding &
QA accuracy\\
\hline


\textbf{CityEQA} &
vision + language &
embodied active exploration; long-horizon planning; spatial reasoning; open-vocabulary embodied QA &
1.4k human-annotated QA tasks (6 categories) in the EmbodiedCity simulator &
QA accuracy + exploration-efficiency \\
\hline

\textbf{UrbanVideo-Bench} &
vision + language &
urban video understanding: recall; perception; reasoning; navigation \& planning &
5.2k MCQs covering 16 tasks and 4 aspects: recall, perception, reasoning, navigation) &
MCQ accuracy \\
\hline


\textbf{CityLens} &
vision + language & socioeconomic indicators prediction &
prediction tasks across economy, education, crime, transport, health, environment &
coefficient of determination~($R^2$) and normalized RMSE (nRMSE) \\
\hline

\textbf{LLM-UrbanPlan} &
language &
urban planning documentation; examinations; routine data analysis; AI algorithm support; thesis writing &
556 tasks across urban planning documentation; examinations; routine data analysis; AI algorithm support; thesis writing &
mixed automatic + human evaluation (e.g., human-rated accuracy/clarity/completeness/conciseness for explanations; correctness/syntax/clarity for code) \\
\hline

\textbf{TravelPlanner} &
language &
long-horizon planning; constraint satisfaction; tool-augmented reasoning &
real-world multi-day travel itinerary planning covering transportation, accommodation, dining, attractions, and inter-city routing under constraints &
delivery rate; commonsense pass rate; hard-constraint pass rate; final pass rate
\\
\hline

\end{tabular}
\caption{Summary of existing UFMs benchmarks by data modalities involved, evaluated abilities, representative tasks, and evaluation metrics.}
\label{tab:urban_benchmarks}
\end{table*}

\subsection{Benchmarks}
Recent years have witnessed a rapid emergence of benchmarks designed to evaluate UFMs across heterogeneous data modalities, reasoning paradigms, and application scenarios. As summarized in Table \ref{tab:urban_benchmarks}, existing benchmarks can be broadly grouped into three themes: spatiotemporal reasoning and decision-making, urban perception and embodiment, and professional urban tasks. 

Spatiotemporal reasoning and decision-making benchmarks focus on assessing whether large models can reason over dynamic urban processes involving space, time, and actions. Benchmarks such as USTBench, CityBench, STBench, and STARK evaluate models on tasks ranging from mobility and congestion forecasting to localization, trajectory reasoning, and navigation-style inference. A key distinction among them lies in how reasoning is evaluated. CityBench, STBench, and STARK primarily emphasize task-level correctness, measuring whether models can infer spatial–temporal relations or numerical outcomes under increasing complexity. In contrast, USTBench explicitly introduces process-level evaluation, probing intermediate reasoning steps (e.g., understanding, forecasting, planning, and reflection) rather than only final outcomes. Empirical findings across these benchmarks consistently show that while LLMs can handle short-horizon prediction and symbolic reasoning, they struggle with long-horizon planning, geometric reasoning, and error correction under feedback, indicating a gap between linguistic reasoning and actionable urban intelligence.

Urban perception and embodiment benchmarks extend evaluation into perceptual and embodied urban settings. Benchmarks such as UrBench, CityEQA, and UrbanVideo-Bench examine how multimodal models interpret urban scenes, reason over visual evidence, and support navigation. UrBench focuses on multi-view urban perception and cross-view consistency, evaluating large multimodal models on geo-localization, scene understanding and reasoning, object understanding, and consistency across street-view, aerial-view, and satellite-view imagery through diverse QA tasks. CityEQA and UrbanVideo-Bench move beyond static perception toward embodied and temporal understanding: CityEQA evaluates embodied active exploration and long-horizon spatial reasoning by requiring agents to navigate a realistic urban simulator to answer open-vocabulary questions, while UrbanVideo-Bench assesses urban video understanding across recall, perception, reasoning, and navigation using motion-rich city-scale video sequences. Collectively, results from these benchmarks reveal that although vision–language models can capture local visual cues, they still struggle with persistent spatial memory, causal and relational reasoning over time, and long-horizon consistency, particularly in open-ended, city-scale embodied settings that require integrating perception, memory, and decision-making.

Professional urban benchmarks target professional urban domain knowledge rather than perception or control. 
CityLens highlights the difficulty of inferring latent socioeconomic indicators from urban imagery, showing that visual grounding alone is insufficient for reliable quantitative prediction. 
LLM-UrbanPlan evaluates LLMs on hundreds of real-world urban planning tasks, spanning planning documentation, professional examinations, routine data analysis, algorithmic support, and academic writing, with a combination of automatic metrics and expert human judgments. TravelPlanner assesses long-horizon, constraint-intensive planning, requiring models to generate realistic multi-day travel itineraries under hard constraints on time, budget, transportation, and logistics, and evaluating plans using fine-grained constraint-satisfaction and execution-validity metrics.
These benchmarks expose a remarkable limitation of current foundation models: despite strong general language fluency and visual–semantic alignment, they struggle to support reliable urban analysis and planning, showing weak causal grounding for quantitative inference and uneven mastery of domain-specific constraints and standards. As a result, they often produce outputs that appear plausible but are brittle, shallow, or incorrect when faced with professional urban tasks. Even advanced reasoning-oriented models fall short of professional-level competence, underscoring the challenge of transferring general-purpose foundation models into specialized urban domains.


\hang{
\subsection{Datasets}
The development of Urban Foundation Models (UFMs) relies on a rich ecosystem of datasets that capture the multifaceted aspects of urban environments, human mobility, and environmental processes. As summarized in Table~\ref{tab:dataset_summary_long}, existing datasets can be categorized into six primary modalities: language, vision, time series, trajectory, geovector, and multimodal, each supporting distinct reasoning or predictive capabilities.

\textbf{Language datasets} provide regulatory, professional, and experiential knowledge essential for cognitive reasoning in urban and geoscience domains. Professional urban planning datasets, such as UrbanPlanBench~\cite{zheng2025urbanplanbench}, encode examination-based instruction pairs with standards-based reasoning, while TravelPlanner~\cite{xie2024travelplanner} and Travel-QA~\cite{meyer2024comparison} capture multi-constraint, real-world travel queries and crowd-sourced experiential knowledge. Geoscience QA datasets, including GeoBench~\cite{deng2024k2}, GeoSignal~\cite{deng2024k2}, and BB-GeoGPT-Dataset~\cite{zhang2024bb}, provide domain-specific knowledge for Earth observation and signal analysis. Environmental monitoring datasets, such as Global Earthquake Event~\cite{wang2024near} and Climate-FEVER~\cite{diggelmann2020climate}, support crisis informatics and climate verification research. Collectively, these linguistic datasets enable UFMs to perform structured reasoning, instruction following, and professional-domain comprehension.

\textbf{Visual datasets} span human-scale street imagery to city-scale aerial observations. Street-view datasets like Know-CL~\cite{liu2023knowledge} integrate imagery with urban knowledge graphs, whereas Million-AID~\cite{long2021creating} provides a global collection of aerial images for large-scale urban perception. Meteorological raster datasets, including ERA5~\cite{hersbach2020era5} and ExtremeWeather~\cite{racah2017extremeweather}, enable models to analyze spatiotemporal patterns in atmospheric processes and extreme events. These datasets support visual reasoning, geospatial understanding, and environmental situational awareness.

\textbf{Time series datasets} reflect the dynamic pulse of urban systems. Energy-focused datasets such as ETT~\cite{zhou2021informer}, Electricity~\cite{lai2018modeling}, and Solar-Energy~\cite{lai2018modeling} provide foundational power consumption sequences. Transportation datasets—including Traffic~\cite{lai2018modeling}, PEMS~\cite{song2020spatial}, METR-LA~\cite{li2018diffusion}, LargeST~\cite{liu2023largest}, TaxiBJ~\cite{zhang2017deep}, and NYC-BIKE~\cite{jin2022selective}—model citywide mobility at increasing spatiotemporal scales. Weather- and air-quality-related datasets, such as Weather~\cite{zhou2021informer}, City Temperature~\cite{xue2023promptcast}, and KnowAir~\cite{wang2020pm2}, provide environmental context crucial for forecasting and spatiotemporal reasoning. Together, these datasets enable UFMs to learn temporal dependencies, trend forecasting, and operational dynamics of urban systems.

\textbf{Trajectory datasets} encode mobility patterns and social behaviors. LBSN check-in datasets like Foursquare~\cite{yang2014modeling}, Gowalla~\cite{cho2011friendship}, and Yelp~\cite{wang2019kgat} capture social and recreational mobility preferences, whereas GPS-based trajectory datasets such as GeoLife~\cite{zheng2010geolife} and Portal-Taxi~\cite{jiang2023continuous} provide dense high-frequency mobility traces. These datasets underpin modeling of movement patterns, route prediction, and human–environment interactions.

\textbf{Geovector datasets} describe the structural and morphological fabric of cities. POI and road network datasets like OSM Data Extracts~\cite{tempelmeier2021geovectors}, HLG/DHM~\cite{zheng2023spatial}, and SARN-Dataset~\cite{chang2023spatial} capture connectivity and spatial topology. Region-level datasets such as PLUTO~\cite{liu2020learning} provide tax-lot and land-use information for planning and infrastructure analysis. Geovector data enable UFMs to reason over urban structure, accessibility, and land-use constraints.

\textbf{Multimodal datasets} integrate multiple modalities to support complex reasoning and planning tasks. Urban planning datasets, such as PlanBench-V~\cite{zhu-etal-2025-plangpt-vl}, combine maps with textual instructions for vision–language VQA. Travel planning datasets like TP-RAG~\cite{ni-etal-2025-tp} merge trajectories, POIs, and textual constraints for retrieval-augmented reasoning. Datasets for image geolocalization (LLMGeo-Dataset~\cite{wang2024llmgeo}) and weather reasoning (WeatherQA~\cite{ma2024weatherqa}) further exemplify cross-modal tasks. These datasets push UFMs toward integrated perception, reasoning, and planning in professional urban contexts.

Collectively, the diverse dataset modalities form the empirical backbone of UFMs, enabling the transition from general-purpose foundation models to specialized agents capable of urban, environmental, and mobility intelligence.
\begingroup
\tiny
\setlength{\tabcolsep}{4.0pt}
\renewcommand{\arraystretch}{1.10}

\begin{longtable}{>{\arraybackslash}m{1.5cm}|>{\arraybackslash}m{2.5cm}|>{\arraybackslash}m{3cm}|>{\arraybackslash}m{3.5cm}}
\caption{Summary of datasets available for building UFMs, by dataset modalities, dataset types, dataset links, and dataset descriptions.}
\label{tab:dataset_summary_long}\\
\hline
\textbf{Data Modality} &
\textbf{Data Type} &
\textbf{Dataset} &
\textbf{Data Description} \\
\hline
\endfirsthead

\hline
\textbf{Data Modality} &
\textbf{Data Type} &
\textbf{Dataset} &
\textbf{Data Description} \\
\hline
\endhead

% ================= Language =================
\multirow{8}{*}{\textbf{Language}}
& Urban Planning
& \href{https://github.com/tsinghua-fib-lab/PlanBench}{UrbanPlanBench~\cite{zheng2025urbanplanbench}}
& Based on 2022 exams; 30k+ instruction pairs; professional urban-planning standards. \\
\cline{2-4}

& \multirow{2}{*}{Travel Planning}
& \href{https://huggingface.co/datasets/osunlp/TravelPlanner}{TravelPlanner~\cite{xie2024travelplanner}}
& 1,000 real-world travel planning queries with multi-constraint itinerary tasks. \\
\cline{3-4}

&
& \href{https://huggingface.co/datasets/soniawmeyer/reddit-travel-QA-finetuning}{Travel-QA~\cite{meyer2024comparison}}
& 10k+ Reddit QA rows filtered by upvote ratio; experiential travel knowledge. \\
\cline{2-4}

& \multirow{3}{*}{Geoscience QA}
& \href{https://github.com/davendw49/k2}{GeoBench~\cite{deng2024k2}}
& Geoscience QA benchmark derived from exams (NPEE). \\
\cline{3-4}

&
& \href{https://github.com/davendw49/k2}{GeoSignal~\cite{deng2024k2}}
& 39k+ geoscience signal samples paired with QA tasks. \\
\cline{3-4}

&
& \href{https://github.com/AGI-GIS/BB-GeoGPT}{BB-GeoGPT-Dataset~\cite{zhang2024bb}}
& GIS-specific pretraining corpus and instruction-tuning dataset. \\
\cline{2-4}

& \multirow{2}{*}{Environmental Monitoring}
& \href{https://github.com/SusuXu-s-Lab/Hierarchical-Earthquake-Casualty-Information-Retrieval}{Global Earthquake Event~\cite{wang2024near}}
& 50M+ multilingual crisis tweets for earthquake casualty estimation. \\
\cline{3-4}

&
& \href{https://github.com/tdiggelm/climate-fever-dataset}{Climate-FEVER~\cite{diggelmann2020climate}}
& Climate claim verification dataset with Wikipedia evidence. \\
\hline

% ================= Vision =================
\multirow{4}{*}{\textbf{Vision}}
& Street-view Image
& \href{https://github.com/tsinghua-fib-lab/UrbanKG-KnowCL}{Know-CL-Dataset~\cite{liu2023knowledge}}
& Street-view and satellite imagery with urban knowledge graphs. \\
\cline{2-4}

& Remote Sensing Image
& \href{https://captain-whu.github.io/DiRS/}{Million-AID~\cite{long2021creating}}
& 1M+ aerial images, 51 categories, global coverage. \\
\cline{2-4}

& \multirow{2}{*}{Meteorological Rasters}
& \href{https://cds.climate.copernicus.eu/datasets/reanalysis-era5-single-levels}{ERA5~\cite{hersbach2020era5}}
& Global atmospheric reanalysis with high spatial-temporal resolution. \\
\cline{3-4}

&
& \href{https://extremeweatherdataset.github.io/}{ExtremeWeather~\cite{racah2017extremeweather}}
& Large-scale simulated extreme weather dataset with multi-channel labels. \\
\hline

% ================= Time Series =================
\multirow{12}{*}{\textbf{Time Series}}
& \multirow{3}{*}{Energy Consumption}
& \href{https://github.com/zhouhaoyi/ETDataset}{ETT~\cite{zhou2021informer}}
& Minute-level load and temperature time series for forecasting. \\
\cline{3-4}

&
& \href{https://github.com/laiguokun/multivariate-time-series-data}{Electricity~\cite{lai2018modeling}}
& Electricity consumption of 370 clients at 15-minute resolution. \\
\cline{3-4}

&
& \href{https://github.com/laiguokun/multivariate-time-series-data}{Solar-Energy~\cite{lai2018modeling}}
& Photovoltaic power generation time series. \\
\cline{2-4}

& \multirow{6}{*}{Transportation}
& \href{https://github.com/laiguokun/multivariate-time-series-data}{Traffic~\cite{lai2018modeling}}
& Multivariate traffic flow data with long-term temporal patterns. \\
\cline{3-4}

&
& \href{https://github.com/Davidham3/STSGCN}{PEMS~\cite{song2020spatial}}
& California freeway speed and flow sensor datasets. \\
\cline{3-4}

&
& \href{https://github.com/liuxu77/LargeST}{LargeST~\cite{liu2023largest}}
& Large-scale traffic forecasting benchmark with rich metadata. \\
\cline{3-4}

&
& \href{https://github.com/liyaguang/DCRNN}{METR-LA~\cite{li2018diffusion}}
& Highway speed dataset from Los Angeles. \\
\cline{3-4}

&
& \href{https://github.com/TolicWang/DeepST/tree/master/data/TaxiBJ}{TaxiBJ~\cite{zhang2017deep}}
& Citywide taxi flow data on 32×32 grids in Beijing. \\
\cline{3-4}

&
& \href{https://github.com/KL4805/CrossTReS}{NYC-BIKE~\cite{jin2022selective}}
& Large-scale bike-sharing ridership time series with weather. \\
\cline{2-4}

& \multirow{2}{*}{Weather}
& \href{https://github.com/zhouhaoyi/Informer2020}{Weather~\cite{zhou2021informer}}
& Daily temperature time series for 110 global cities. \\
\cline{3-4}

&
& \href{https://github.com/cruiseresearchgroup/PISA-PromptCast}{City Temperature~\cite{xue2023promptcast}}
& Sentence-style global temperature forecasting dataset. \\
\cline{2-4}

& Air Quality
& \href{https://github.com/shuowang-ai/PM2.5-GNN}{KnowAir~\cite{wang2020pm2}}
& PM2.5 and meteorological time series across Chinese cities. \\
\hline

% ================= Trajectory =================
\multirow{5}{*}{\textbf{Trajectory}}
& \multirow{3}{*}{POI Check-in}
& \href{https://sites.google.com/site/yangdingqi/home/foursquare-dataset}{Foursquare~\cite{yang2014modeling}}
& User check-in trajectories with social links. \\
\cline{3-4}

&
& \href{https://snap.stanford.edu/data/loc-gowalla.html}{Gowalla~\cite{cho2011friendship}}
& Global location-based social network mobility dataset. \\
\cline{3-4}

&
& \href{https://business.yelp.com/data/resources/open-dataset/}{Yelp~\cite{wang2019kgat}}
& POI check-ins and reviews across multiple cities. \\
\cline{2-4}

& \multirow{2}{*}{GPS Trajectory}
& \href{https://www.microsoft.com/en-us/research/publication/geolife-gps-trajectory-dataset-user-guide/}{GeoLife~\cite{zheng2010geolife}}
& High-frequency GPS trajectories with transportation modes. \\
\cline{3-4}

&
& \href{https://archive.ics.uci.edu/dataset/339/taxi+service+trajectory+prediction+challenge+ecml+pkdd+2015}{Portal-Taxi~\cite{jiang2023continuous}}
& Taxi GPS trajectories from Porto over nine months. \\
\hline

% ================= Geovector =================
\multirow{4}{*}{\textbf{Geovector}}
& POI
& \href{https://download.geofabrik.de/}{OSM Data Extracts~\cite{tempelmeier2021geovectors}}
& OpenStreetMap POIs and road networks for geospatial modeling. \\
\cline{2-4}

& \multirow{2}{*}{Road Network}
& \href{https://github.com/tsinghua-fib-lab/DRL-urban-planning}{HLG, DHM~\cite{zheng2023spatial}}
& Beijing road and land-block datasets for planning tasks. \\
\cline{3-4}

&
& \href{https://github.com/changyanchuan/SARN}{SARN-Dataset~\cite{chang2023spatial}}
& Road network embeddings preserving spatial topology. \\
\cline{2-4}

& Region
& \href{https://github.com/jackmiemie/GMEL/tree/master/data/PLUTO}{PLUTO~\cite{liu2020learning}}
& NYC land-use and tax-lot dataset with rich attributes. \\
\hline

% ================= Multimodal =================
\multirow{4}{*}{\textbf{Multimodal}}
& Urban Planning
& \href{https://github.com/zhuchichi56/PlanGPT-VL}{PlanBench-V~\cite{zhu-etal-2025-plangpt-vl}}
& Vision-language VQA on urban planning maps. \\
\cline{2-4}

& Travel Planning
& \href{https://github.com/usail-hkust/TP-RAG}{TP-RAG~\cite{ni-etal-2025-tp}}
& Retrieval-augmented travel planning with trajectories and POIs. \\
\cline{2-4}

& Image Geolocalization
& \href{https://github.com/yeyimilk/LLMGeo}{LLMGeo-Dataset~\cite{wang2024llmgeo}}
& Street-view images for country-level geolocation reasoning. \\
\cline{2-4}

& Weather QA
& \href{https://github.com/chengqianma/WeatherQA}{WeatherQA~\cite{ma2024weatherqa}}
& Multimodal reasoning over severe weather scenarios. \\
\hline

\end{longtable}

\endgroup
}

==> sections/taxonomy.tex <==
\begin{figure*}[tb]
\centering
\includegraphics[width=2\columnwidth]{figs/taxonomy_240114.png}
\caption{A detailed taxonomy of existing UFMs-related works based on the types of urban data modalities.}
\label{fig:taxonomy}
\end{figure*}

\onecolumn
\small % 或 \footnotesize 或 \scriptsize
\begin{longtable}{m{5mm}|m{2cm}m{2cm}m{2cm}m{2cm}m{2cm}m{2cm}m{2cm}}
    \caption{Summary of existing works.} \label{table:summary} \\
    \toprule
    \textbf{} & \textbf{Study} & \textbf{Data Type} & \textbf{Pre-training} & \textbf{Adaptation} & \textbf{Cross-modal transfer} & \textbf{Cross-domain transfer} & \textbf{Application} \\
    \midrule
    \endfirsthead

    \multicolumn{8}{c}{{\bfseries Table \thetable\ Summary of existing works (continued).}} \\
    \toprule
    \textbf{} & \textbf{Study} & \textbf{Data Type} & \textbf{Pre-training} & \textbf{Adaptation} & \textbf{Cross-modal transfer} & \textbf{Cross-domain transfer} & \textbf{Application} \\
    \midrule
    \endhead

    \midrule
    \multicolumn{8}{r}{{Continued on next page}} \\ 
    \endfoot

    \bottomrule
    \endlastfoot

    \multirow{10}{*}{\rotatebox{90}{\textbf{Language-based Models}}} & ERNIE-GeoL~\cite{huang2022ernie} & POI corpus, user behavior logs & Generative & Model fine-tuning & - & - & Map services \\
    \cline{2-8}
    ~ & MGeo~\cite{ding2023mgeo} & POI corpus & Generative, contrastive & Model fine-tuning & - & - & Query-POI matching \\
    \cline{2-8}
    ~ & Ji et al.~\cite{ji2023evaluating} & Geo-text, user instructions & - & Prompt engineering & - & General to geospatial & Geographic information systems \\
    \cline{2-8}
    ~ & Bhandari et al.~\cite{bhandari2023large} & Geo-text, user instructions & - & Prompt engineering & - & General to geospatial & Geographic information systems \\
    \cline{2-8}
    ~ & GPT4GEO~\cite{roberts2023gpt4geo} & Geo-text, user instructions & - & Prompt engineering & - & General to geospatial & Geographic information systems \\
    \cline{2-8}
    ~ & Mooney et al.~\cite{mooney2023towards} & Geo-text, user instructions & - & Prompt engineering & - & General to geospatial & Geographic information systems \\
    \cline{2-8}
    ~ & Mai et al.~\cite{mai2023opportunities} & Geo-text, user instructions & - & Prompt engineering & - & General to geospatial & Geographic information systems \\
    \cline{2-8}
    ~ & Fu et al.~\cite{fu2023towards} & Documents, geo-text, user instructions & - & Prompt engineering & - & General to urban science & Urban science \\
    \cline{2-8}
    ~ & Aghzal et al.~\cite{aghzal2023can} & Geo-text, user instructions & - & Prompt engineering & - & General to path planning & Path planning \\
    \cline{2-8}
    ~ & GeoLLM~\cite{manvi2023geollm} & POI corpus & - & Prompt engineering & - & General to geospatial & Geospatial prediction \\
    \cline{2-8}
    ~ & Zheng et al.~\cite{zheng2023chatgpt} & Traffic documents, user instructions & - & Prompt engineering & - & General to transportation & Intelligent transportation \\
    \cline{2-8}
    ~ & SpaBERT~\cite{li2022spabert}, GeoLM~\cite{li2023geolm} & Geo-text & - & Model fine-tuning & - & General to geospatial & Geographic language understanding \\
    \cline{2-8}
    ~ & QUERT~\cite{xie2023quert} & User behavior logs & - & Model fine-tuning & - & General to travel domain search & Travel query understanding \\
    \cline{2-8}
    ~ & GEDR~\cite{mei2023improving} & POI corpus, user behavior logs & - & Model fine-tuning & - & General to POI search & Query-POI matching \\
    \cline{2-8}
    ~ & Wang et al.~\cite{wang2023optimizing} & LLM-generated instructions & - & Model fine-tuning & - & General to urban renewal & Urban renewal \\
    \cline{2-8}
    ~ & K2~\cite{deng2023learning} & Geo-text, geoscience instructions & - & Model fine-tuning & - & General to geoscience & Geoscience tasks \\
    \midrule[0.5pt]
    
    \multirow{10}{*}{\rotatebox{90}{\textbf{Vision-based Models}}} & Urban2vec~\cite{wang2020urban2vec} & Street-view images & Contrastive & Model fine-tuning & - & - & \tabincell{c}{Demographic prediction, socioeconomic prediction} \\
    \cline{2-8}
    ~ & Li et al.~\cite{li2022predicting} & Street-view images & Contrastive & Model fine-tuning & - & - & Socioeconomic prediction \\
    \cline{2-8}
    ~ & KnowCL~\cite{liu2023knowledge} & Street-view images & Contrastive & Model fine-tuning & - & - & Socioeconomic prediction \\
    \cline{2-8}
    ~ & Wang et al.~\cite{wang2022advancing} & Remote sensing images & Generative & Model fine-tuning & - & - & \tabincell{c}{Remote sensing image analysis} \\
    \cline{2-8}
    ~ & ScaleMAE~\cite{reed2023scale} & Remote sensing images & Generative & Model fine-tuning & - & - & \tabincell{c}{Remote sensing image analysis} \\
    \cline{2-8}
    ~ & Cha et al.~\cite{cha2023billion} & Remote sensing images & Generative & Model fine-tuning & - & - & \tabincell{c}{Remote sensing image analysis} \\
    \cline{2-8}
    ~ & RingMo~\cite{sun2022ringmo} & Remote sensing images & Generative & Model fine-tuning & - & - & \tabincell{c}{Remote sensing image analysis} \\
    \cline{2-8}
    ~ & RingMo-Sense~\cite{yao2023ringmo} & Remote sensing images & Generative & Model fine-tuning & - & - & \tabincell{c}{Remote sensing spatiotemporal prediction} \\
    \cline{2-8}
    ~ & CSP~\cite{mai2023csp} & Remote sensing images & Contrastive & Model fine-tuning & Unimodel & - & \tabincell{c}{Satellite image classification} \\
    \cline{2-8}
    ~ & \tabincell{c}{FourCastNet~\cite{pathak2022fourcastnet}, Pangu-Weather~\cite{bi2023accurate}, FengWu~\cite{chen2023fengwu}} & Grid-based meteorological data & Generative & - & - & - & \tabincell{c}{Weather forecasting, tropical cyclones tracking} \\
    \cline{2-8}
    ~ & ClimaX~\cite{nguyen2023climax} & Grid-based meteorological data & Generative & Model fine-tuning & - & - & \tabincell{c}{Weather and climate modeling} \\
    \cline{2-8}
    ~ & W-MAE~\cite{man2023w} & Grid-based meteorological data & Generative & Model fine-tuning & - & - & \tabincell{c}{Weather forecasting, precipitation forecasting} \\
    \cline{2-8}
    ~ & SAMRS~\cite{wang2023samrs}, RSPrompter~\cite{chen2023rsprompter} & Remote sensing images & - & Prompt engineering & - & General to remote sensing & \tabincell{c}{Remote sensing semantic segmentation} \\
    \cline{2-8}
    ~ & Roberts et al.~\cite{roberts2023charting} & Remote sensing images & - & Prompt engineering & - & General to remote sensing & \tabincell{c}{Remote sensing image analysis} \\
    \cline{2-8}
    ~ & GeoSAM~\cite{sultan2023geosam} & Remote sensing images & - & Model fine-tuning & - & General to remote sensing & \tabincell{c}{Mobility infrastructure segmentation} \\
    \cline{2-8}
    ~ & RingMo-SAM~\cite{yan2023ringmo} & Remote sensing images & - & Model fine-tuning & - & General to remote sensing & \tabincell{c}{Multi-source remote sensing segmentation} \\
    \cline{2-8}
    ~ & Zhang et al.~\cite{zhang2022migratable} & Street-view images & - & Model fine-tuning & - & General to street scene sensing & \tabincell{c}{Street-view image analysis} \\
    \cline{2-8}
    ~ &  StreetCLIP~\cite{sultan2023geosam} & Street-view images & - & Model fine-tuning & - & General to street scene sensing & \tabincell{c}{Image geolocalization} \\
    
    % Trajectory-based Models
    \midrule[0.5pt]
    \multirow{10}{*}{\rotatebox{90}{\textbf{Trajectory-based Models}}} & t2vec~\cite{t2vec2018} & Trajectory in road networks & Generative & Model fine-tuning & - & - & \tabincell{c}{Similar trajectory search} \\
    \cline{2-8}
    ~ & traj2vec~\cite{traj2vec2017} & Trajectory in road networks & Generative & Model fine-tuning & - & - & \tabincell{c}{Trajectory cluster} \\
    \cline{2-8}
    ~ & Trembr~\cite{Trembr2020} & Trajectory in road networks & Generative & Model fine-tuning & - & - & \tabincell{c}{Similar trajectory search, travel time estimation, destination prediction} \\
    \cline{2-8}
    ~ & Toast~\cite{toast2021} & Trajectory in road networks & Generative & Model fine-tuning & - & - & \tabincell{c}{Road label classification, traffic inference, trajectory similarity search, travel time estimation} \\
    \cline{2-8}
    ~ & PIM~\cite{pim2021} & Trajectory in road networks & Contrastive & Model fine-tuning & - & - & \tabincell{c}{Travel time estimation, path ranking} \\
    \cline{2-8}
    ~ & STPT~\cite{stpt2023} & Trajectory in road networks & Contrastive & Model fine-tuning & - & - & \tabincell{c}{Trajectory classification, driving activity identification} \\
    \cline{2-8}
    ~ & LightPath~\cite{lightpath2023} & Trajectory in road networks & Generative & Model fine-tuning & - & - & \tabincell{c}{Travel time estimation, path ranking} \\
    \cline{2-8}
    ~ & MMTEC~\cite{mmtec2023} & Trajectory in road networks & Maximum Entropy Coding & Prompt engineering & - & - & \tabincell{c}{Similar trajectory search, travel time estimation,  destination prediction.} \\
    \cline{2-8}
    ~ & START~\cite{start2023} & Trajectory in road networks & \tabincell{c}{Generative, contrastive} & Prompt engineering & - & - & \tabincell{c}{Travel time estimation, trajectory classification, most similar trajectory search} \\
    \cline{2-8}
    ~ & HMTRL~\cite{hmtrl2022} & Trajectory in road networks & \tabincell{c}{Generative, contrastive} & Model fine-tuning & - & - & \tabincell{c}{Route recommendation} \\
    \cline{2-8}
    ~ & Movesim~\cite{movesim2020} & Trajectory in free space & \tabincell{c}{Generative, contrastive} & - & - & - & \tabincell{c}{Human mobility simulation} \\
    \cline{2-8}
    ~ & SML~\cite{sml2021} & Trajectory in free space & Contrastive & Model fine-tuning & - & - & \tabincell{c}{Location prediction, trajectory–user linking} \\
    \cline{2-8}
    ~ &  CTLE~\cite{ctle2021} & Trajectory in free space & Generative & - & - & - & \tabincell{c}{Next location prediction} \\
    \cline{2-8}
    ~ &  CACSR~\cite{cacsr2023} & Trajectory in free space & Contrastive & Model fine-tuning & - & - & \tabincell{c}{Next location prediction, trajectory user linking} \\
    \cline{2-8}
    ~ &  CATUS~\cite{CATUS2023} & Trajectory in free space & Contrastive & Model fine-tuning & - & - & \tabincell{c}{Next location prediction} \\
    \cline{2-8}
    ~ &  AuxMobLCast~\cite{auxmoblcast2022} & \tabincell{c}{Mobility prompt, user instructions} & - & Prompt engineering & Cross-modal & General to human mobility & \tabincell{c}{Human mobility forecasting} \\
    \cline{2-8}
    ~ &  LLM-Mob~\cite{llmmob2023} & \tabincell{c}{Mobility prompt, user instructions} & - & Prompt engineering & Cross-modal & General to human mobility & \tabincell{c}{Next location prediction} \\
    \cline{2-8}
    ~ &  Zhang et al.~\cite{zhang2023large} & \tabincell{c}{Mobility prompt, user instructions} & - & Prompt engineering & Cross-modal & General to human mobility & \tabincell{c}{Anomalous trajectory detection} \\
    \cline{2-8}
    ~ &  LLM-MPE~\cite{llmmpe2023} & \tabincell{c}{Mobility prompt, user instructions} & - & Prompt engineering & Cross-modal & General to human mobility & \tabincell{c}{Human mobility forecasting} \\
    \cline{2-8}
    ~ &  Keysan et al.~\cite{keysan2023can} & \tabincell{c}{Text description of scene, user instructions} & - & Prompt engineering & Cross-modal & General to autonomous driving & \tabincell{c}{Motion planning, driving trajectory prediction} \\
    \cline{2-8}
    ~ &  GPT-Driver~\cite{gptdriver2023} & \tabincell{c}{Text description of scene, user instructions} & - & Prompt engineering & Cross-modal & General to autonomous driving & \tabincell{c}{Motion planning, driving trajectory prediction} \\
    \cline{2-8}
    ~ &  LanguageMPC~\cite{languagempc2023} & \tabincell{c}{Text description of scene, user instructions} & - & Prompt engineering & Cross-modal & General to autonomous driving & \tabincell{c}{Motion planning, driving trajectory prediction} \\
    
    % Time series-based Models
    \midrule[0.5pt]
    \multirow{33}{*}{\rotatebox{90}{\textbf{Time series-based Models}}} 
    & Oreshkin et al.~\cite{oreshkin2021meta} & Ordinary time series & Supervised & - & Unimodal & Electricity to traffic & \tabincell{c}{Energy consumption forecasting, traffic forecasting}\\
    \cline{2-8}
    ~ & Lag-Llama~\cite{rasul2023lag} & Ordinary time series & Supervised & - & Unimodal & General to traffic & Traffic forecasting\\
    \cline{2-8}
    ~ & SASA~\cite{cai2021time} & Ordinary time series & Supervised & - & Unimodal & - & Air quality regression\\
    \cline{2-8}
    ~ & TST~\cite{zerveas2021transformer} & Ordinary time series & Generative & - & Unimodal & - & Traffic regression\\
    \cline{2-8}
    ~ & SimMTM~\cite{dong2023simmtm} & Ordinary time series & Generative & - & Unimodal & Weather to traffic & \tabincell{c}{Weather forecasting, energy consumption forecasting, traffic forecasting}\\
    \cline{2-8}
    ~ & PatchTST~\cite{nie2022time} & Ordinary time series & Generative & - & Unimodal & Electricity to others & \tabincell{c}{Weather forecasting, energy consumption forecasting, traffic forecasting}\\
    \cline{2-8}
    ~ & TSMixer~\cite{ekambaram2023tsmixer} & Ordinary time series & Generative & - & Unimodal & - & \tabincell{c}{Weather forecasting, energy consumption forecasting, traffic forecasting}\\
    \cline{2-8}
    ~ & PT-Tuning~\cite{liu2023pt} & Ordinary time series & Generative & Prompt engineering & Unimodal & - & \tabincell{c}{Weather forecasting, energy consumption forecasting, traffic forecasting}\\
    \cline{2-8}
    ~ & T-Loss~\cite{franceschi2019unsupervised} & Ordinary time series & Contrastive & - & Unimodal & - & \tabincell{c}{Traffic forecasting, energy consumption forecasting}\\
    \cline{2-8}
    ~ & COST~\cite{woo2022cost} & Ordinary time series & Contrastive & - & Unimodal & - & \tabincell{c}{Weather forecasting, energy consumption forecasting, traffic forecasting}\\
    \cline{2-8}
    ~ & TS2Vec~\cite{yue2022ts2vec} & Ordinary time series & Contrastive & - & Unimodal & - & \tabincell{c}{Traffic classification, energy consumption classification}\\
    \cline{2-8}
    ~ & SimTS~\cite{zheng2023simts} & Ordinary time series & Contrastive & - & Unimodal & - & \tabincell{c}{Weather forecasting, traffic forecasting}\\
    \cline{2-8}
    ~ & UniTime~\cite{liu2023unitime} & Ordinary time series & Hybrid & - & Unimodal & General to urban time series & \tabincell{c}{Weather forecasting, energy consumption forecasting, traffic forecasting}\\
    \cline{2-8}
    ~ & ST-GSP~\cite{zhao2022st} & Spatial time series & Generative & - & Unimodal & - & Traffic forecasting\\
    \cline{2-8}
    ~ & STGCL~\cite{liu2022contrastive} & Spatial time series & Contrastive & - & Unimodal & - & Traffic forecasting\\
    \cline{2-8}
    ~ & STEP~\cite{shao2022pre} & Spatial time series & Generative & - & Unimodal & - & Traffic forecasting\\
    \cline{2-8}
    ~ & TransGTR~\cite{jin2023transferable} & Spatial time series & Hybrid & - & Unimodal & - & Traffic forecasting\\
    \cline{2-8}
    ~ & MC-STL~\cite{zhang2023mask} & Spatial time series & Hybrid & - & Unimodal & - & Traffic forecasting\\
    \cline{2-8}
    ~ & TPB~\cite{liu2023cross} & Spatial time series & Hybrid & - & Unimodal & - & Traffic forecasting\\
    \cline{2-8}
    ~ & GPT-ST~\cite{li2023gpt} & Spatial time series & Generative & - & Unimodal & - & Traffic forecasting\\
    \cline{2-8}
    ~ & PromptST~\cite{zhang2023promptst} & Spatial time series & - & Prompt engineering & Unimodal & - & \tabincell{c}{Traffic forecasting, complaint forecasting}\\
    \cline{2-8}
    ~ & MetePFL~\cite{chen2023prompt} & Spatial time series & - & Prompt engineering & Unimodal & - & Weather forecasting\\
    \cline{2-8}
    ~ & FedWing~\cite{chen2023spatial} & Spatial time series & - & Prompt engineering & Unimodal & - & Weather forecasting\\
    \cline{2-8}
    ~ & PromptCast~\cite{xue2023promptcast} & Ordinary time series & - & Prompt engineering & Cross-modal & Language to time series & \tabincell{c}{Weather forecasting, energy consumption forecasting, human mobility forecasting}\\
    \cline{2-8} 
    ~ & LLMTime~\cite{gruver2023large} & Ordinary time series & - & Prompt engineering & Cross-modal & Language to time series & \tabincell{c}{Weather forecasting, energy consumption forecasting, traffic forecasting}\\
    \cline{2-8} 
    ~ & GPT(6)~\cite{zhou2023one1_nips} & Ordinary time series & - & Model fine-tuning & Cross-modal & Language to time series & \tabincell{c}{Weather forecasting, energy consumption forecasting, traffic forecasting}\\
    \cline{2-8} 
    ~ & GPT(6)-adapter~\cite{zhou2023one2} & Ordinary time series & - & Model fine-tuning & Cross-modal & Language to time series & \tabincell{c}{Weather forecasting, energy consumption forecasting, traffic forecasting}\\
    \cline{2-8} 
    ~ & LLM4TS~\cite{chang2023llm4ts} & Ordinary time series & - & Model fine-tuning & Cross-modal & Language to time series & \tabincell{c}{Weather forecasting, energy consumption forecasting, traffic forecasting}\\
    \cline{2-8} 
    ~ & TEMPO~\cite{cao2023tempo} & Ordinary time series & - & Model fine-tuning & Cross-modal & Language to time series & \tabincell{c}{Weather forecasting, energy consumption forecasting, traffic forecasting}\\
    \cline{2-8} 
    ~ & GATGPT~\cite{chen2023gatgpt} & Spatial time series & - & Model fine-tuning & Cross-modal & Language to time series & \tabincell{c}{Traffic forecasting, air quality imputation}\\
    \cline{2-8} 
    ~ & V2S~\cite{yang2021voice2series} & Ordinary time series & - & Model Reprogramming & Cross-modal & Speech to time series & Traffic classification\\
    \cline{2-8} 
    ~ & Time-LLM~\cite{jin2023time} & Ordinary time series & - & Model reprogramming & Cross-modal & Language to time series & Traffic forecasting\\
    \cline{2-8}
    ~ & TEST~\cite{sun2023test} & Ordinary time series & - & Model reprogramming & Cross-modal & Language to time series & \tabincell{c}{Traffic forecasting, energy consumption forecasting, air quality forecasting}\\
    
    \midrule[0.5pt]
    \multirow{14}{*}{\rotatebox{90}{\textbf{Multimodal Models}}} &  UrbanCLIP~\cite{yan2023urban} & Satellite image, textual description	& Contrastive & Model fine-tuning & LLM for image & General to urban science & Urban region profiling \\
    \cline{2-8}
    ~ & TengYun~\cite{zhao2023parallel} & Traffic-related text and image & Generative & Prompt tuning & - & - & \tabincell{c}{Traffic prediction and control, transportation planning} \\
    \cline{2-8}
    ~ & CityFM~\cite{balsebre2023city} & Spatial, visual, and textual geo-data & Contrastive	& -	& -	& -	& \tabincell{c}{Traffic speed inference, building functionality classification}\\
    \cline{2-8}
    ~ & AllSpark~\cite{shao2023allspark} & Text, image, trajectory, graph, etc.	& Contrastive &	Prompt engineering & - & - & Spatiotemporal data analysis \\
    \cline{2-8}
    ~ & TrafficGPT~\cite{zhang2023trafficgpt} & Multimodal traffic data & - & Prompt engineering & - & General to traffic management & Traffic management \\
    \cline{2-8}
    ~ & GeoGPT~\cite{zhang2023geogpt} & Multimodal geospatial data	& -	& Prompt tuning	& -	& General to geospatial & \tabincell{c}{Autonomous geospatial data collection, processing, and analysis} \\
    \cline{2-8}
    ~ & VELMA~\cite{schumann2023velma} & Street image, navigation instruction	& -	& Model fine-tuning	& LLM for image	& General to urban navigation & Autonomous street navigation \\
    \cline{2-8}
    ~ & UGI~\cite{xu2023urban} & \tabincell{c}{Urban textual, visual, knowledge graph, human behavior data} & - & \tabincell{c}{Continue learning,  model fine-tuning} & - & General to urban environment & \tabincell{c}{Urban planning and simulation, location recommendation} \\
    % \bottomrule[1pt]
\end{longtable}
\normalsize
\twocolumn



% \begin{table*}[tb]
%     % \tiny
%     % \small
%     \centering
%     \caption{Summary of existing works.}
%     \vspace{-2mm}
%     % \setlength{\tabcolsep}{2.5mm}{
%     \resizebox{\textwidth}{!}{
%         \begin{tabular}{c|ccccccc}
%             \toprule[1pt]
%             \textbf{} & 
%             \textbf{Study} & \textbf{Data Type} & \textbf{Pre-training} & \textbf{Adaptation} & \textbf{Cross-modal transfer} & \textbf{Cross-domain transfer} & \textbf{Application} \\
%             \midrule[0.5pt]
%             \multirow{10}{*}{\rotatebox{90}{\textbf{Language-based Models}}} & ERNIE-GeoL~\cite{huang2022ernie} & POI corpus, user behavior logs & Generative & Model fine-tuning & - & - & Map services \\
%             \cline{2-8}
%             ~ & MGeo~\cite{ding2023mgeo} & POI corpus & Generative, contrastive & Model fine-tuning & - & - & Query-POI matching \\
%             \cline{2-8}
%             ~ & \tabincell{c}{Ji et al.~\cite{ji2023evaluating}, Bhandari et al.~\cite{bhandari2023large}, \\ GPT4GEO~\cite{roberts2023gpt4geo}, Mooney et al.~\cite{mooney2023towards}, \\ Mai et al.~\cite{mai2023opportunities}} & Geo-text, user instructions & - & Prompt engineering & - & General to geospatial & Geographic information systems \\
%             \cline{2-8}
%             ~ & Fu et al.~\cite{fu2023towards} & Documents, geo-text, user instructions & - & Prompt engineering & - & General to urban science & Urban science \\
%             \cline{2-8}
%             ~ & Aghzal et al.~\cite{aghzal2023can} & Geo-text, user instructions & - & Prompt engineering & - & General to path planning & Path planning \\
%             \cline{2-8}
%             ~ & GeoLLM~\cite{manvi2023geollm} & POI corpus & - & Prompt engineering & - & General to geospatial & Geospatial prediction \\
%             \cline{2-8}
%             ~ & Zheng et al.~\cite{zheng2023chatgpt} & Traffic documents, user instructions & - & Prompt engineering & - & General to transportation & Intelligent transportation \\
%             \cline{2-8}
%             ~ & SpaBERT~\cite{li2022spabert}, GeoLM~\cite{li2023geolm} & Geo-text & - & Model fine-tuning & - & General to geospatial & Geographic language understanding \\
%             \cline{2-8}
%             ~ & QUERT~\cite{xie2023quert} & User behavior logs & - & Model fine-tuning & - & General to travel domain search & Travel query understanding \\
%             \cline{2-8}
%             ~ & GEDR~\cite{mei2023improving} & POI corpus, user behavior logs & - & Model fine-tuning & - & General to POI search & Query-POI matching \\
%             \cline{2-8}
%             ~ & Wang et al.~\cite{wang2023optimizing} & LLM-generated instructions & - & Model fine-tuning & - & General to urban renewal & Urban renewal \\
%             \cline{2-8}
%             ~ & K2~\cite{deng2023learning} & Geo-text, geoscience instructions & - & Model fine-tuning & - & General to geoscience & Geoscience tasks \\
%             \cline{2-8}
%             \midrule[0.5pt]
            
%             \multirow{10}{*}{\rotatebox{90}{\textbf{Vision-based Models}}} & Urban2vec~\cite{wang2020urban2vec} & Street-view images & Contrastive & Model fine-tuning & - & - & \tabincell{c}{Demographic prediction, \\ socioeconomic prediction} \\
%             \cline{2-8}
%             ~ & Li et al.~\cite{li2022predicting} & Street-view images & Contrastive & Model fine-tuning & - & - & Socioeconomic prediction \\
%             \cline{2-8}
%             ~ & KnowCL~\cite{liu2023knowledge} & Street-view images & Contrastive & Model fine-tuning & - & - & Socioeconomic prediction \\
%             \cline{2-8}
%             ~ & \tabincell{c}{Wang et al.~\cite{wang2022advancing}, ScaleMAE~\cite{reed2023scale}, \\ Cha et al.~\cite{cha2023billion}, RingMo~\cite{sun2022ringmo}} & Remote sensing images & Generative & Model fine-tuning & - & - & \tabincell{c}{Remote sensing image analysis} \\
%             \cline{2-8}
%             ~ & RingMo-Sense~\cite{yao2023ringmo} & Remote sensing images & Generative & Model fine-tuning & - & - & \tabincell{c}{Remote sensing spatiotemporal prediction} \\
%             \cline{2-8}
%             % ~ & ScaleMAE~\cite{reed2023scale} & Remote sensing images & Generative & Model fine-tuning & Unimodel & - & \tabincell{c}{Remote sensing object detection \\ and semantic segmentation} \\
%             % \cline{2-8}
%             % ~ & Cha et al.~\cite{cha2023billion} & Remote sensing images & Generative & Model fine-tuning & Unimodel & - & \tabincell{c}{Remote sensing scene classification, \\ object detection, semantic segmentation, and change detection} \\
%             % \cline{2-8}
%             % ~ & RingMo~\cite{yao2023ringmo} & Remote sensing images & Generative & Model fine-tuning & Unimodel & - & \tabincell{c}{Remote sensing scene classification \\ and semantic segmentation} \\
%             % \cline{2-8}
%             ~ & CSP~\cite{mai2023csp} & Remote sensing images & Contrastive & Model fine-tuning & Unimodel & - & \tabincell{c}{Satellite image classification} \\
%             \cline{2-8}
%             ~ & \tabincell{c}{FourCastNet~\cite{pathak2022fourcastnet}, \\ Pangu-Weather~\cite{bi2023accurate}, FengWu~\cite{chen2023fengwu}} & Grid-based meteorological data & Generative & - & - & - & \tabincell{c}{Weather forecasting, \\ tropical cyclones tracking} \\
%             \cline{2-8}
%             ~ & ClimaX~\cite{nguyen2023climax} & Grid-based meteorological data & Generative & Model fine-tuning & - & - & \tabincell{c}{Weather and climate modeling} \\
%             \cline{2-8}
%             ~ & W-MAE~\cite{man2023w} & Grid-based meteorological data & Generative & Model fine-tuning & - & - & \tabincell{c}{Weather forecasting, \\ precipitation forecasting} \\
%             \cline{2-8}
%             ~ & SAMRS~\cite{wang2023samrs}, RSPrompter~\cite{chen2023rsprompter} & Remote sensing images & - & Prompt engineering & - & General to remote sensing & \tabincell{c}{Remote sensing semantic segmentation} \\
%             \cline{2-8}
%             \cline{2-8}
%             ~ & Roberts et al.~\cite{roberts2023charting} & Remote sensing images & - & Prompt engineering & - & General to remote sensing & \tabincell{c}{Remote sensing image analysis} \\
%             \cline{2-8}
%             ~ & GeoSAM~\cite{sultan2023geosam} & Remote sensing images & - & Model fine-tuning & - & General to remote sensing & \tabincell{c}{Mobility infrastructure segmentation} \\
%             \cline{2-8}
%             ~ & RingMo-SAM~\cite{yan2023ringmo} & Remote sensing images & - & Model fine-tuning & - & General to remote sensing & \tabincell{c}{Multi-source remote sensing segmentation} \\
%             \cline{2-8}
%             ~ & Zhang et al.~\cite{zhang2022migratable} & Street-view images & - & Model fine-tuning & - & General to street scene sensing & \tabincell{c}{Street-view image analysis} \\
%             \cline{2-8}
%             ~ &  StreetCLIP~\cite{sultan2023geosam} & Street-view images & - & Model fine-tuning & - & General to street scene sensing & \tabincell{c}{Image geolocalization} \\
%             \cline{2-8}
            
%             % Trajectory-based Models
%             \midrule[0.5pt]
%             \multirow{40}{*}{\rotatebox{90}{\textbf{Trajectory-based Models}}} & t2vec~\cite{t2vec2018} & Trajectory in road networks & Generative & Model fine-tuning & - & - & \tabincell{c}{Similar trajectory search} \\
%             \cline{2-8}
%             ~ & traj2vec~\cite{traj2vec2017} & Trajectory in road networks & Generative & Model fine-tuning & - & - & \tabincell{c}{Trajectory cluster} \\
%             \cline{2-8}
%             ~ & Trembr~\cite{Trembr2020} & Trajectory in road networks & Generative & Model fine-tuning & - & - & \tabincell{c}{Similar trajectory search,\\ travel time estimation,\\ destination prediction} \\
%             \cline{2-8}
%             ~ & Toast~\cite{toast2021} & Trajectory in road networks & Generative & Model fine-tuning & - & - & \tabincell{c}{Road label classification,\\ traffic inference,\\ trajectory similarity search,\\ travel time estimation} \\
%             \cline{2-8}
%             ~ & PIM~\cite{pim2021} & Trajectory in road networks & Contrastive & Model fine-tuning & - & - & \tabincell{c}{Travel time estimation,\\ path ranking} \\
%             \cline{2-8}
%             ~ & STPT~\cite{stpt2023} & Trajectory in road networks & Contrastive & Model fine-tuning & - & - & \tabincell{c}{Trajectory classification,\\ driving activity identification} \\
%             \cline{2-8}
%             ~ & LightPath~\cite{lightpath2023} & Trajectory in road networks & Generative & Model fine-tuning & - & - & \tabincell{c}{Travel time estimation,\\ path ranking} \\
%             \cline{2-8}
%             ~ & MMTEC~\cite{mmtec2023} & Trajectory in road networks & Maximum Entropy Coding & Prompt engineering & - & - & \tabincell{c}{Similar trajectory search,\\ travel time estimation,\\  destination prediction.} \\
%             % \cline{2-8}
%             \cline{2-8}
%             ~ & START~\cite{start2023} & Trajectory in road networks & \tabincell{c}{Generative,\\ contrastive} & Prompt engineering & - & - & \tabincell{c}{Travel time estimation,\\ trajectory classification,\\ most similar trajectory search} \\
%             \cline{2-8}
%             ~ & HMTRL~\cite{hmtrl2022} & Trajectory in road networks & \tabincell{c}{Generative,\\ contrastive} & Model fine-tuning & - & - & \tabincell{c}{Route recommendation} \\
%             \cline{2-8}
%             ~ & Movesim~\cite{movesim2020} & Trajectory in free space & \tabincell{c}{Generative,\\ contrastive} & - & - & - & \tabincell{c}{Human mobility simulation} \\
%             \cline{2-8}
%             ~ & SML~\cite{sml2021} & Trajectory in free space & Contrastive & Model fine-tuning & - & - & \tabincell{c}{Location prediction,\\ trajectory–user linking} \\
%             \cline{2-8}
%             ~ &  CTLE~\cite{ctle2021} & Trajectory in free space & Generative & - & - & - & \tabincell{c}{Next location prediction} \\
%             \cline{2-8}
%             ~ &  CACSR~\cite{cacsr2023} & Trajectory in free space & Contrastive & Model fine-tuning & - & - & \tabincell{c}{Next location prediction,\\ trajectory user linking} \\
%             \cline{2-8}
%             ~ &  CATUS~\cite{CATUS2023} & Trajectory in free space & Contrastive & Model fine-tuning & - & - & \tabincell{c}{Next location prediction} \\
%             \cline{2-8}
%             ~ &  AuxMobLCast~\cite{auxmoblcast2022} & \tabincell{c}{Mobility prompt,\\ user instructions} & - & Prompt engineering & Cross-modal & General to human mobility & \tabincell{c}{Human mobility forecasting} \\
%             \cline{2-8}
%             ~ &  LLM-Mob~\cite{llmmob2023} & \tabincell{c}{Mobility prompt,\\ user instructions} & - & Prompt engineering & Cross-modal & General to human mobility & \tabincell{c}{Next location prediction} \\
%             \cline{2-8}
%             ~ &  Zhang et al.~\cite{zhang2023large} & \tabincell{c}{Mobility prompt,\\ user instructions} & - & Prompt engineering & Cross-modal & General to human mobility & \tabincell{c}{Anomalous trajectory detection} \\
%             \cline{2-8}
%             ~ &  LLM-MPE~\cite{llmmpe2023} & \tabincell{c}{Mobility prompt,\\ user instructions} & - & Prompt engineering & Cross-modal & General to human mobility & \tabincell{c}{Human mobility forecasting} \\
%             \cline{2-8}
%             ~ &  Keysan et al.~\cite{keysan2023can} & \tabincell{c}{Text description of scene,\\ user instructions} & - & Prompt engineering & Cross-modal & General to autonomous driving & \tabincell{c}{Motion planning,\\ driving trajectory prediction} \\
%             \cline{2-8}
%             ~ &  GPT-Driver~\cite{gptdriver2023} & \tabincell{c}{Text description of scene,\\ user instructions} & - & Prompt engineering & Cross-modal & General to autonomous driving & \tabincell{c}{Motion planning,\\ driving trajectory prediction} \\
%             \cline{2-8}
%             ~ &  LanguageMPC~\cite{languagempc2023} & \tabincell{c}{Text description of scene,\\ user instructions} & - & Prompt engineering & Cross-modal & General to autonomous driving & \tabincell{c}{Motion planning,\\ driving trajectory prediction} \\
%             \cline{2-8}
            
%             % Time series-based Models
%             \midrule[0.5pt]
%             \multirow{33}{*}{\rotatebox{90}{\textbf{Time series-based Models}}} 
%             & Oreshkin et al.~\cite{oreshkin2021meta} & Ordinary time series & Supervised & - & Unimodal & Electricity to traffic & \tabincell{c}{Energy consumption forecasting,\\ traffic forecasting}\\
%             \cline{2-8}
%             ~ & Lag-Llama~\cite{rasul2023lag} & Ordinary time series & Supervised & - & Unimodal & General to traffic & Traffic forecasting\\
%             \cline{2-8}
%             % ~ & CoDATS~\cite{wilson2020multi} & Ordinary time series & Supervised & - & Unimodal & - & -\\
%             % \cline{2-8}
%             ~ & SASA~\cite{cai2021time} & Ordinary time series & Supervised & - & Unimodal & - & Air quality regression\\
%             \cline{2-8}
            
%             ~ & TST~\cite{zerveas2021transformer} & Ordinary time series & Generative & - & Unimodal & - & Traffic regression\\
%             \cline{2-8}
%             ~ & SimMTM~\cite{dong2023simmtm} & Ordinary time series & Generative & - & Unimodal & Weather to traffic & \tabincell{c}{Weather forecasting,\\ energy consumption forecasting,\\ traffic forecasting}\\
%             \cline{2-8}
%             ~ & PatchTST~\cite{nie2022time} & Ordinary time series & Generative & - & Unimodal & Electricity to others & \tabincell{c}{Weather forecasting,\\ energy consumption forecasting,\\ traffic forecasting}\\
%             \cline{2-8}
%             ~ & TSMixer~\cite{ekambaram2023tsmixer} & Ordinary time series & Generative & - & Unimodal & - & \tabincell{c}{Weather forecasting,\\ energy consumption forecasting,\\ traffic forecasting}\\
%             \cline{2-8}
%             ~ & PT-Tuning~\cite{liu2023pt} & Ordinary time series & Generative & Prompt engineering & Unimodal & - & \tabincell{c}{Weather forecasting,\\ energy consumption forecasting,\\ traffic forecasting}\\
%             \cline{2-8}
            
%             ~ & T-Loss~\cite{franceschi2019unsupervised} & Ordinary time series & Contrastive & - & Unimodal & - & \tabincell{c}{Traffic forecasting,\\ energy consumption forecasting}\\
%             \cline{2-8}
%             % ~ & TS-TCC~\cite{eldele2021time} & Ordinary time series & Contrastive & - & Unimodal & - & -\\
%             % \cline{2-8}
%             ~ & COST~\cite{woo2022cost} & Ordinary time series & Contrastive & - & Unimodal & - & \tabincell{c}{Weather forecasting,\\ energy consumption forecasting,\\ traffic forecasting}\\
%             \cline{2-8}
%             % ~ & TNC~\cite{tonekaboni2021unsupervised} & Ordinary time series & Contrastive & - & Unimodal & - & -\\
%             % \cline{2-8}
%             ~ & TS2Vec~\cite{yue2022ts2vec} & Ordinary time series & Contrastive & - & Unimodal & - & \tabincell{c}{Traffic classification,\\ energy consumption classification}\\
%             \cline{2-8}
%             ~ & SimTS~\cite{zheng2023simts} & Ordinary time series & Contrastive & - & Unimodal & - & \tabincell{c}{Weather forecasting,\\ traffic forecasting}\\
%             \cline{2-8}
            
%             % ~ & SLARDA~\cite{ragab2022self} & Ordinary time series & Hybrid & - & Unimodal & - & -\\
%             % \cline{2-8}
%             ~ & UniTime~\cite{liu2023unitime} & Ordinary time series & Hybrid & - & Unimodal & General to urban time series & \tabincell{c}{Weather forecasting,\\ energy consumption forecasting,\\ traffic forecasting}\\
%             \cline{2-8}
            
%             ~ & ST-GSP~\cite{zhao2022st} & Spatial time series & Generative & - & Unimodal & - & Traffic forecasting\\
%             \cline{2-8}
%             ~ & STGCL~\cite{liu2022contrastive} & Spatial time series & Contrastive & - & Unimodal & - & Traffic forecasting\\
%             \cline{2-8}
%             ~ & STEP~\cite{shao2022pre} & Spatial time series & Generative & - & Unimodal & - & Traffic forecasting\\
%             \cline{2-8}
%             ~ & TransGTR~\cite{jin2023transferable} & Spatial time series & Hybrid & - & Unimodal & - & Traffic forecasting\\
%             \cline{2-8}
%             ~ & MC-STL~\cite{zhang2023mask} & Spatial time series & Hybrid & - & Unimodal & - & Traffic forecasting\\
%             \cline{2-8}
%             ~ & TPB~\cite{liu2023cross} & Spatial time series & Hybrid & - & Unimodal & - & Traffic forecasting\\
%             \cline{2-8}
%             ~ & GPT-ST~\cite{li2023gpt} & Spatial time series & Generative & - & Unimodal & - & Traffic forecasting\\
%             \cline{2-8}
            
%             % ~ & POND~\cite{wang2023prompt} & Ordinary time series & - & Prompt engineering & Unimodal & - & -\\
%             % \cline{2-8}
%             ~ & PromptST~\cite{zhang2023promptst} & Spatial time series & - & Prompt engineering & Unimodal & - & \tabincell{c}{Traffic forecasting,\\ complaint forecasting}\\
%             \cline{2-8}
%             ~ & MetePFL~\cite{chen2023prompt} & Spatial time series & - & Prompt engineering & Unimodal & - & Weather forecasting\\
%             \cline{2-8}
%             ~ & FedWing~\cite{chen2023spatial} & Spatial time series & - & Prompt engineering & Unimodal & - & Weather forecasting\\
%             \cline{2-8}

%             ~ & PromptCast~\cite{xue2023promptcast} & Ordinary time series & - & Prompt engineering & Cross-modal & Language to time series & \tabincell{c}{Weather forecasting,\\ energy consumption forecasting,\\ human mobility forecasting}\\
%             \cline{2-8} 
%             ~ & LLMTime~\cite{gruver2023large} & Ordinary time series & - & Prompt engineering & Cross-modal & Language to time series & \tabincell{c}{Weather forecasting,\\ energy consumption forecasting,\\ traffic forecasting}\\
%             \cline{2-8} 
%             ~ & GPT(6)~\cite{zhou2023one1_nips} & Ordinary time series & - & Model fine-tuning & Cross-modal & Language to time series & \tabincell{c}{Weather forecasting,\\ energy consumption forecasting,\\ traffic forecasting}\\
%             \cline{2-8} 
%             ~ & GPT(6)-adapter~\cite{zhou2023one2} & Ordinary time series & - & Model fine-tuning & Cross-modal & Language to time series & \tabincell{c}{Weather forecasting,\\ energy consumption forecasting,\\ traffic forecasting}\\
%             \cline{2-8} 
%             ~ & LLM4TS~\cite{chang2023llm4ts} & Ordinary time series & - & Model fine-tuning & Cross-modal & Language to time series & \tabincell{c}{Weather forecasting,\\ energy consumption forecasting,\\ traffic forecasting}\\
%             \cline{2-8} 
%             ~ & TEMPO~\cite{cao2023tempo} & Ordinary time series & - & Model fine-tuning & Cross-modal & Language to time series & \tabincell{c}{Weather forecasting,\\ energy consumption forecasting,\\ traffic forecasting}\\
%             \cline{2-8} 
%             ~ & GATGPT~\cite{chen2023gatgpt} & Spatial time series & - & Model fine-tuning & Cross-modal & Language to time series & \tabincell{c}{Traffic forecasting,\\ air quality imputation}\\
%             \cline{2-8} 
%             ~ & V2S~\cite{yang2021voice2series} & Ordinary time series & - & Model Reprogramming & Cross-modal & Speech to time series & Traffic classification\\
%             \cline{2-8} 
%             ~ & Time-LLM~\cite{jin2023time} & Ordinary time series & - & Model reprogramming & Cross-modal & Language to time series & Traffic forecasting\\
%             \cline{2-8}
%             ~ & TEST~\cite{sun2023test} & Ordinary time series & - & Model reprogramming & Cross-modal & Language to time series & \tabincell{c}{Traffic forecasting,\\ energy consumption forecasting,\\ air quality forecasting}\\
            
%             \midrule[0.5pt]
%             \multirow{14}{*}{\rotatebox{90}{\textbf{Multimodal Models}}} &  UrbanCLIP~\cite{yan2023urban} & Satellite image, textual description	& Contrastive & Model fine-tuning & LLM for image & General to urban science & Urban region profiling \\
%             \cline{2-8}
%             ~ & TengYun~\cite{zhao2023parallel} & Traffic-related text and image & Generative & Prompt tuning & - & - & \tabincell{c}{Traffic prediction and control,\\ transportation planning} \\
%             \cline{2-8}
%             ~ & CityFM~\cite{balsebre2023city} & Spatial, visual, and textual geo-data & Contrastive	& -	& -	& -	& \tabincell{c}{Traffic speed inference,\\ building functionality classification}\\
%             \cline{2-8}
%             ~ & AllSpark~\cite{shao2023allspark} & Text, image, trajectory, graph, etc.	& Contrastive &	Prompt engineering & - & - & Spatiotemporal data analysis \\
%             \cline{2-8}
%             ~ & TrafficGPT~\cite{zhang2023trafficgpt} & Multimodal traffic data & - & Prompt engineering & - & General to traffic management & Traffic management \\
%             \cline{2-8}
%             ~ & GeoGPT~\cite{zhang2023geogpt} & Multimodal geospatial data	& -	& Prompt tuning	& -	& General to geospatial & \tabincell{c}{Autonomous geospatial data\\ collection, processing, and analysis} \\
%             \cline{2-8}
%             ~ & VELMA~\cite{schumann2023velma} & Street image, navigation instruction	& -	& Model fine-tuning	& LLM for image	& General to urban navigation & Autonomous street navigation \\
%             \cline{2-8}
%             ~ & UGI~\cite{xu2023urban} & \tabincell{c}{Urban textual, visual, knowledge graph,\\ human behavior data} & - & \tabincell{c}{Continue learning, \\ model fine-tuning} & - & General to urban environment & \tabincell{c}{Urban planning and simulation,\\ location recommendation} \\
%             \bottomrule[1pt]
%     \end{tabular}}
%     \label{table:summary}
% \end{table*}	

\section{Overview of Urban Foundation Models} \label{overview}
As illustrated in \figref{fig:taxonomy}, we introduce a data-centric taxonomy for the UFMs-related studies to shed light on the progress and efforts made in this field. Based on the urban data modalities, we categorize the existing works on UFMs into six classes: language-based models,  vision-based models, trajectory-based models, time series-based models, multimodal models, and others. Moreover, we further categorize the studies of each class into two subclasses based on their technical approaches: pretraining-based approaches and adaptation-based approaches.

\input{sections/language-based}

\input{sections/vision-based}

\input{sections/v2_trajectory-based}

\input{sections/time-series/v2_time-series-based}

\input{sections/multimodal-based}

\input{sections/others}

==> sections/time-series/merge_time-series-based.tex <==
\subsection{Time Series-based Approaches} 
Time series data are ubiquitous in urban scenarios attributed with diverse machine learning tasks such as traffic flow forecasting~\cite{gruver2023large}, air quality regression~\cite{cai2021time}, energy consumption forecasting~\cite{xue2023promptcast}, etc. In this section we review the recent advances in adopting foundation models for addressing time series data in urban scenarios. 
Generally, foundation model follows a 'pre-train, fine-tune' paradigm, which is associated with two key techniques: pre-training and adaptation, and we and respectively summarize existing research efforts for time series tasks. 
For time series data, we could denote it as $\mathbf{X}\in\mathbb{R}^{T\times N}$, where $T$ is the number of time steps and $N$ is the number of variables. For multivariate time series, a lot of works~\cite{shao2022pre} treat it as spatio-temporal data which explicitly incorporate dependencies between variables, and we denote it as $\mathbf{\mathcal{X}}\in\mathbb{R}^{T\times N\times C}$, where $C$ denotes the number of channels.

\subsubsection{Pre-training-based Approaches}
We respectively illustrate the pre-training methods for foundation models on time series and spatio-temporal data.

\textbf{\textsl{1) Time series-based approaches.}}
Specifically, we focus on two main-streams of foundation models: large language models (LLMs) and pre-trained foundation models (PFMs).

\textsl{(1) LLM-based approaches.}
Due to the success of large language models (LLMs) in natural language modeling, recently, a lot of research efforts have been devoted to directly using LLMs as foundation models for time series data. Lag-Llama~\cite{rasul2023lag} develops a foundation model with LLaMA as the backbone, which push the limits of zero-shot forecasting on unseen time series data. Lag-Llama is pre-trained over a large corpus of time series, and the inputs are enhanced by lag features to capture the seasonalities of various time series. Likewise, UniTime~\cite{liu2023unitime} aims at pre-training a unified model capable of generalizing across various unseen domains for time series forecasting, and further focuses on multi-source pre-training that learns from diverse domains via batch learning. To capture the variations of temporal characteristics over source domains, it empowers the input embedding with domain-specific text information as the manual prompt. Additionally, UniTime utilizes input and output padding to adapt varied data characteristics (\eg length of history and horizon), and designs input masking mechanism for imbalanced learning which is robust to varying convergence rates.

\textsl{(2) PFM-based approaches.}
Pre-trained foundation models (PFMs) are the large-scale pre-trained models that can be adapted to solve diverse downstream tasks~\cite{jin2023large}. Though LLMs also belong to PFMs, in this section PFMs refer to the foundation models pre-trained in time series domain primarily. Generally, recent studies of time series pre-training could be categorized into three types: supervised, contrastive and generative methods, to obtain appropriate representations for downstream novel tasks or novel data. 

Supervised approaches directly pre-train the model with ground truth information (\eg labels for classification, future values for forecasting). \cite{oreshkin2021meta} proposes a meta-learning framework for zero-shot univariate time series forecasting to tackle the cold start problem of existing time series models. In addition, many supervised pre-training methods~\cite{cai2021time,wilson2020multi,ragab2022self} for time series classification could be treated as unsupervised domain adaptation problem that has access to the data of target domain but without target ground truths. To name a few, CoDATS~\cite{wilson2020multi} proposes a domain classifier to discriminate features from source and target domains, and designs adversarial learning framework to train the feature extractor and domain classifier, to achieve domain-invariant representations. Also, the weak supervision information is utilized as constraints for parameter searching. Based on the adversarial framework, SLARDA~\cite{ragab2022self} use contrastive learning as regularization to capture the temporal pattern of time series. Further, to exploit the temporal dynamics property, it designs an autoregressive domain discriminator considering temporal dimension. SLARDA also proposes a teacher-based confident pseudo labeling for time series classification to adapt the fine-grained class distributions between domains. Except for adversarial learning, an alternative method for unsupervised domain adaptation is based on Maximum Mean Discrepancy (MMD)~\cite{ma2023survey}. For instance, to extract domain-invariant information from time series data, SASA~\cite{cai2021time} proposes sparse associative structure alignment as a regularization for source-target data, by minimizing MMD of the attention maps of multi-scale segments and multiple variables. Besides, SASA explicitly captures the dependencies of multiple variables for the time series representation.

Contrastive approaches aim to maximize the consistency between representations of time series objects with similar semantics (\ie positive pairs), while minimizing those with unrelated semantic information (\ie negative pairs). The key of contrastive-based time series pre-training lies in how to define the consistency of positive pairs that should be draw close to each other. Inspired by~\cite{ma2023survey}, we stress five types of consistency: subseries consistency~\cite{franceschi2019unsupervised} that assumes the representations of a reference time series should be similar to its subseries; transformation consistency~\cite{eldele2021time,woo2022cost} indicates that time series of distinct augmentation views should be consistent; temporal consistency~\cite{tonekaboni2021unsupervised} means that adjacent subseries in a time series should be similar; contextual consistency~\cite{yue2022ts2vec} assumes that the representations of the same timestamp in two augmented view of the same subseries should be consistent; consecutive consistency~\cite{ragab2022self,eldele2021time,zheng2023simts} implies that the two consecutive parts: history and horizon, of a time series should be consistent. To name a few, TS2Vec~\cite{yue2022ts2vec} aims to learn fine-grained representations for low-level tasks such as time series forecasting and anomaly detection,via contextual consistency-based contrastive learning without strong inductive bias. Besides, to distinguish the multi-scale contextual information with different granularities, TS2Vec propose temporal and instance contrast with different scales of negative pairs. Because the non-stationary property may hinder the generalization of time series representations, COST~\cite{woo2022cost} proposes trend-seasonal disentangled contrastive learning, including time domain contrast for trend feature and frequency domain contrast for seasonal feature. SimTS~\cite{zheng2023simts} is tailored for time series forecasting, via contrastive paradigm that predicts the future based on past time windows rather than discriminating between instances. Moreover, due to the challenge of negative sampling without bias, SimTS proposes a siamese architecture that needs no negative pairs.

Generative approaches usually use a masked reconstruction scheme that adds random masking to input time series and trains the model to recover the missing contents. TST~\cite{zerveas2021transformer} proposes an encoder-only Transformer architecture with elaborated masking strategy for reconstruction-based pre-training, adopted for downstream time series classification and regression. Further, SimMTM~\cite{dong2023simmtm} observes that directly masking a portion of time series will seriously ruin the temporal semantic variations. It regards masked reconstruction from a manifold perspective and proposes an idea of recovering the original time series from multiple masked series. To avoid the over-smoothing caused by naive averaging of multiple time series reconstruction, SimMTM proposes a similarity-based weighted aggregation. In addition, it proposes a contrastive constraint to lest trivial aggregation. Other masked reconstruction-based pre-training approaches focus on how to improve the model architecture for better time series analysis. PatchTST~\cite{nie2022time} proposes two intriguing techniques: patching and channel-independence, to reduce time and space complexity and enable a much longer look-back window for time series forecasting. TSMixer~\cite{ekambaram2023tsmixer} finds that the self-attention block in Transformer results in severe temporal information loss and thus utilizes lightweight MLP-Mixers without disturbing the temporal ordering of input. Besides, it proposes two reconciliation heads to capture inherent temporal hierarchical structure and cross-channel dependency. Additionally, PT-Tuning~\cite{liu2023pt} proposes a Cross-MAE architecture that conducts cross-attention for unmasked and masked time points.  

\textbf{\textsl{2) Spatio-temporal-based approaches.}}
In terms of how to capture the spatial information, some works~\cite{wang2018cross,yao2019learning,zhao2022st} model the spatial relations as a grid map with fixed sizes and employ convolution neural networks (CNNs) to encode the spatial pattern. For example, ST-GSP~\cite{zhao2022st} proposes a semantic flow encoder with ResNet as the backbone to capture the spatial dependencies. Besides, it devises a Transformer encoder with early-fusion paradigm to capture multi-scale temporal information for recosntruction-based pre-training and downstream urban flow prediction. However, grid-based spatial modelling is limited to local regular dependencies and fail to exploit the irregular and arbitrary variable-wise connections. 

In light of that, recent works~\cite{pan2019urban,jin2022selective,lu2022spatio,tang2022domain,liu2022contrastive} focus on graph-based spatial encoding and usually use Spatio-Temporal Graph Neural Networks (STGNNs) to extract the spatio-temporal information. For instance, due to the data scarcity, STGCL~\cite{liu2022contrastive} devises a contrastive pre-training framework for spatio-temporal forecasting. Specifically, for spatio-temporal contrastive learning, it proposes node- and graph-level contrast paradigms, four data augmentation techniques, and debiased negative filtering strategies from both temporal and spatial views. However, these methods adopt pre-defined graph structures which are noisy and biased, which negatively impact spatial information extraction~\cite{shao2022pre} or knowledge transfer~\cite{jin2023transferable}.

To address aforementioned drawbacks, STEP~\cite{shao2022pre} proposes a graph structure learning module in downstream forecasting. STGNNs only consider short-term historical time series, but the analysis of temporal and spatial patterns requires long-term historical time series data, thus STEP devises TSFormer for time series pretraining to capture long-time temporal pattern with segment-level representations. Further, TransGTR~\cite{jin2023transferable} focuses on how to learn the graph structure in a transferable way, which pre-trains a structure generator and transfers both the generator and the spatio-temporal forecasting module across cities. Specifically, TransGTR firstly extracts city-agnostic node features via knowledge distillation from the TSFormer~\cite{shao2022pre} pre-trained with long-term time series in data-rich source cities. Then it proposes a temporal decoupled regularization to learn transferable graph structures with discrepancy-based domain adaptation paradigm. 
Further, MC-STL~\cite{zhang2023mask} spots the spatio-temporal heterogeneity (\ie spatial correlation and region importance are time-varied), and proposes two pre-training strategies: 
spatial masked reconstruction which employs multi-head attention to dynamically calculate inter-region correlations, and temporal contrastive learning that uses a global-local cross-attention module, expecting global urban flow changes across periods to learn the importance changes of in regions across periods. 
Similar to TransGTR, TPB~\cite{liu2023cross} focuses on cross-city transfer learning for spatio-temporal forecasting. Specifically, to capture the traffic patterns in data-rich cities for transferring to data-scarce cities, TPB generates the representative traffic patterns via clustering, and conduct pattern aggregation during downstream forecasting. Additionally, it devises an attention-based graph reconstruction followed by STGNN for spatio-temporal pattern extraction. Note that during downstream forecasting, the modules in forecasting are not trained from scratch but initialized by meta-learning from multiple source cities.
GPT-ST~\cite{li2023gpt} observes that exisiting methods encounter the lack of customized representations of spatio-temporal patterns and insufficient consideration of different levels of spatial dependencies and pre-trains the spatio-temporal input encodings used for STGNN models. Concretely, it designs a hierarchical hypergraph structure to capture temporal and multi-level spatial dependencies from a global perspective, with a model parameter customization scheme.

\subsubsection{Adaptation-based Approaches}
The adaption methods are introduced respectively for foundation models on time series and spatio-temporal data.

\textbf{\textsl{1) Time series-based approaches.}}
Similarly, we investigate the adaptation methods for LLMs and PFMs respectively.

\textsl{(1) LLM-based approaches.}
Upon whether the LLMs are open-sourced or purely black-box, we categorize them into two types: embedding-visibal LLM (\eg GPT-2~\cite{radford2019language}, LLaMA~\cite{touvron2023llama}) and embedding-invisibal LLM (\eg ChatGPT\footnote{\url{https://openai.com/blog/chatgpt/}}, GPT-4\footnote{\url{https://openai.com/blog/gpt-4-api-general-availability}}), which follows~\cite{jin2023large}. For the former type of LLMs, we can fine-tune the model parameters in various tasks, while for the latter type, we could just inference by prompting with API calls.

As the lack of the large amount of data to train a foundation model from scratch for time series analysis, many works have contributed to how to fine-tune embedding-visibal LLMs for time series tasks. GPT(6)~\cite{zhou2023one1_nips} adopts pre-trained LLMs for diverse time series tasks. Specifically, it only fine-tunes small partial of parameters of LLM (\ie positional embedding and layer normalization layer) for efficiency, and uses linear probing and patching to align the time series to language modality. Incrementally, GPT(6)-adapter~\cite{zhou2023one2} designs frequency adapter, temporal adapter channel adapter for tuning, to strengthen the LLM-based time series analysis. To align the modalities of time series and language, LLM4TS~\cite{chang2023llm4ts} designs a two-satge fine-tuning process: firstly adopts autoregressive supervised fine-tuning for time series; then fine-tunes the pre-trained model for downstream time series forecasting. TEST~\cite{sun2023test} focuses on a data-centric framework that freeze all the parameters of pre-trained LLM and tries to elaborate the model inputs. Concretely, to make the LLM understand the time series embedding, TEST aligns it to the text representation space with text-prototype-based contrastive learning and add tunable prompts to help the LLM fit in the downstream forecasting and classification tasks. Further, TEMPO~\cite{cao2023tempo} highlights that LLMs fail to capture the time series characteristics such as the trend, seasonality and distribution shift. It adopts the trend-seasonality decomposition for the input time series and respectively pass them to the LLM for reasoning. Also, tunable prompts are added to conquer the distribution shift in diverse time series data. To align times series to natural language and unleash the potential of LLMs for time series forecasting, Time-LLM~\cite{jin2023time} reprogram time series into text prototype representations and add language-based prompts that describe the statistics of time series data.

However, some recent released LLMs hold striking capabilities but are closed-sourced (\ie embedding-invisibal). A plausible solution for adaptation is to transform the time series into natural language sentences as the prompts for API calls. PromptCast~\cite{xue2023promptcast} fisrtly proposes a novel prompt-based forecasting paradigm and release a large-scale dataset PISA constructed with template-based prompts for forecasting inputs and outputs. Further, LLMTime~\cite{gruver2023large} contends that LLMs can be used directly as zero-shot forecasters without any added text or prompt engineering, if the input time series data are carefully preprocessed.

To conclude, LLM-based adaptation approaches hinge on how to align the modalities of natural language and time series~\cite{jin2023time}. Existing works either leverage the neural networks to automatically achieve the alignment in a data-driven way (\eg input embedding~\cite{zhou2023one1_nips,zhou2023one2,chang2023llm4ts}, prompt tuning~\cite{sun2023test,cao2023tempo}), or explore the characteristics of time series (\eg input decomposition~\cite{cao2023tempo}), or explicitly utilize text information as the guidance (\eg reprogramming~\cite{sun2023test,jin2023time} and manual prompting~\cite{jin2023time,xue2023promptcast,gruver2023large}).

\textbf{(2) PFM-based approaches.} 
For PFMs on time series, most efforts are put into the pre-training design and few studies focus on advanced adaptation techniques. A fascinating work is V2S~\cite{yang2021voice2series} that leverages pre-trained acoustic model for time series classification, by input reprogramming and output label mapping. However, there exist few works that explore how to fine-tune time series PFMs. 

Recently, due to the emergence of prompt tuning methods in a wide range of fields (\eg natural language, vision and graph), prompting methods for time series also receive some attention. For example, PT-Tuning~\cite{liu2023pt} adds tunable prompts into masked tokens to achieve the consistency of task objectives between pre-training (\ie masked reconstruction) and adaptation (\ie forecasting). For time series classification, POND~\cite{wang2023prompt} further designs an instance-level prompt generator for adaptive prompting, besides the common prompt. Also, to capture diverse domain-specific information, POND proposes a meta-learning paradigm as well as elaborated contrastive constraints for prompt initialization.

\textbf{\textsl{2) Spatio-temporal-based approaches.}}
For the adaptation of foundation models on spatio-temporal data, recent works focus on the prompt tuning techniques. To name a few, PromptST~\cite{zhang2023promptst} adds tunable prompts to spatio-temporal data to efficiently fine-tuning and avoid catastrophic foregetting issue. MetePFL~\cite{chen2023prompt} and FedWing~\cite{chen2023spatial} focus on federated weather forecasting and use prompting techniques for personalized federated learning to reduce communication overheads and enhance privacy protection.

==> sections/time-series/spatio-temporal-based.tex <==
\subsection{Spatio-Temporal Raster Data-based Approach}
For multivariate time series, a lot of works treat it as spatio-temporal data which explicitly incorporate dependencies between variables~\cite{shao2022pre}, and we name it as spatio-temporal raster data. For spatio-temporal data, we could denote it as $\mathbf{X}\in\mathbb{R}^{T\times N\times C}$, where $T$ is the number of time steps, $N$ is the number of variables and $C$ denotes the number of channels. Due to difficulty of capturing both spatial and temporal patterns, there are limited works on LLM-based approach for spatio-temporal data. An advanced work is GATGPT~\cite{chen2023gatgpt} that use a graph attention module for spatial graph encoding and pass the embeddings to pre-trained GPT-2 model for downstream spatio-temporal imputation. Except for that, most works focus on PFM-based approaches equipped with well-designed pre-training and adaptation techniques.

\subsubsection{Pre-training-based Approaches}
In terms of how to capture the spatial information, some works~\cite{wang2018cross,yao2019learning,zhao2022st} model the spatial relations as a grid map with fixed sizes and employ convolution neural networks (CNNs) to encode the spatial pattern. For example, ST-GSP~\cite{zhao2022st} proposes a semantic flow encoder with ResNet as the backbone to capture the spatial dependencies. Besides, it devises a Transformer encoder with early-fusion paradigm to capture multi-scale temporal information for recosntruction-based pre-training and downstream urban flow prediction. However, grid-based spatial modelling is limited to local regular dependencies and fail to exploit the irregular and arbitrary variable-wise connections. 

In light of that, recent works~\cite{pan2019urban,jin2022selective,lu2022spatio,tang2022domain,liu2022contrastive} focus on graph-based spatial encoding and usually use Spatio-Temporal Graph Neural Networks (STGNNs) to extract the spatio-temporal information. For instance, due to the data scarcity, STGCL~\cite{liu2022contrastive} devises a contrastive pre-training framework for spatio-temporal forecasting. Specifically, for spatio-temporal contrastive learning, it proposes node- and graph-level contrast paradigms, four data augmentation techniques, and debiased negative filtering strategies from both temporal and spatial views. However, these methods adopt pre-defined graph structures which are noisy and biased, which negatively impact spatial information extraction~\cite{shao2022pre} or knowledge transfer~\cite{jin2023transferable}.

To address aforementioned drawbacks, STEP~\cite{shao2022pre} proposes a graph structure learning module in downstream forecasting. STGNNs only consider short-term historical time series, but the analysis of temporal and spatial patterns requires long-term historical time series data, thus STEP devises TSFormer for time series pretraining to capture long-time temporal pattern with segment-level representations. Further, TransGTR~\cite{jin2023transferable} focuses on how to learn the graph structure in a transferable way, which pre-trains a structure generator and transfers both the generator and the spatio-temporal forecasting module across cities. Specifically, TransGTR firstly extracts city-agnostic node features via knowledge distillation from the TSFormer~\cite{shao2022pre} pre-trained with long-term time series in data-rich source cities. Then it proposes a temporal decoupled regularization to learn transferable graph structures with discrepancy-based domain adaptation paradigm. 
Further, MC-STL~\cite{zhang2023mask} spots the spatio-temporal heterogeneity (\ie spatial correlation and region importance are time-varied), and proposes two pre-training strategies: 
spatial masked reconstruction which employs multi-head attention to dynamically calculate inter-region correlations, and temporal contrastive learning that uses a global-local cross-attention module, expecting global urban flow changes across periods to learn the importance changes of in regions across periods. 
Similar to TransGTR, TPB~\cite{liu2023cross} focuses on cross-city transfer learning for spatio-temporal forecasting. Specifically, to capture the traffic patterns in data-rich cities for transferring to data-scarce cities, TPB generates the representative traffic patterns via clustering, and conduct pattern aggregation during downstream forecasting. Additionally, it devises an attention-based graph reconstruction followed by STGNN for spatio-temporal pattern extraction. Note that during downstream forecasting, the modules in forecasting are not trained from scratch but initialized by meta-learning from multiple source cities.
GPT-ST~\cite{li2023gpt} observes that exisiting methods encounter the lack of customized representations of spatio-temporal patterns and insufficient consideration of different levels of spatial dependencies and pre-trains the spatio-temporal input encodings used for STGNN models. Concretely, it designs a hierarchical hypergraph structure to capture temporal and multi-level spatial dependencies from a global perspective, with a model parameter customization scheme.

\subsubsection{Adaptation-based Approaches} 
For the adaptation of foundation models on spatio-temporal data, recent works focus on the prompt tuning techniques. To name a few, PromptST~\cite{zhang2023promptst} adds tunable prompts to spatio-temporal data to efficiently fine-tuning and avoid catastrophic foregetting issue. MetePFL~\cite{chen2023prompt} and FedWing~\cite{chen2023spatial} focus on federated weather forecasting and use prompting techniques for personalized federated learning to reduce communication overheads and enhance privacy protection.

==> sections/time-series/time_series-based.tex <==
\subsection{Time Series-based Approaches} 
Time series data are ubiquitous in urban scenarios attributed with diverse machine learning tasks such as traffic flow forecasting~\cite{gruver2023large}, air quality regression~\cite{cai2021time}, energy consumption forecasting~\cite{xue2023promptcast}, etc. In this section we review the recent advances in adopting foundation models for addressing time series data in urban scenarios. For time series data, we could denote it as $\mathbf{X}\in\mathbb{R}^{T\times N}$, where $T$ is the number of time steps and $N$ is the number of variables. Generally, foundation model follows a 'pre-train, fine-tune' paradigm, which is associated with two key techniques: pre-training and adaptation, and we and respectively summarize existing research efforts for time series tasks. 

\subsubsection{Pre-training-based Approaches}
Specifically, we focus on two main-streams of foundation models: large language models (LLMs) and pre-trained foundation models (PFMs).

\textsl{1) LLM-based Approaches}
Due to the success of large language models (LLMs) in natural language modeling, recently, a lot of research efforts have been devoted to directly using LLMs as foundation models for time series data. Lag-Llama~\cite{rasul2023lag} develops a foundation model with LLaMA as the backbone, which push the limits of zero-shot forecasting on unseen time series data. Lag-Llama is pre-trained over a large corpus of time series, and the inputs are enhanced by lag features to capture the seasonalities of various time series. Likewise, UniTime~\cite{liu2023unitime} aims at pre-training a unified model capable of generalizing across various unseen domains for time series forecasting, and further focuses on multi-source pre-training that learns from diverse domains via batch learning. To capture the variations of temporal characteristics over source domains, it empowers the input embedding with domain-specific text information as the manual prompt. Additionally, UniTime utilizes input and output padding to adapt varied data characteristics (\eg length of history and horizon), and designs input masking mechanism for imbalanced learning which is robust to varying convergence rates.

\textsl{2) PFM-based Approaches}
Pre-trained foundation models (PFMs) are the large-scale pre-trained models that can be adapted to solve diverse downstream tasks~\cite{jin2023large}. Though LLMs also belong to PFMs, in this section PFMs refer to the foundation models pre-trained in time series domain primarily. Generally, recent studies of time series pre-training could be categorized into three types: supervised learning, contrastive learning and masked reconstruction, to obtain appropriate representations for downstream novel tasks or novel data. 

\textbf{(1) Supervised Learning.} Supervised approaches directly pre-train the model with ground truth information (\eg labels for classification, future values for forecasting). \cite{oreshkin2021meta} proposes a meta-learning framework for zero-shot univariate time series forecasting to tackle the cold start problem of existing time series models. In addition, many supervised pre-training methods~\cite{cai2021time,wilson2020multi,ragab2022self} for time series classification could be treated as unsupervised domain adaptation problem that has access to the data of target domain but without target ground truths. To name a few, CoDATS~\cite{wilson2020multi} proposes a domain classifier to discriminate features from source and target domains, and designs adversarial learning framework to train the feature extractor and domain classifier, to achieve domain-invariant representations. Also, the weak supervision information is utilized as constraints for parameter searching. Based on the adversarial framework, SLARDA~\cite{ragab2022self} use contrastive learning as regularization to capture the temporal pattern of time series. Further, to exploit the temporal dynamics property, it designs an autoregressive domain discriminator considering temporal dimension. SLARDA also proposes a teacher-based confident pseudo labeling for time series classification to adapt the fine-grained class distributions between domains. Except for adversarial learning, an alternative method for unsupervised domain adaptation is based on Maximum Mean Discrepancy (MMD)~\cite{ma2023survey}. For instance, to extract domain-invariant information from time series data, SASA~\cite{cai2021time} proposes sparse associative structure alignment as a regularization for source-target data, by minimizing MMD of the attention maps of multi-scale segments and multiple variables. Besides, SASA explicitly captures the dependencies of multiple variables for the time series representation.

\textbf{(2) Contrastive Learning.} Contrastive-based pre-training methods aim to maximize the consistency between representations of time series objects with similar semantics (\ie positive pairs), while minimizing those with unrelated semantic information (\ie negative pairs). The key of contrastive-based time series pre-training lies in how to define the consistency of positive pairs that should be draw close to each other. Inspired by~\cite{ma2023survey}, we stress five types of consistency: subseries consistency~\cite{franceschi2019unsupervised} that assumes the representations of a reference time series should be similar to its subseries; transformation consistency~\cite{eldele2021time,woo2022cost} indicates that time series of distinct augmentation views should be consistent; temporal consistency~\cite{tonekaboni2021unsupervised} means that adjacent subseries in a time series should be similar; contextual consistency~\cite{yue2022ts2vec} assumes that the representations of the same timestamp in two augmented view of the same subseries should be consistent; consecutive consistency~\cite{ragab2022self,eldele2021time,zheng2023simts} implies that the two consecutive parts: history and horizon, of a time series should be consistent. To name a few, TS2Vec~\cite{yue2022ts2vec} aims to learn fine-grained representations for low-level tasks such as time series forecasting and anomaly detection,via contextual consistency-based contrastive learning without strong inductive bias. Besides, to distinguish the multi-scale contextual information with different granularities, TS2Vec propose temporal and instance contrast with different scales of negative pairs. Because the non-stationary property may hinder the generalization of time series representations, COST~\cite{woo2022cost} proposes trend-seasonal disentangled contrastive learning, including time domain contrast for trend feature and frequency domain contrast for seasonal feature. SimTS~\cite{zheng2023simts} is tailored for time series forecasting, via contrastive paradigm that predicts the future based on past time windows rather than discriminating between instances. Moreover, due to the challenge of negative sampling without bias, SimTS proposes a siamese architecture that needs no negative pairs.

\textbf{(3) Masked Reconstruction.} Reconstruction-based pre-training approaches add random masking to input time series and train the model to recover the missing contents. TST~\cite{zerveas2021transformer} proposes an encoder-only Transformer architecture with elaborated masking strategy for reconstruction-based pre-training, adopted for downstream time series classification and regression. Further, SimMTM~\cite{dong2023simmtm} observes that directly masking a portion of time series will seriously ruin the temporal semantic variations. It regards masked reconstruction from a manifold perspective and proposes an idea of recovering the original time series from multiple masked series. To avoid the over-smoothing caused by naive averaging of multiple time series reconstruction, SimMTM proposes a similarity-based weighted aggregation. In addition, it proposes a contrastive constraint to lest trivial aggregation. Other masked reconstruction-based pre-training approaches focus on how to improve the model architecture for better time series analysis. PatchTST~\cite{nie2022time} proposes two intriguing techniques: patching and channel-independence, to reduce time and space complexity and enable a much longer look-back window for time series forecasting. TSMixer~\cite{ekambaram2023tsmixer} finds that the self-attention block in Transformer results in severe temporal information loss and thus utilizes lightweight MLP-Mixers without disturbing the temporal ordering of input. Besides, it proposes two reconciliation heads to capture inherent temporal hierarchical structure and cross-channel dependency. Additionally, PT-Tuning~\cite{liu2023pt} proposes a Cross-MAE architecture that conducts cross-attention for unmasked and masked time points.  



\subsubsection{Adaptation-based Approaches}
Similarly, we investigate the adaptation methods for LLMs and PFMs respectively.

\textsl{1) LLM-based Approaches.}
Upon whether the LLMs are open-sourced or purely black-box, we categorize them into two types: embedding-visibal LLM (\eg GPT-2~\cite{radford2019language}, LLaMA~\cite{touvron2023llama}) and embedding-invisibal LLM (\eg ChatGPT\footnote{\url{https://openai.com/blog/chatgpt/}}, GPT-4\footnote{\url{https://openai.com/blog/gpt-4-api-general-availability}}), which follows~\cite{jin2023large}. For the former type of LLMs, we can fine-tune the model parameters in various tasks, while for the latter type, we could just inference by prompting with API calls.

\textbf{(1) Embedding-visibal LLM.}
As the lack of the large amount of data to train a foundation model from scratch for time series analysis, many works have contributed to how to fine-tune pre-trained LLMs for time series tasks. GPT(6)~\cite{zhou2023one1_nips} adopts pre-trained LLMs for diverse time series tasks. Specifically, it only fine-tunes small partial of parameters of LLM (\ie positional embedding and layer normalization layer) for efficiency, and uses linear probing and patching to align the time series to language modality. Incrementally, GPT(6)-adapter~\cite{zhou2023one2} designs frequency adapter, temporal adapter channel adapter for tuning, to strengthen the LLM-based time series analysis. To align the modalities of time series and language, LLM4TS~\cite{chang2023llm4ts} designs a two-satge fine-tuning process: firstly adopts autoregressive supervised fine-tuning for time series; then fine-tunes the pre-trained model for downstream time series forecasting. TEST~\cite{sun2023test} focuses on a data-centric framework that freeze all the parameters of pre-trained LLM and tries to elaborate the model inputs. Concretely, to make the LLM understand the time series embedding, TEST aligns it to the text representation space with text-prototype-based contrastive learning and add tunable prompts to help the LLM fit in the downstream forecasting and classification tasks. Further, TEMPO~\cite{cao2023tempo} highlights that LLMs fail to capture the time series characteristics such as the trend, seasonality and distribution shift. It adopts the trend-seasonality decomposition for the input time series and respectively pass them to the LLM for reasoning. Also, tunable prompts are added to conquer the distribution shift in diverse time series data. To align times series to natural language and unleash the potential of LLMs for time series forecasting, Time-LLM~\cite{jin2023time} reprogram time series into text prototype representations and add language-based prompts that describe the statistics of time series data.

\textbf{(2) Embedding-invisibal LLM.} Some recent released LLMs hold striking capabilities but are closed-sourced. A plausible solution for adaptation is to transform the time series into natural language sentences as the prompts for API calls. PromptCast~\cite{xue2023promptcast} fisrtly proposes a novel prompt-based forecasting paradigm and release a large-scale dataset PISA constructed with template-based prompts for forecasting inputs and outputs. Further, LLMTime~\cite{gruver2023large} contends that LLMs can be used directly as zero-shot forecasters without any added text or prompt engineering, if the input time series data are carefully preprocessed.

To conclude, LLM-based adaptation approaches hinge on how to align the modalities of natural language and time series~\cite{jin2023time}. Existing works either leverage the neural networks to automatically achieve the alignment in a data-driven way (\eg input embedding~\cite{zhou2023one1_nips,zhou2023one2,chang2023llm4ts}, prompt tuning~\cite{sun2023test,cao2023tempo}), or explore the characteristics of time series (\eg input decomposition~\cite{cao2023tempo}), or explicitly utilize text information as the guidance (\eg reprogramming~\cite{sun2023test,jin2023time} and manual prompting~\cite{jin2023time,xue2023promptcast,gruver2023large}).

\textbf{2) PFM-based Approaches.} 
For PFMs on time series, most efforts are put into the pre-training design and few studies focus on advanced adaptation techniques. A fascinating work is V2S~\cite{yang2021voice2series} that leverages pre-trained acoustic model for time series classification, by input reprogramming and output label mapping. However, there exist few works that explore how to fine-tune time series PFMs. 

Recently, due to the emergence of prompt tuning methods in a wide range of fields (\eg natural language, vision and graph), prompting methods for time series also receive some attention. For example, PT-Tuning~\cite{liu2023pt} adds tunable prompts into masked tokens to achieve the consistency of task objectives between pre-training (\ie masked reconstruction) and adaptation (\ie forecasting). For time series classification, POND~\cite{wang2023prompt} further designs an instance-level prompt generator for adaptive prompting, besides the common prompt. Also, to capture diverse domain-specific information, POND proposes a meta-learning paradigm as well as elaborated contrastive constraints for prompt initialization.


==> sections/time-series/urban_compress_merge_time_series-based.tex <==
\subsection{Time Series-based Models} 
Time series data are ubiquitous in urban scenarios attributed with diverse machine learning tasks such as traffic forecasting~\cite{ning2023uukg}, air quality forecasting~\cite{cai2021time}, energy consumption prediction~\cite{xue2023promptcast}, etc. In this section we review the recent advances in adopting foundation models for addressing time series data in urban scenarios. 
Generally, foundation model follows a ``pre-train, fine-tune'' paradigm, which is associated with two key techniques: pre-training and adaptation.
% For time series data, we could denote it as $\mathbf{X}\in\mathbb{R}^{T\times N}$, where $T$ is the number of time steps and $N$ is the number of variables. For multivariate time series, a lot of works~\cite{shao2022pre} treat it as spatio-temporal data which explicitly incorporate dependencies between variables, and we denote it as $\mathbf{\mathcal{X}}\in\mathbb{R}^{T\times N\times C}$, where $C$ denotes the number of channels.

\subsubsection{Pretraining-based Approaches}
Pre-training is a critical concept in time series foundation models, which involves training a neural network on a large time series
dataset in a supervised or self-supervised manner. In pre-training, the foundation model learns to capture the intricate temporal patterns within the time series. 
In this section, we respectively illustrate the pre-training methods for foundation models on ordinary time series and spatial time series.

\subsec{Pre-training on ordinary time series.}
% Specifically, we focus on two main-streams of foundation models: large language models (LLMs) and pre-trained foundation models (PFMs).
% Pre-trained foundation models (PFMs) are the large-scale pre-trained models that can be adapted to solve diverse downstream tasks~\cite{jin2023large}. Though LLMs also belong to PFMs, in this section PFMs refer to the foundation models pre-trained in time series domain primarily. 
Generally, recent studies of time pre-training strategies for time series foundation models could be categorized into three types: supervised, contrastive and generative methods, to obtain appropriate representations for downstream novel tasks or novel data. 

Supervised approaches directly pre-train the model with ground truth information (\eg labels for classification, future values for forecasting). \cite{oreshkin2021meta} proposes a meta-learning framework for zero-shot univariate time series forecasting to tackle the cold start problem of existing models. In addition, many supervised pre-training methods~\cite{cai2021time,wilson2020multi,ragab2022self} for time series classification could be treated as unsupervised domain adaptation problem that has access to the data of target domain but without target ground truths. For example, CoDATS~\cite{wilson2020multi} proposes a domain classifier to discriminate features from source and target domains, and designs adversarial learning framework to train the feature extractor and domain classifier, to achieve domain-invariant representations. Also, the weak supervision information is utilized as constraints for parameter searching. Except for adversarial learning, an alternative method for unsupervised domain adaptation is based on Maximum Mean Discrepancy (MMD)~\cite{ma2023survey}. For instance, to extract domain-invariant information from time series data, SASA~\cite{cai2021time} proposes sparse associative structure alignment as a regularization for air quality data in source-target cities, by minimizing MMD of the attention maps of multi-scale segments and multiple variables. Besides, SASA explicitly captures the dependencies of multiple variables for the time series representation.

Contrastive approaches aim to maximize the consistency between representations of time series objects with similar semantics (\ie positive pairs), while minimizing those with unrelated semantic information (\ie negative pairs). The key of contrastive-based time series pre-training lies in how to define the consistency of positive pairs that should be draw close to each other. Inspired by~\cite{ma2023survey}, we stress five types of consistency: subseries consistency~\cite{franceschi2019unsupervised} that assumes the representations of a reference time series should be similar to its subseries; transformation consistency~\cite{eldele2021time,woo2022cost} indicates that time series of distinct augmentation views should be consistent; temporal consistency~\cite{tonekaboni2021unsupervised} means that adjacent subseries in a time series should be similar; contextual consistency~\cite{yue2022ts2vec} assumes that the representations of the same timestamp in two augmented view of the same subseries should be consistent; consecutive consistency~\cite{ragab2022self,eldele2021time,zheng2023simts} implies that the two consecutive parts: history and horizon, of a time series should be consistent. To name a few, TS2Vec~\cite{yue2022ts2vec} aims to learn fine-grained representations for low-level tasks such as time series forecasting and anomaly detection, via contextual consistency-based contrastive learning without strong inductive bias. Besides, to distinguish the multi-scale contextual information with different granularities, TS2Vec proposes temporal and instance contrast with different scales of negative pairs. 
Because the non-stationary property may hinder the generalization of weather and electricity time series representations, COST~\cite{woo2022cost} proposes trend-seasonal disentangled contrastive learning, including time domain contrast for trend feature and frequency domain contrast for seasonal feature. 
SimTS~\cite{zheng2023simts} is tailored for the forecasting tasks in time series domains such weather and electricity, via contrastive paradigm that predicts the future based on past time windows rather than discriminating between instances. Moreover, due to the challenge of negative sampling without bias, SimTS proposes a siamese architecture that needs no negative pairs.

Generative approaches usually use a masked reconstruction scheme that adds random masking to input time series and trains the model to recover the missing contents~\cite{zerveas2021transformer}. Further, SimMTM~\cite{dong2023simmtm} observes that in urban domains (\eg weather, electricity, traffic), directly masking a portion of time series will seriously ruin the temporal semantic variations. It regards masked reconstruction from a manifold perspective and proposes an idea of recovering the original time series from multiple masked series. To avoid the over-smoothing caused by naive averaging of multiple time series reconstruction, SimMTM proposes a similarity-based weighted aggregation. In addition, it proposes a contrastive constraint to lest trivial aggregation. Besides, many other masked reconstruction-based pre-training approaches~\cite{nie2022time,ekambaram2023tsmixer,liu2023pt} focus on how to improve the model architecture for better time series analysis.

Besides the foundation model architecture well designed for time series analysis, recently, some research efforts~\cite{rasul2023lag,liu2023unitime} have been devoted to directly using LLMs as foundation models for time series pre-training, since the success of LLMs in natural language modeling. Lag-Llama~\cite{rasul2023lag} develops a foundation model with LLaMA as the backbone, which push the limits of zero-shot forecasting on unseen traffic time series data. Lag-Llama is pre-trained over a large corpus of time series, and the inputs are enhanced by lag features to capture the seasonalities of various time series. Likewise, UniTime~\cite{liu2023unitime} aims at pre-training a unified model capable of generalizing across various unseen domains for time series forecasting, and further focuses on multi-source pre-training that learns from diverse domains via batch learning. To capture the variations of temporal characteristics over source domains (\eg weather, electricity), it empowers the input embedding with domain-specific text information as the manual prompt. Additionally, UniTime utilizes input and output padding to adapt varied data characteristics (\eg length of history and horizon), and designs input masking mechanism for imbalanced learning which is robust to varying convergence rates.

\subsec{Pre-training on spatial time series.}
Compared to the studies that are pre-training on ordinary time series, usually considering only the temporal dimension, the works about pre-training on spatial time series additionally incorporate the spatial dimension, explicitly involving the dependencies between variables. Specially, in urban scenarios, most related works also name it as spatio-temporal data.

In terms of how to capture the spatial information in city regions, some works~\cite{wang2018cross,yao2019learning,zhao2022st} model the spatial relations as a grid map with fixed sizes and employ convolution neural networks (CNNs) to encode the spatial pattern. For example, ST-GSP~\cite{zhao2022st} proposes a semantic flow encoder with ResNet as the backbone to capture the spatial dependencies. Besides, it devises a Transformer encoder with early-fusion paradigm to capture multi-scale temporal information for recosntruction-based pre-training and downstream urban flow prediction. However, grid-based spatial modelling is limited to local regular dependencies and fail to exploit the irregular and arbitrary variable-wise connections. 

In light of that, recent works~\cite{pan2019urban,jin2022selective,lu2022spatio,tang2022domain,liu2022contrastive} focus on graph-based spatial encoding and usually use Spatio-Temporal Graph Neural Networks (STGNNs) to extract the spatio-temporal information. For instance, due to the data scarcity, STGCL~\cite{liu2022contrastive} devises a contrastive pre-training framework for traffic forecasting. Specifically, for spatio-temporal contrastive learning, it proposes node- and graph-level contrast paradigms, four data augmentation techniques, and debiased negative filtering strategies from both temporal and spatial views. However, these methods adopt pre-defined graph structures which are noisy and biased, which negatively impact spatial information extraction~\cite{shao2022pre} or cross-city knowledge transfer~\cite{jin2023transferable}.

To address aforementioned drawbacks, STEP~\cite{shao2022pre} proposes a graph structure learning module in downstream forecasting. STGNNs only consider short-term historical time series, but the analysis of temporal and spatial patterns requires long-term historical time series data, thus STEP devises TSFormer for time series pretraining to capture long-time temporal pattern with segment-level representations. Further, TransGTR~\cite{jin2023transferable} focuses on how to learn the graph structure in a transferable way, which pre-trains a structure generator and transfers both the generator and the spatio-temporal forecasting module across cities. Specifically, TransGTR firstly extracts city-agnostic node features via knowledge distillation from the TSFormer~\cite{shao2022pre} pre-trained with long-term time series in data-rich source cities. Then it proposes a temporal decoupled regularization to learn transferable graph structures with discrepancy-based domain adaptation paradigm. 
Further, MC-STL~\cite{zhang2023mask} spots the spatio-temporal heterogeneity (\ie spatial correlation and region importance are time-varied), and proposes two pre-training strategies: 
spatial masked reconstruction which employs multi-head attention to dynamically calculate inter-region correlations, and temporal contrastive learning that uses a global-local cross-attention module, expecting global urban flow changes across periods to learn the importance changes of in regions across periods. 
Similar to TransGTR, TPB~\cite{liu2023cross} focuses on cross-city transfer learning for spatio-temporal forecasting. Specifically, to capture the traffic patterns in data-rich cities for transferring to data-scarce cities, TPB generates the representative traffic patterns via clustering, and conduct pattern aggregation during downstream forecasting. Additionally, it devises an attention-based graph reconstruction followed by STGNN for spatio-temporal pattern extraction. Note that during downstream forecasting, the modules in forecasting are not trained from scratch but initialized by meta-learning from multiple source cities.
GPT-ST~\cite{li2023gpt} observes that exisiting methods encounter the lack of customized representations of spatio-temporal patterns and insufficient consideration of different levels of spatial dependencies and pre-trains the spatio-temporal input encodings used for STGNN models. Concretely, it designs a hierarchical hypergraph structure to capture temporal and multi-level spatial dependencies from a global perspective, with a model parameter customization scheme.

\subsubsection{Adaptation-based Approaches}
Adaptation is also a pivotal technique for time series foundation models, which aims at tailoring the pre-trained foundation models (PFMs) to specific downstream time series tasks or data for performance enhancement.
Specifically, the adaption methods are introduced respectively for foundation models on ordinary time series and spatial time series.

\subsec{Adaptation on ordinary time series}
According to which modality is the foundation model pre-trained, we investigate how to adapt time series PFMs and how to adapt foundation models from other modalities (\eg language, speech).

\textsl{1) Adaptation from PFMs on time series.} 
For PFMs on time series, most efforts are put into the pre-training design and few studies focus on advanced fine-tuning techniques.
Recently, due to the emergence of prompt tuning methods in a wide range of fields (\eg natural language, vision and graph), prompting methods for time series also receive some attention. For example, PT-Tuning~\cite{liu2023pt} adds tunable prompts into masked tokens to achieve the consistency of task objectives between pre-training (\ie masked reconstruction) and adaptation (\ie forecasting) in urban time series data. For time series classification, POND~\cite{wang2023prompt} further designs an instance-level prompt generator for adaptive prompting, besides the common prompt. Also, to capture diverse domain-specific information, POND proposes a meta-learning paradigm as well as elaborated contrastive constraints for prompt initialization.

\textsl{2) Adaptation from PFMs on other modalities.}
As the lack of the large amount of data to train a foundation model from scratch for time series analysis, many works leverage the PFMs from other modalities for time series tasks. For instance, a fascinating work is V2S~\cite{yang2021voice2series} that leverages pre-trained acoustic model for time series classification, by input reprogramming and output label mapping. While most recent studies focus on how to adapt pre-trained LLMs for time series.

Upon whether the LLMs are open-sourced or purely black-box, we categorize them into two types: embedding-visibal LLM (\eg GPT-2~\cite{radford2019language}, LLaMA~\cite{touvron2023llama}) and embedding-invisibal LLM (\eg ChatGPT\footnote{\url{https://openai.com/blog/chatgpt/}}, GPT-4\footnote{\url{https://openai.com/blog/gpt-4-api-general-availability}}), which follows~\cite{jin2023large}. For the former type of LLMs, we can fine-tune the model parameters in various tasks, while for the latter type, we could just inference by prompting with API calls.

As the data scarcity of time series, many works have contributed to how to fine-tune embedding-visibal LLMs for time series tasks. GPT(6)~\cite{zhou2023one1_nips} adopts pre-trained LLMs for diverse time series tasks. Specifically, it only fine-tunes small partial of parameters of LLM (\ie positional embedding and layer normalization layer) for efficiency, and uses linear probing and patching to align the time series of various urban domains (weather, electricity, traffic) to language modality. Incrementally, GPT(6)-adapter~\cite{zhou2023one2} designs frequency adapter, temporal adapter channel adapter for tuning, to strengthen the LLM-based time series analysis. To align the modalities of time series and language, LLM4TS~\cite{chang2023llm4ts} designs a two-satge fine-tuning process: firstly adopts autoregressive supervised fine-tuning for time series; then fine-tunes the pre-trained model for downstream time series forecasting. TEST~\cite{sun2023test} focuses on a data-centric framework that freezes all the parameters of pre-trained LLM and tries to elaborate the model inputs. Concretely, to make the LLM understand the time series embedding, TEST aligns it to the text representation space with text-prototype-based contrastive learning and add tunable prompts to help the LLM fit in the downstream forecasting and classification tasks. Further, TEMPO~\cite{cao2023tempo} highlights that LLMs fail to capture the time series characteristics such as the trend, seasonality and distribution shift. It adopts the trend-seasonality decomposition for the input time series and respectively pass them to the LLM for reasoning. Also, tunable prompts are added to conquer the distribution shift in diverse time series data. To align times series to natural language and unleash the potential of LLMs for time series forecasting, Time-LLM~\cite{jin2023time} reprogram time series into text prototype representations and add language-based prompts that describe the statistics of time series data.

However, some recent released LLMs hold striking capabilities but are closed-sourced (\ie embedding-invisibal). A plausible solution for adaptation is to transform the time series into natural language sentences as the prompts for API calls. PromptCast~\cite{xue2023promptcast} fisrtly proposes a novel prompt-based forecasting paradigm and release a large-scale dataset PISA constructed with template-based prompts including weather temperature, electricity consumption and human mobility prediction tasks. Further, LLMTime~\cite{gruver2023large} contends that LLMs can be used directly as zero-shot forecasters without any added text or prompt engineering, if the input time series data are carefully preprocessed.

To conclude, LLM-based adaptation approaches hinge on how to align the modalities of natural language and time series~\cite{jin2023time}. Existing works either leverage the neural networks to automatically achieve the alignment in a data-driven way (\eg input embedding~\cite{zhou2023one1_nips,zhou2023one2,chang2023llm4ts}, prompt tuning~\cite{sun2023test,cao2023tempo}), or explore the characteristics of time series (\eg input decomposition~\cite{cao2023tempo}), or explicitly utilize text information as the guidance (\eg reprogramming~\cite{sun2023test,jin2023time} and manual prompting~\cite{jin2023time,xue2023promptcast,gruver2023large}).

\subsec{Adaptation on spatial time series.}
For the adaptation of foundation models on spatial time series, recent works focus on the prompt tuning techniques. To name a few, PromptST~\cite{zhang2023promptst} adds tunable prompts to spatio-temporal data to efficiently fine-tune the pre-trained traffic forecasting model and avoid catastrophic foregetting issue. MetePFL~\cite{chen2023prompt} and FedWing~\cite{chen2023spatial} focus on federated weather forecasting and use prompting techniques for personalized federated learning to reduce communication overheads and enhance privacy protection.


==> sections/time-series/v2_time-series-based.tex <==
\subsection{Time Series-based Models} 
Time series is the collection of observable records in an ordered manner, which represents the evolution of the variable states in the real world. 
In urban scenarios, time series data are ubiquitous due to the temporal characteristic of urban data, associated with diverse machine learning tasks such as traffic forecasting~\cite{ning2023uukg,zhang2020semi,liu2022practical}, air quality forecasting~\cite{han2022semi,han2023kill, han2023machine}, energy consumption prediction~\cite{xue2023promptcast}. 
Formally, we could denote a time series as $\mathbf{X}\in\mathbb{R}^{T\times N}$, where $T$ is the number of time steps and $N$ is the number of variables. For multivariate time series, some works~\cite{shao2022pre} treat it as spatio-temporal data which explicitly incorporate dependencies between variables, and we denote it as $\mathbf{\mathcal{X}}\in\mathbb{R}^{T\times N\times C}$, where $C$ denotes the number of channels.
In this section, we review the recent advances in adopting foundation models for handling time series data related to urban contexts,  classifying them as two primary categories: 1) unimodal approaches and 2) cross-modal transfer approaches.

\subsubsection{Unimodal Approaches} Unimodal foundation models comprise two pivotal techniques: pre-training and adaptation. Typically, they are pre-trained with large-scale data in the modality of time series, and then be adapted to specific downstream tasks or data.

\subsec{Pre-training.} Pre-training typically involves training deep neural networks on numerous large time series datasets in a supervised or self-supervised manner. In pre-training, the model learns to capture the intricate temporal patterns and inter-variable correlations within the data. This section respectively illustrates the pre-training methods of foundation models on ordinary time series and spatial-correlated time series.

\subsubsec{(1) Ordinary time series.} For ordinary time series, existing works focus on how to extract the temporal dependencies during pre-training and can be categorized into four types: supervised, generative, contrastive, and hybrid methods, according to the training schemes.

Supervised approaches directly pre-train the model with ground truth information (\eg labels for classification, future values for forecasting). 
Oreshkin et al.~\cite{oreshkin2021meta} proposes a meta-learning framework for zero-shot univariate time series forecasting to tackle the cold start problem of existing models. 
Drawn by the strong capacities of LLMs, Lag-Llama~\cite{rasul2023lag} develops a foundation model with LLaMA as the backbone, which pushes the limits of zero-shot forecasting on unseen traffic time series data. Specifically, Lag-Llama is pre-trained over a large corpus of time series forecasting data, and lag features enhance the inputs to capture the seasonalities of various time series. 
Due to the scarcity of real-world time series data, ForecastPFN~\cite{dooley2024forecastpfn} constructs a synthetic time series distribution via Prior-data Fitted Networks (PFNs) for pre-training, that could achieve remarkable zero-shot forecasting capabilities.
Beyond the one-generation time series forecasting schema, GPHT~\cite{liu2024generative} delves into the auto-regressive pre-training strategy similar to language modeling, which could sufficiently capture the temporal patterns within the predicted series and generalize to arbitrary horizon lengths. GPHT is also characterized by hierarchical Transformer blocks that learn multi-scale representations with coarse-to-fine patterns. 
To accommodate various time series tasks and data characteristics, Timer~\cite{liu2024timer} convert heterogeneous time series into a unified format. Similar to GPHT, Timer adopts the GPT-style training objective which predicts the next token.
Likewise, to harmonize diverse time series data with multiple resolutions (\ie the sampling rate), TTM~\cite{ekambaram2024ttms} proposes three enhancements based on TSMixer~\cite{ekambaram2023tsmixer}: adaptive patching, data augmentation via down-sampling and resolution prefix tuning, for pre-training a light-weight model via the forecasting pretext task.
Recently, TimesFM~\cite{dasdecoder} explores the question of how to build a time series foundation model with good zero-shot forecasting performances. This work builds a large time series corpus and designs a decoder-only model architecture, and strikingly achieves close to state-of-the-art zero-shot forecasting performance. Specifically, TimesFM uses Longer output patches for the better balance between accuracy and efficiency, and designs a novel patch masking mechanism to accommodate all possible context lengths.
In addition, many supervised pre-training methods~\cite{cai2021time,wilson2020multi,ragab2022self} for time series classification could be treated as unsupervised domain adaptation problem that has access to the data of the target domain but without target ground truths. 
For example, except for training the source-domain time series classifier, CoDATS~\cite{wilson2020multi} proposes a domain classifier to discriminate features from source and target domains, and designs an adversarial learning framework to train the feature extractor and domain classifier, to achieve domain-invariant representations. 
% Also, the weak supervision information is utilized as a constraint for parameter searching. 
Except for adversarial learning, an alternative method for unsupervised domain adaptation is based on Maximum Mean Discrepancy (MMD)~\cite{ma2023survey}. For instance, to extract domain-invariant information from time series data, SASA~\cite{cai2021time} proposes sparse associative structure alignment as a regularization for air quality data in source-target cities, by minimizing MMD of the attention maps of multi-scale segments and multiple variables. 
% Besides, SASA explicitly captures the dependencies of multiple variables for the time series representation.

Generative approaches usually use a masked reconstruction scheme that adds random masking to input time series and trains the model to recover the missing contents~\cite{zerveas2021transformer}. Further, SimMTM~\cite{dong2023simmtm} observes that in urban domains (\eg weather, electricity, traffic), directly masking a portion of time series will seriously ruin the temporal semantic variations. It regards masked reconstruction from a manifold perspective and proposes the idea of recovering the original time series from multiple masked series. 
% To avoid the over-smoothing caused by naive averaging of multiple time series reconstruction, SimMTM proposes a similarity-based weighted aggregation. In addition, it proposes a contrastive constraint to lest trivial aggregation. 
Besides, many other masked reconstruction-based pre-training approaches~\cite{nie2022time,ekambaram2023tsmixer,liu2023pt} focus on how to improve the model architecture for better time series analysis. 
For instance, PatchTST~\cite{nie2022time} proposes two intriguing techniques: patching and channel-independence, based on Transformer architecture, to reduce time and space complexity and enable a much longer look-back window for time series forecasting. TSMixer~\cite{ekambaram2023tsmixer} finds that the self-attention block in Transformer results in severe temporal information loss and thus utilizes lightweight MLP-Mixers without disturbing the temporal ordering of input. Besides, it proposes two reconciliation heads to capture inherent temporal hierarchical structure and cross-channel dependency. 
Additionally, PT-Tuning~\cite{liu2023pt} proposes a Cross-MAE architecture that conducts cross-attention for unmasked and masked time points. 
Lately, based on the decoupled auto-encoder architecture~\cite{cheng2023timemae}, HiMTM~\cite{zhao2024himtm} has devoted the pioneering efforts to integrating multi-scale temporal pattern extraction into masked time series reconstruction. Concretely, HiMTM segments time series to fine-to-coarse representations and reconstruct the masked parts at each hierarchical level.
Inspired by contrastive learning, TimSiam~\cite{dong2024timesiam} designs a novel reconstruction-based pre-training strategy, which models the correlation among distanced subseries beyond the current context thus can capture the global dynamics of the whole time series. Specifically, TimSiam firstly samples the distanced subseries within the whole series for the current subseries, and adopts Siamese networks to reconstruct the current series by the sampled subseries pairs.

Contrastive approaches aim to enhance the consistency between the representations of time series objects that share similar semantic meaning (i.e., positive pairs) and reduce that for those with disparate semantics (i.e., negative pairs).
The key to contrastive-based time series pre-training lies in how to define the consistency of positive pairs that should be drawing close to each other. Inspired by~\cite{ma2023survey}, we stress five types of consistency: subseries consistency~\cite{franceschi2019unsupervised} that assumes the representations of a reference time series should be similar to its subseries; transformation consistency~\cite{eldele2021time,woo2022cost} indicates that time series of distinct augmentation views should be consistent; temporal consistency~\cite{tonekaboni2021unsupervised} means that adjacent subseries in a time series should be similar; contextual consistency~\cite{yue2022ts2vec} assumes that the representations of the same timestamp in two augmented view of the same subseries should be consistent; consecutive consistency~\cite{ragab2022self,eldele2021time,zheng2023simts} implies that the two consecutive parts: history and horizon, of a time series should be consistent. To name a few, TS2Vec~\cite{yue2022ts2vec} aims to learn fine-grained representations for low-level tasks such as time series forecasting and anomaly detection, via contextual consistency-based contrastive learning without strong inductive bias. Besides, to distinguish the multi-scale contextual information with different granularities, TS2Vec proposes temporal and instance contrast with different scales of negative pairs. 
Because the non-stationary property may hinder the generalization of weather and electricity time series representations, COST~\cite{woo2022cost} proposes trend-seasonal disentangled contrastive learning, including time domain contrast for trend features and frequency domain contrast for seasonal features. 
SimTS~\cite{zheng2023simts} is tailored for the forecasting tasks in time series domains such as weather and electricity, via a contrastive paradigm that predicts the future based on past time windows within a series rather than discriminating between series instances. Moreover, due to the bias introduced by negative sampling, SimTS proposes a Siamese architecture with stop-gradient operation, that abolishes negative samples.

Hybrid approaches integrate the aforementioned training schemes for robust pre-training. For example, UniTime~\cite{liu2024unitime} aims at pre-training a unified model capable of generalizing across various unseen domains for time series forecasting, and further focuses on multi-source pre-training that learns from diverse domains via batch learning. To capture the variations of temporal characteristics over source domains (\eg weather, electricity), it empowers the input embedding with domain-specific text information as the manual prompt. Additionally, UniTime utilizes input and output padding to adapt varied data characteristics (\eg length of history and horizon), and designs input masking mechanism for imbalanced learning which is robust to varying convergence rates. Likewise, UniTS~\cite{gao2024units} architecture is tailored to accommodate the variability of temporal dynamics among multi-domain time series data. In addition, UniTS supports multi-task supervised training or unified masked reconstruction pre-training, and could be applied to diverse time series tasks empowered by the prompting framework.

In a summary, the four training schemes differ in how to construct the supervision signals. Due to the scarcity of labeled data in urban time series analysis, recently, generative and contrastive approaches have attracted increasing attention. 

\underline{\textsl{(2) Spatial-correlated time series.}} Beyond ordinary time series pre-training that considers only the temporal dimension, the studies on spatial-correlated time series additionally incorporate the spatial dimension, explicitly involving the dependencies between variables. In urban scenarios, many relevant literature~\cite{yuan2024unist,liu2022contrastive,shao2022pre}also names it as spatio-temporal data.

In terms of how to capture the spatial information in city regions, some works~\cite{wang2018cross,yao2019learning,zhao2022st} model the spatial relations as a grid map with fixed sizes and employ Convolution Neural Networks (CNNs) to encode the spatial pattern. For example, ST-GSP~\cite{zhao2022st} proposes a semantic flow encoder with ResNet as the backbone to capture the spatial dependencies. Besides, it devises a Transformer encoder with an early-fusion paradigm to capture multi-scale temporal information for reconstruction-based pre-training and downstream urban flow prediction. Lately, UniST~\cite{yuan2024unist} further proposes a universal foundation model for spatio-temporal prediction that could generalize diverse data formats and variations of data distributions. Concretely, UniST firstly patches and transform 3D data into 1D sequential data, and then applies four distinct masking techniques from both spatial and temporal perspectives for generative pre-training.
However, grid-based spatial modeling is limited to local regular dependencies and fails to exploit irregular and arbitrary variable-wise connections. 

In light of that, recent works~\cite{pan2019urban,jin2022selective,lu2022spatio,tang2022domain,liu2022contrastive} focus on graph-based spatial encoding and usually use Spatio-Temporal Graph Neural Networks (STGNNs) to extract the spatio-temporal information. For instance, due to data scarcity, STGCL~\cite{liu2022contrastive} devises a contrastive pre-training framework for traffic forecasting. Specifically, for spatiotemporal contrastive learning, it proposes node- and graph-level contrast paradigms, four data augmentation techniques, and debiased negative filtering strategies from both temporal and spatial views. However, these methods adopt pre-defined graph structures that may be noisy and biased, which negatively impact spatial information extraction~\cite{shao2022pre} or cross-city knowledge transfer~\cite{jin2023transferable}.

To address the aforementioned drawbacks, STEP~\cite{shao2022pre} proposes a graph structure learning module in downstream forecasting. STGNNs only consider short-term historical time series, but the analysis of temporal and spatial patterns requires long-term historical time series data, thus STEP devises TSFormer for time series pre-training to capture long-time temporal patterns with segment-level representations. Further, TransGTR~\cite{jin2023transferable} focuses on how to learn the graph structure in a transferable way, which pre-trains a structure generator and transfers both the generator and the spatiotemporal forecasting module across cities. Specifically, TransGTR firstly extracts city-agnostic node features via knowledge distillation from the TSFormer~\cite{shao2022pre} pre-trained with long-term time series in data-rich source cities. Then it proposes a temporal decoupled regularization to learn transferable graph structures with a discrepancy-based domain adaptation paradigm. 
    \zhaobite{Further, MC-STL~\cite{zhang2023mask} spots the spatio-temporal heterogeneity (\ie spatial correlation and region importance are time-varied), and proposes two pre-training strategies: 
    spatial masked reconstruction which employs multi-head attention to dynamically calculate inter-region correlations, and temporal contrastive learning that uses a global-local cross-attention module, expecting global urban flow changes across periods to learn the importance changes of in regions across periods. }
Further, MC-STL~\cite{zhang2023mask} spots the spatiotemporal heterogeneity (\ie spatial correlation and region importance are time-varied), and proposes two pre-training strategies. The first is spatial masked reconstruction, which utilizes a multi-head attention mechanism to dynamically estimate the inter-region correlations. The second is temporal contrastive learning, which leverages a global-local cross-attention block to understand the shifts in global urban flow over time and the corresponding changes in regional importance across different periods.
Similar to TransGTR, TPB~\cite{liu2023cross} focuses on cross-city transfer learning for spatio-temporal forecasting. Specifically, to capture the traffic patterns in data-rich cities for transferring to data-scarce cities, TPB generates the representative traffic patterns via clustering, and conducts pattern aggregation during downstream forecasting. Additionally, it devises an attention-based graph reconstruction followed by STGNN for spatio-temporal pattern extraction. Note that during downstream forecasting, the modules are not trained from scratch but initialized by meta-learning from multiple source cities.
GPT-ST~\cite{li2023gpt} observes that existing methods encounter the lack of customized representations of spatio-temporal patterns and insufficient consideration of different levels of spatial dependencies and pre-trains the spatio-temporal input encodings used for STGNN models. Concretely, it designs a hierarchical hypergraph structure to capture temporal and multi-level spatial dependencies from a global perspective, with a model parameter customization scheme.

\subsec{Adaptation.} Adaptation for time series foundation models aims to tailor the pre-trained foundation models to new time series tasks or data for downstream performance enhancement. 
In the area of time series foundation models, despite most research efforts being the design of pre-training, advanced fine-tuning strategies receive little attention.
Alternatively, due to the emergence of prompt tuning methods in data modalities like natural language, vision, and graph~\cite{sun2023all}, prompting methods for time series also receive growing attention. For example, PT-Tuning~\cite{liu2023pt} adds tunable prompts into masked tokens to achieve the consistency of task objectives between pre-training (\ie masked reconstruction) and adaptation (\ie forecasting) in urban time series data. For time series classification, POND~\cite{wang2023prompt} further designs an instance-level prompt generator for adaptive prompting, besides the common prompt. Also, to capture diverse domain-specific information, POND proposes a meta-learning paradigm as well as elaborated contrastive constraints for prompt initialization.
Moreover, there have been some studies on prompt tuning for spatial-correlated time series tasks. To name a few, PromptST~\cite{zhang2023promptst} adds tunable prompts to spatiotemporal data to efficiently fine-tune the pre-trained traffic forecasting model and avoid catastrophic forgetting issue. STGP~\cite{hu2024prompt} designs a tow-stage prompting pipeline for spatio-temporal graph learning, which enables the prompts to curate domain knowledge and task-specific properties.
UniST~\cite{yuan2024unist} proposes a prior knowledge-guided prompt network to automatically learn the specific prompts for each case. Specifically, UniST firstly learns a spatial and a temporal memory pool with key-value structured parameters, and then it learns representations for each input with four aspects of spatio-temporal domain knowledge. The knowledge-guided prompts are extracted by quering the prompt memory pools with input representations.
MetePFL~\cite{chen2023prompt} and FedWing~\cite{chen2023spatial} focus on federated weather forecasting and use prompting techniques for personalized federated learning to reduce communication overheads and enhance privacy protection.

In a summary, existing unimodal approaches have put some preliminary efforts into building a universal time series foundation model. Diverse pre-training techniques have contributed to the development of time series foundation model. Some recent works have also paid the attention on more challenging questions, including how to enhance the universality of foundation model~\cite{yuan2024unist,liu2024unitime}, how to prompt the pre-trained model~\cite{hu2024prompt,yuan2024unist}, and how to improve the zero-shot capabilities~\cite{dasdecoder}. However, due to the intricate characteristics of spatiotemporal data, the foundation model tailored for urban scenarios is situated in the nascent state.

\subsubsection{Cross-modal transfer approaches} Due to insufficient time series data to train a foundation model from scratch, cross-modal transfer approaches directly adopt the foundation models pre-trained on other modalities and aim to transfer the modality-sharing knowledge to time series tasks. For instance, a fascinating work is V2S~\cite{yang2021voice2series} that leverages a pre-trained acoustic model for time series classification, by input reprogramming and output label mapping. 

\zhaobite{
    Recently, most cross-modal studies have focused on how to adapt pre-trained LLMs for time series to leverage the remarkable abilities of LLMs sufficiently. Upon whether the LLMs are open-sourced or purely black-box, we categorize them into two types: embedding-invisible LLM (\eg ChatGPT\footnote{\url{https://openai.com/blog/chatgpt/}}, GPT-4\footnote{\url{https://openai.com/blog/gpt-4-api-general-availability}}) and embedding-visible LLM (\eg GPT-2~\cite{radford2019language}, LLaMA~\cite{touvron2023llama}), which follows~\cite{jin2023large}. For the former type of LLMs, we could just infer by prompting with API calls, while for the latter type, we can fine-tune the model parameters or reprogram the time series inputs in various tasks.
}
Recently, most cross-modal studies have focused on adapting pre-trained LLMs for time series to sufficiently leverage the remarkable abilities of LLMs~\cite{jin2023large,jin2024position}. Upon whether the LLMs are open-sourced or purely black-box, we categorize them into two types: embedding-invisible LLM (\eg ChatGPT, GPT-4\footnote{\url{https://openai.com/blog/gpt-4-api-general-availability}}) and embedding-visible LLM (\eg GPT-2~\cite{radford2019language}, LLaMA~\cite{touvron2023llama}), which follows~\cite{jin2023large}. For the former type of LLMs, we could just infer by prompting with API calls, while for the latter type, we can fine-tune the model parameters or reprogram the time series inputs in various tasks.

\subsec{Prompt engineering.} Some recently released LLMs hold striking capabilities but are closed-sourced (\ie embedding-invisible). A plausible solution for adaptation is to transform the time series into natural language sentences as the prompts for API calls. PromptCast~\cite{xue2023promptcast} fisrtly proposes a novel prompt-based forecasting paradigm and releases a large-scale dataset PISA constructed with template-based prompts including weather temperature, electricity consumption and human mobility prediction tasks. Further, LLMTime~\cite{gruver2023large} contends that LLMs can be used directly as zero-shot forecasters without any added text or prompt engineering, if the input time series data are carefully preprocessed.

\subsec{Model fine-tuning.} Beyond prompting the generalist LLM, many works have contributed to fine-tuning embedding-visible LLMs for time series tasks. GPT(6)~\cite{zhou2023one1_nips} adopts pre-trained LLMs for diverse time series tasks. Specifically, it only fine-tunes a small part of the parameters of LLM (\ie positional embedding and layer normalization layer) for efficiency, and uses linear probing and patching to align the time series of various urban domains (weather, electricity, traffic) to language modality. Incrementally, GPT(6)-adapter~\cite{zhou2023one2} designs frequency adapter, temporal adapter, and channel adapter for tuning, to strengthen the LLM-based time series analysis. To align the modalities of time series and language, LLM4TS~\cite{chang2023llm4ts} design a two-stage fine-tuning process: firstly adopts auto-regressive supervised fine-tuning for time series; then fine-tunes the pre-trained model for downstream time series forecasting. Further, TEMPO~\cite{cao2023tempo} highlights that LLMs fail to capture the time series characteristics such as the trend, seasonality and distribution shift. It adopts the trend-seasonality decomposition for the input time series and respectively passes them to the LLM for reasoning. Also, tunable prompts are added to conquer the distribution shift in diverse time series data. To tackle time series with diverse context lengths, AutoTimes~\cite{liu2024autotimes} proposes an auto-regressive LLM-based forecasting approach, and adopts next token prediction as the training objective which is consistent with the LLM acquisition. Besides, AutoTimes designs token-wise prompting technique that utilizes the LLM generate the prompts indicating timestamp information.

To adapt the LLM for spatial-correlated time series, GATGPT~\cite{chen2023gatgpt} uses a graph attention module for spatial graph encoding and passes the spatio-temporal embeddings to the pre-trained GPT-2 model for downstream spatio-temporal imputation. TPLLM~\cite{ren2024tpllm} adopts 1-D convolutional neural networks and graph convolutional networks to enable LLMs to understand spatio-temporal patterns in traffic data.
Additionally, STG-LLM~\cite{liu2024can} proposes a spatio-temporal tokenizer to transform spatio-temporal data into tokens and an adapter architecture for efficient adaptation, which facilitate the understanding of pre-trained LLMs. Similarly, ST-LLM~\cite{liu2024spatial} treats the time steps at each spatial location as tokens, and fuse various spatial and temporal prior information into input embedding to facilitate traffic prediction. 

\subsec{Model reprogramming.} To explicitly align times series to natural language,  model reprogramming is an effective way that neither edits the time series inputs directly nor fine-tunes the pre-trained LLM. For example, TEST~\cite{sun2023test} focuses on a data-centric framework that freezes all the parameters of pre-trained LLM and tries to elaborate the model inputs. Concretely, to make the LLM understand the time series embedding, TEST aligns it to the text representation space with text-prototype-based contrastive learning and adds tunable prompts to help the LLM fit in the downstream forecasting and classification tasks. 
To unleash the potential of LLMs for time series forecasting, Time-LLM~\cite{jin2024time} reprogram time series into text prototype representations and add language-based prompts that describe the statistics of time series data. To avoid the large and dense reprogramming space, Time-LLM only maintains a small collection of the vocabulary by linearly probing the pretrained word embeddings.
To enhance the reprogramming framework for spatio-temporal data, RePST~\cite{wang2024empowering} decouples the spatio-temporal data in the frequency space to capture intricate spatio-temporal dependencies. Also RePST discretely samples word embeddings from the whole vocabulary to avoid semantic mixing and enhance the expressivity of text prototypes for spatio-temporal data.
To align the spatio-temporal dependencies with the comprehension space of LLMs, UrbanGPT~\cite{li2024urbangpt} proposes a spatio-temporal instruction tuning paradigm which aligns spatio-temporal data with the knowledge space of LLMs.


% \subsec{Summary.} 
% To conclude, LLM-based adaptation approaches hinge on how to align the modalities of natural language and time series~\cite{jin2024time}. Existing works either leverage the neural networks to automatically achieve the alignment in a data-driven way (\eg linear probing~\cite{zhou2023one1_nips,zhou2023one2,chang2023llm4ts,chen2023gatgpt}, prompt tuning~\cite{sun2023test,cao2023tempo}), explore the characteristics of time series (\eg trend-seasonal decomposition~\cite{cao2023tempo}, spatial correlation encoding~\cite{chen2023gatgpt}), or explicitly utilize text information as the guidance (\eg reprogramming~\cite{sun2023test,jin2024time} and manual prompting~\cite{jin2024time,xue2023promptcast,gruver2023large}).

To conclude, the cross-modal transfer approaches, especially LLM-based adaptation approaches, hinge on how to make LLMs comprehend time series data, hence we can unleash the significant reasoning ability of LLMs. 
The three adaptation techniques above have showed remarkable capability to align the modalities of natural language and time series, and could be adopted to diverging tasks and data domains. 
Specifically, prompt engineering approaches~\cite{xue2023promptcast, gruver2023large} are highly portable and flexible to use without needs to delve into the complicated model, and they have the potential to tackle various domains of time series data and diverging tasks. However, the performance is not guaranteed since the great gap between time series and natural language, and it is tricky to explore manual prompts in a heuristic manner to unleash the abilities of LLMs for urban time series analysis. 
Therefore, most recent works focus on model fine-tuning to align the time series with the knowledge space of LLMs, and put efforts on the parameter-efficient tuning~\cite{zhou2023one1_nips} and how to capture the intricate patterns of time series~\cite{cao2023tempo,liu2024spatial} and language data~\cite{chang2023llm4ts,liu2024autotimes}. 
Furthermore, model reprogramming provides a more interpretable way for cross-modal transfer, which aims at reprogram time series into prototypical textual tokens that facilitates the comprehension of LLMs~\cite{jin2024time}. However, most of these works are limited to a very high-level understanding of LLM for time series data.

\subsubsection{Outlook and Future Opportunities} In this section, we will discuss the current limitations and potential research opportunities of time series-based UFMs.

\subsec{Universality of time series-based UFMs.} 
Most of existing time series-based UFMs are limited into specific data domains, data formats or downstream tasks, which disobeys the universal property of foundation models. Based on these preliminary progress, there have been some works~\cite{liu2024timer,ekambaram2024ttms,gao2024units,yuan2024unist} that focus on the universality of time series-based UFMs. However, there still lack a generally accepted universal UFM that could be applied to various domains and heterogeneous formats of data and diverse downstream tasks.

\subsec{Theoretical analysis of LLMs.}
Recently, some studies have drawn inspirations from the success of LLMs to refine the time series UFM, such as adopting the auto-regressive pre-training strategy that is consistent with language modeling~\cite{liu2024generative,liu2024timer,chang2023llm4ts,liu2024autotimes}. However, how LLMs make effective predictions on urban time series domain is scarcely discussed. More studies should incorporate the understanding of LLMs as inspirations to reform current time series UFMs, by devising a urban-specific model architecture for unimodal pre-training, or a urban-aware alignment technique for cross-model transfer.

\subsec{Prior knowledge fusion for urban time series.}
There have been some works integrating the prior knowledge of time series into either pre-training or adaptation, such as multi-scale temporal pattern~\cite{liu2024generative,zhao2024himtm}, trend-seasonal property~\cite{cao2023tempo,dooley2024forecastpfn} and spatial correlations~\cite{liu2024spatial}. However, there still exist rich prior characteristics of urban time series in both temporal and spatial, local and global perspectives, which require future works to explore.

% \subsubsection{Outlook and Future Opportunities} In this section, we will discuss the current limitations and potential research opportunities of time series-based UFMs.

% \subsec{Universality of time series-based UFMs.} 
% Most of existing time series-based UFMs are limited into specific data domains, data formats or downstream tasks, which disobeys the universal property of foundation models. Based on these preliminary progress, there have been some works~\cite{liu2024timer,ekambaram2024ttms,gao2024units,yuan2024unist} that focus on the universality of time series-based UFMs. However, there still lack a generally accepted universal UFM that could be applied to various domains and heterogeneous formats of data and diverse downstream tasks.

% \subsec{Theoretical analysis of LLMs.}
% Recently, some studies have drawn inspirations from the success of LLMs to refine the time series UFM, such as adopting the auto-regressive pre-training strategy that is consistent with language modeling~\cite{liu2024generative,liu2024timer,chang2023llm4ts,liu2024autotimes}. However, the effectiveness of LLMs is scarcely discussed among existing works on time series UFMs, and more studies should incorporate the understanding of LLMs as inspirations to reform current time series UFMs.

% \subsec{Prior knowledge fusion for urban time series.}
% There have been some works integrating the prior knowledge of time series into either pre-training or adaptation, such as multi-scale temporal pattern~\cite{liu2024generative,zhao2024himtm}, trend-seasonal property~\cite{cao2023tempo,dooley2024forecastpfn} and spatial correlations~\cite{liu2024spatial}. However, there still exist rich prior characteristics of urban time series in both temporal and spatial, local and global perspectives, which require future works to explore.

% \subsec{Spatio-temporal UFMs.}
% Due to the complicated patterns of spatio-temporal data, the study of UFMs of spatial-correlated time series has lagged behind. For instance, the prompt engineering works for spatial-correlated time series are absent. Therefore more research efforts should be devoted to the pre-processing of spatio-temporal data and how to make LLMs comprehend the coupled spatio-temporal correlations.


==> sections/time-series/v3_time-series-based.tex <==
\subsection{Time Series-based Models} 
Time series is the collection of observable records in an ordered manner, which represents the evolution of the variable states in the real world. 
In urban scenarios, time series data are ubiquitous due to the temporal characteristic of urban data, associated with diverse machine learning tasks such as traffic forecasting~\cite{lyu2024autostf,zhang2020semi,liu2022practical}, air quality forecasting~\cite{han2022semi,han2023kill, han2023machine}, energy consumption prediction~\cite{xue2023promptcast}. 
Formally, we could denote a time series as $\mathbf{X}\in\mathbb{R}^{T\times N}$, where $T$ is the number of time steps and $N$ is the number of variables. For multivariate time series, some works~\cite{shao2022pre} treat it as spatio-temporal data which explicitly incorporate dependencies between variables, and we denote it as $\mathbf{\mathcal{X}}\in\mathbb{R}^{T\times N\times C}$, where $C$ denotes the number of channels.
In this section, we review the recent advances in adopting foundation models for handling time series data related to urban contexts,  classifying them as two primary categories: 1) unimodal approaches and 2) cross-modal transfer approaches.

\subsubsection{Unimodal Approaches} Unimodal foundation models comprise two pivotal techniques: pre-training and adaptation. Typically, they are pre-trained with large-scale data in the modality of time series, and then be adapted to specific downstream tasks or data.

\subsec{Pre-training.} Pre-training typically involves training deep neural networks on numerous large time series datasets in a supervised or self-supervised manner. In pre-training, the model learns to capture the intricate temporal patterns and inter-variable correlations within the data. This section respectively illustrates the pre-training methods of foundation models on ordinary time series and spatial-correlated time series.

\subsubsec{(1) Ordinary time series.} For ordinary time series, existing works focus on how to extract the temporal dependencies during pre-training and can be categorized into four types: supervised, generative, contrastive, and hybrid methods, according to the training schemes.

Supervised approaches~\cite{oreshkin2021meta,rasul2023lag,dooley2024forecastpfn,liu2024generative,liu2024timer,ekambaram2024ttms,dasdecoder} directly pre-train the model with ground truth information (\eg future values for forecasting, labels for classification). 
To name a few, GPHT~\cite{liu2024generative} delves into the auto-regressive pre-training strategy similar to language modeling, which could sufficiently capture the temporal patterns within the predicted series and generalize to arbitrary horizon lengths.
Recently, TimesFM~\cite{dasdecoder} explores the question of how to build a time series foundation model with good zero-shot forecasting performances, which builds a large time series corpus and designs a decoder-only model architecture.
Opencity~\cite{li2024opencity} crafts a versatile, resilient and adaptive foundation model for traffic prediction, which handles the spatiotemporal heterogeneity.

Generative approaches usually use a masked reconstruction scheme that adds random masking to input time series and trains the model to recover the missing contents~\cite{zerveas2021transformer}. 
For instance, SimMTM~\cite{dong2024simmtm} observes that in urban domains (\eg weather, electricity, traffic), directly masking a portion of time series will seriously ruin the temporal semantic variations. It regards masked reconstruction from a manifold perspective and proposes the idea of recovering the original time series from multiple masked series. 
Besides, many other masked reconstruction-based pre-training approaches~\cite{nie2023time,ekambaram2023tsmixer,liu2023pt} focus on how to improve the model architecture for better time series analysis. 
Lately, based on the decoupled auto-encoder architecture~\cite{cheng2023timemae}, HiMTM~\cite{zhao2024himtm} has devoted the pioneering efforts to integrating multi-scale temporal pattern extraction into masked time series reconstruction. 
Inspired by contrastive learning, TimSiam~\cite{dong2024timesiam} designs a novel reconstruction-based pre-training strategy, which models the correlation among distanced subseries beyond the current context thus can capture the global dynamics of the whole time series. 

Contrastive approaches aim to enhance the consistency between the representations of time series objects that share similar semantic meaning (i.e., positive pairs) and reduce that for those with disparate semantics (i.e., negative pairs).
The key to contrastive-based time series pre-training lies in how to define the consistency of positive pairs that should be drawing close to each other. Inspired by~\cite{ma2023survey}, we stress five types of consistency: subseries consistency~\cite{franceschi2019unsupervised} that assumes the representations of a reference time series should be similar to its subseries; transformation consistency~\cite{eldele2021time,woo2022cost} indicates that time series of distinct augmentation views should be consistent; temporal consistency~\cite{tonekaboni2021unsupervised} means that adjacent subseries in a time series should be similar; contextual consistency~\cite{yue2022ts2vec} assumes that the representations of the same timestamp in two augmented view of the same subseries should be consistent; consecutive consistency~\cite{ragab2022self,eldele2021time,zheng2023simts} implies that the two consecutive parts: history and horizon, of a time series should be consistent. 

Hybrid approaches~\cite{liu2024unitime,gao2024units} integrate the aforementioned training schemes for robust pre-training. For example, UniTime~\cite{liu2024unitime} aims at pre-training a unified model capable of generalizing across various unseen domains for time series forecasting, and further focuses on multi-source pre-training that learns from diverse domains via batch learning. To capture the variations of temporal characteristics over source domains (\eg weather, electricity), it empowers the input embedding with domain-specific text information as the manual prompt. Additionally, UniTime utilizes input and output padding to adapt varied data characteristics (\eg length of history and horizon), and designs input masking mechanism for imbalanced learning which is robust to varying convergence rates. Likewise, UniTS~\cite{gao2024units} architecture is tailored to accommodate the variability of temporal dynamics among multi-domain time series data. In addition, UniTS supports multi-task supervised training or unified masked reconstruction pre-training, and could be applied to diverse time series tasks empowered by the prompting framework.

In a summary, the four training schemes differ in how to construct the supervision signals. Due to the scarcity of labeled data in urban time series analysis, recently, generative and contrastive approaches have attracted increasing attention. 

\underline{\textsl{(2) Spatial-correlated time series.}} Beyond ordinary time series pre-training that considers only the temporal dimension, the studies on spatial-correlated time series additionally incorporate the spatial dimension, explicitly involving the dependencies between variables. In urban scenarios, many relevant literature~\cite{yuan2024unist,liu2022contrastive,shao2022pre}also names it as spatio-temporal data.

In terms of how to capture the spatial information in city regions, some works~\cite{wang2018cross,yao2019learning,zhao2022st} model the spatial relations as a grid map with fixed sizes and employ Convolution Neural Networks (CNNs) to encode the spatial pattern. For example, ST-GSP~\cite{zhao2022st} proposes a semantic flow encoder with ResNet as the backbone to capture the spatial dependencies. Besides, it devises a Transformer encoder with an early-fusion paradigm to capture multi-scale temporal information for reconstruction-based pre-training and downstream urban flow prediction. Lately, UniST~\cite{yuan2024unist} further proposes a universal foundation model for spatio-temporal prediction that could generalize diverse data formats and variations of data distributions. Concretely, UniST firstly patches and transform 3D data into 1D sequential data, and then applies four distinct masking techniques from both spatial and temporal perspectives for generative pre-training.
However, grid-based spatial modeling is limited to local regular dependencies and fails to exploit irregular and arbitrary variable-wise connections. 

In light of that, recent works~\cite{pan2019urban,jin2022selective,lu2022spatio,tang2022domain,liu2022contrastive} focus on graph-based spatial encoding and usually use Spatio-Temporal Graph Neural Networks (STGNNs) to extract the spatio-temporal information. For instance, due to data scarcity, STGCL~\cite{liu2022contrastive} devises a contrastive pre-training framework for traffic forecasting. Specifically, for spatiotemporal contrastive learning, it proposes node- and graph-level contrast paradigms, four data augmentation techniques, and debiased negative filtering strategies from both temporal and spatial views. However, these methods adopt pre-defined graph structures that may be noisy and biased, which negatively impact spatial information extraction~\cite{shao2022pre} or cross-city knowledge transfer~\cite{jin2023transferable}.

To address the aforementioned drawbacks, STEP~\cite{shao2022pre} proposes a graph structure learning module in downstream forecasting. STGNNs only consider short-term historical time series, but the analysis of temporal and spatial patterns requires long-term historical time series data, thus STEP devises TSFormer for time series pre-training to capture long-time temporal patterns with segment-level representations. 
Further, TransGTR~\cite{jin2023transferable} focuses on how to learn the graph structure in a transferable way, which pre-trains a structure generator and transfers both the generator and the spatiotemporal forecasting module across cities. 
Further, MC-STL~\cite{zhang2023mask} spots the spatiotemporal heterogeneity (\ie spatial correlation and region importance are time-varied), and proposes spatial and temporal pre-training strategies respectively. 
Similar to TransGTR, TPB~\cite{liu2023cross} focuses on cross-city transfer learning for spatio-temporal forecasting. Specifically, to capture the traffic patterns in data-rich cities for transferring to data-scarce cities, TPB generates the representative traffic patterns via clustering, and conducts pattern aggregation during downstream forecasting. Additionally, it devises an attention-based graph reconstruction followed by STGNN for spatio-temporal pattern extraction. 
GPT-ST~\cite{li2023gpt} observes that existing methods encounter the lack of customized representations of spatio-temporal patterns and insufficient consideration of different levels of spatial dependencies and pre-trains the spatio-temporal input encodings used for STGNN models. Concretely, it designs a hierarchical hypergraph structure to capture temporal and multi-level spatial dependencies from a global perspective, with a model parameter customization scheme.

\subsec{Adaptation.} Adaptation for time series foundation models aims to tailor the pre-trained foundation models to new time series tasks or data for downstream performance enhancement. 
In the area of time series foundation models, despite most research efforts being the design of pre-training, advanced fine-tuning strategies receive little attention.
Alternatively, due to the emergence of prompt tuning methods in data modalities like natural language, vision, and graph~\cite{sun2023all}, prompting methods for time series also receive growing attention. For example, PT-Tuning~\cite{liu2023pt} adds tunable prompts into masked tokens to achieve the consistency of task objectives between pre-training (\ie masked reconstruction) and adaptation (\ie forecasting) in urban time series data. For time series classification, POND~\cite{wang2023prompt} further designs an instance-level prompt generator for adaptive prompting, besides the common prompt. Also, to capture diverse domain-specific information, POND proposes a meta-learning paradigm as well as elaborated contrastive constraints for prompt initialization.

Moreover, there have been some studies on prompt tuning for spatial-correlated time series tasks. To name a few, PromptST~\cite{zhang2023promptst} adds tunable prompts to spatiotemporal data to efficiently fine-tune the pre-trained traffic forecasting model and avoid catastrophic forgetting issue. STGP~\cite{hu2024prompt} designs a tow-stage prompting pipeline for spatio-temporal graph learning, which enables the prompts to curate domain knowledge and task-specific properties.
UniST~\cite{yuan2024unist} proposes a prior knowledge-guided prompt network to automatically learn the specific prompts for each case. Specifically, UniST firstly learns a spatial and a temporal memory pool with key-value structured parameters, and then it learns representations for each input with four aspects of spatio-temporal domain knowledge. The knowledge-guided prompts are extracted by quering the prompt memory pools with input representations.
MetePFL~\cite{chen2023prompt} and FedWing~\cite{chen2023spatial} focus on federated weather forecasting and use prompting techniques for personalized federated learning to reduce communication overheads and enhance privacy protection.

In a summary, existing unimodal approaches have put some preliminary efforts into building a universal time series foundation model. Diverse pre-training techniques have contributed to the development of time series foundation model. Some recent works have also paid the attention on more challenging questions, including how to enhance the universality of foundation model~\cite{yuan2024unist,liu2024unitime}, how to prompt the pre-trained model~\cite{hu2024prompt,yuan2024unist}, and how to improve the zero-shot capabilities~\cite{dasdecoder}. However, due to the intricate characteristics of spatiotemporal data, the foundation model tailored for urban scenarios is situated in the nascent state.

\subsubsection{Cross-modal transfer approaches} Due to insufficient time series data to train a foundation model from scratch, cross-modal transfer approaches directly adopt the foundation models pre-trained on other modalities and aim to transfer the modality-sharing knowledge to time series tasks. For instance, a fascinating work is V2S~\cite{yang2021voice2series} that leverages a pre-trained acoustic model for time series classification, by input reprogramming and output label mapping. 
Recently, most cross-modal studies have focused on adapting pre-trained LLMs for time series to sufficiently leverage the remarkable abilities of LLMs~\cite{jin2023large,jin2024position}. Upon whether the LLMs are open-sourced or purely black-box, we categorize them into two types: embedding-invisible LLM (\eg ChatGPT, GPT-4\footnote{\url{https://openai.com/blog/gpt-4-api-general-availability}}) and embedding-visible LLM (\eg GPT-2~\cite{radford2019language}, LLaMA~\cite{touvron2023llama}), which follows~\cite{jin2023large}. For the former type of LLMs, we could just infer by prompting with API calls, while for the latter type, we can fine-tune the model parameters or reprogram the time series inputs in various tasks.

\subsec{Prompt engineering.} Some recently released LLMs hold striking capabilities but are closed-sourced (\ie embedding-invisible). A plausible solution for adaptation is to transform the time series into natural language sentences as the prompts for API calls. PromptCast~\cite{xue2023promptcast} fisrtly proposes a novel prompt-based forecasting paradigm and releases a large-scale dataset PISA constructed with template-based prompts including weather temperature, electricity consumption and human mobility prediction tasks. Further, LLMTime~\cite{gruver2023large} contends that LLMs can be used directly as zero-shot forecasters without any added text or prompt engineering, if the input time series data are carefully preprocessed.

\subsec{Model fine-tuning.} Beyond prompting the generalist LLM, many works have contributed to fine-tuning embedding-visible LLMs for time series tasks. GPT(6)~\cite{zhou2023one1_nips} adopts pre-trained LLMs for diverse time series tasks. Specifically, it only fine-tunes a small part of the parameters of LLM (\ie positional embedding and layer normalization layer) for efficiency, and uses linear probing and patching to align the time series of various urban domains (weather, electricity, traffic) to language modality. Incrementally, GPT(6)-adapter~\cite{zhou2023one2} designs frequency adapter, temporal adapter, and channel adapter for tuning, to strengthen the LLM-based time series analysis. To align the modalities of time series and language, LLM4TS~\cite{chang2023llm4ts} design a two-stage fine-tuning process: firstly adopts auto-regressive supervised fine-tuning for time series; then fine-tunes the pre-trained model for downstream time series forecasting. Further, TEMPO~\cite{cao2023tempo} highlights that LLMs fail to capture the time series characteristics such as the trend, seasonality and distribution shift. It adopts the trend-seasonality decomposition for the input time series and respectively passes them to the LLM for reasoning. Also, tunable prompts are added to conquer the distribution shift in diverse time series data. To tackle time series with diverse context lengths, AutoTimes~\cite{liu2024autotimes} proposes an auto-regressive LLM-based forecasting approach, and adopts next token prediction as the training objective which is consistent with the LLM acquisition. Besides, AutoTimes designs token-wise prompting technique that utilizes the LLM generate the prompts indicating timestamp information.

To adapt the LLM for spatial-correlated time series, GATGPT~\cite{chen2023gatgpt} uses a graph attention module for spatial graph encoding and passes the spatio-temporal embeddings to the pre-trained GPT-2 model for downstream spatio-temporal imputation. TPLLM~\cite{ren2024tpllm} adopts 1-D convolutional neural networks and graph convolutional networks to enable LLMs to understand spatio-temporal patterns in traffic data.
Additionally, STG-LLM~\cite{liu2024can} proposes a spatio-temporal tokenizer to transform spatio-temporal data into tokens and an adapter architecture for efficient adaptation, which facilitate the understanding of pre-trained LLMs. Similarly, ST-LLM~\cite{liu2024spatial} treats the time steps at each spatial location as tokens, and fuse various spatial and temporal prior information into input embedding to facilitate traffic prediction. 

\subsec{Model reprogramming.} To explicitly align times series to natural language,  model reprogramming is an effective way that neither edits the time series inputs directly nor fine-tunes the pre-trained LLM. For example, TEST~\cite{sun2023test} focuses on a data-centric framework that freezes all the parameters of pre-trained LLM and tries to elaborate the model inputs. Concretely, to make the LLM understand the time series embedding, TEST aligns it to the text representation space with text-prototype-based contrastive learning and adds tunable prompts to help the LLM fit in the downstream forecasting and classification tasks. 
To unleash the potential of LLMs for time series forecasting, Time-LLM~\cite{jin2024time} reprogram time series into text prototype representations and add language-based prompts that describe the statistics of time series data. To avoid the large and dense reprogramming space, Time-LLM only maintains a small collection of the vocabulary by linearly probing the pretrained word embeddings.
To enhance the reprogramming framework for spatio-temporal data, RePST~\cite{wang2024empowering} decouples the spatio-temporal data in the frequency space to capture intricate spatio-temporal dependencies. Also RePST discretely samples word embeddings from the whole vocabulary to avoid semantic mixing and enhance the expressivity of text prototypes for spatio-temporal data.
To align the spatio-temporal dependencies with the comprehension space of LLMs, UrbanGPT~\cite{li2024urbangpt} proposes a spatio-temporal instruction tuning paradigm which aligns spatio-temporal data with the knowledge space of LLMs.


% \subsec{Summary.} 
% To conclude, LLM-based adaptation approaches hinge on how to align the modalities of natural language and time series~\cite{jin2024time}. Existing works either leverage the neural networks to automatically achieve the alignment in a data-driven way (\eg linear probing~\cite{zhou2023one1_nips,zhou2023one2,chang2023llm4ts,chen2023gatgpt}, prompt tuning~\cite{sun2023test,cao2023tempo}), explore the characteristics of time series (\eg trend-seasonal decomposition~\cite{cao2023tempo}, spatial correlation encoding~\cite{chen2023gatgpt}), or explicitly utilize text information as the guidance (\eg reprogramming~\cite{sun2023test,jin2024time} and manual prompting~\cite{jin2024time,xue2023promptcast,gruver2023large}).

To conclude, the cross-modal transfer approaches, especially LLM-based adaptation approaches, hinge on how to make LLMs comprehend time series data, hence we can unleash the significant reasoning ability of LLMs. 
Prompt engineering approaches~\cite{xue2023promptcast, gruver2023large} are flexible to use and are easy to generalize across various domains of time series data and diverging tasks. However, the disregard of parameter updating severely hinders the alignment between time series and natural language, which may render the failure on more intricate urban scenarios.
Therefore, most recent works focus on model fine-tuning. Specifically , they commit to the parameter-efficient tuning~\cite{zhou2023one1_nips} and how to capture the intricate patterns of time series~\cite{cao2023tempo,liu2024spatial} and language data~\cite{chang2023llm4ts,liu2024autotimes}. 
Furthermore, model reprogramming provides a more portable way for cross-modal transfer, which aims at reprogram time series into language-aware representations that facilitates the comprehension of LLMs~\cite{jin2024time}. However, most of these works are limited to a very high-level understanding of LLM for time series data.

\subsubsection{Outlook and Future Opportunities} In this section, we will discuss the current limitations and potential research opportunities of time series-based UFMs.

\subsec{Universality of time series-based UFMs.} 
Most of existing time series-based UFMs are limited into specific data domains, data formats or downstream tasks, which disobeys the universal property of foundation models. Based on these preliminary progress, there have been some works~\cite{liu2024timer,ekambaram2024ttms,gao2024units,yuan2024unist} that focus on the universality of time series-based UFMs. However, there still lack a generally accepted universal UFM that could be applied to various domains and heterogeneous formats of data and diverse downstream tasks.

\subsec{Theoretical analysis of LLMs.}
Recently, some studies have drawn inspirations from the success of LLMs to refine the time series UFM, such as adopting the auto-regressive pre-training strategy that is consistent with language modeling~\cite{liu2024generative,liu2024timer,chang2023llm4ts,liu2024autotimes}. However, how LLMs make effective predictions on urban time series domain is scarcely discussed. More studies should incorporate the understanding of LLMs as inspirations to reform current time series UFMs, by devising a urban-specific model architecture for unimodal pre-training, or a urban-aware alignment technique for cross-model transfer.

\subsec{Prior knowledge fusion for urban time series.}
There have been some works integrating the prior knowledge of time series into either pre-training or adaptation, such as multi-scale temporal pattern~\cite{liu2024generative,zhao2024himtm}, trend-seasonal property~\cite{cao2023tempo,dooley2024forecastpfn} and spatial correlations~\cite{liu2024spatial}. However, there still exist rich prior characteristics of urban time series in both temporal and spatial, local and global perspectives, which require future works to explore.

% \subsubsection{Outlook and Future Opportunities} In this section, we will discuss the current limitations and potential research opportunities of time series-based UFMs.

% \subsec{Universality of time series-based UFMs.} 
% Most of existing time series-based UFMs are limited into specific data domains, data formats or downstream tasks, which disobeys the universal property of foundation models. Based on these preliminary progress, there have been some works~\cite{liu2024timer,ekambaram2024ttms,gao2024units,yuan2024unist} that focus on the universality of time series-based UFMs. However, there still lack a generally accepted universal UFM that could be applied to various domains and heterogeneous formats of data and diverse downstream tasks.

% \subsec{Theoretical analysis of LLMs.}
% Recently, some studies have drawn inspirations from the success of LLMs to refine the time series UFM, such as adopting the auto-regressive pre-training strategy that is consistent with language modeling~\cite{liu2024generative,liu2024timer,chang2023llm4ts,liu2024autotimes}. However, the effectiveness of LLMs is scarcely discussed among existing works on time series UFMs, and more studies should incorporate the understanding of LLMs as inspirations to reform current time series UFMs.

% \subsec{Prior knowledge fusion for urban time series.}
% There have been some works integrating the prior knowledge of time series into either pre-training or adaptation, such as multi-scale temporal pattern~\cite{liu2024generative,zhao2024himtm}, trend-seasonal property~\cite{cao2023tempo,dooley2024forecastpfn} and spatial correlations~\cite{liu2024spatial}. However, there still exist rich prior characteristics of urban time series in both temporal and spatial, local and global perspectives, which require future works to explore.

% \subsec{Spatio-temporal UFMs.}
% Due to the complicated patterns of spatio-temporal data, the study of UFMs of spatial-correlated time series has lagged behind. For instance, the prompt engineering works for spatial-correlated time series are absent. Therefore more research efforts should be devoted to the pre-processing of spatio-temporal data and how to make LLMs comprehend the coupled spatio-temporal correlations.


==> sections/trajectory-based.tex <==
\subsection{Trajectory-based Models}
% \TODO{ add pre-training task-based taxonomy and conclusion}

Trajectory data, a prevalent modality in urban applications, plays a crucial role in various downstream tasks such as trajectory classification, next location prediction, and human mobility analysis. Several studies have focused on empowering UFMs to effectively comprehend trajectory data and adapt to a broad spectrum of downstream tasks. In this section, we discuss two primary types of trajectory-based approaches: (1) pretraining-based approaches; and (2) adaptation-based approaches.
\subsubsection{Pretraining-based Approaches}

The unique nature of trajectory data has led to research focusing on the development of domain-specific foundation models through targeted pre-training processes. This pre-training is designed either for specific downstream tasks or to cover a broader spectrum of multiple downstream tasks. We analyze these approaches in detail, categorizing them according to the type of self-supervised pre-training task employed in their pre-training: (1)~generative pre-training; (2)~contrastive pre-training; (3)~hybrid pre-training.

% location representation
% \textbf{\textsl{1) generative pre-training.}} 
\subsec{Generative pre-training.}
In generative pre-training, the primary goal of pre-training tasks is typically to generate or reconstruct trajectory points, thereby enhancing the pre-trained model's proficiency in point-level downstream tasks.
CTLE~\cite{ctle2021} presents a pre-training model tailored to learn representations of individual locations, primarily for tasks such as next location prediction. This model uses the masked language model (MLM) pre-training task from BERT, and generates location embeddings by considering contextual neighbors within trajectories, effectively addressing the multi-functional properties of locations.
Similarly, Trajectory-BERT~\cite{trajbert2023} introduces a method called Masked Trajectory Model (MTM) designed to accurately estimate trajectories in the presence of noise and missing points. It masks trajectories with a given probability and then feeds them into the BERT model to predict missing points.
% trajectory representation learning
\subsec{Contrastive pre-training.}
In contrast to generative pre-training tasks, models pre-trained using contrastive pre-training tasks frequently exhibit superior performance in sequence-level downstream tasks.
SML~\cite{sml2021} is a framework developed for modeling human mobility. By utilizing spatio-temporal context learning and integrating common data augmentation techniques, it addresses data sparsity, thereby improving its capability to understand human mobility patterns accurately. Additionally, the authors implement a pre-training task for model pre-training, followed by fine-tuning through contrastive trajectory learning. The effectiveness of SML is demonstrated in downstream location-based tasks, such as next location prediction and trajectory classification.
% trajectory representation learning
STPT~\cite{stpt2023} introduces a spatial-temporal pre-training and fine-tuning paradigm for learning a model that effectively represents human trajectories. This model significantly aids various downstream tasks by fine-tuning with task-specific data. During the pre-training phase, the model learns to predict the source of sub-trajectories through a self-supervised sub-trajectory similarity learning task. In the fine-tuning phase, the pre-trained model is adapted to diverse downstream tasks by incorporating corresponding task-specific adapters. STPT demonstrates notable enhancements in two fine-tuning tasks: multi-class trajectory classification and the distinction between seeking vs. serving trajectories.
\cite{cacsr2023} proposes an adversarial contrastive model CACSR to learn representation of check-in sequences. This model constructs a contrastive learning-based pre-training task for pre-training the encoder, enhancing representation learning. Post pre-training, CACSR undergoes fine-tuning for various multi-classification problems, such as location prediction and trajectory-user link tasks, where it demonstrates impressive performance.

% human mobility 
\subsec{Hybrid pre-training.}
To develop a more versatile trajectory-based foundation model, several studies have opted for hybrid self-supervised pre-training approaches.
\cite{movesim2020} introduces MoveSim, a generative adversarial framework aimed at simulating human mobility. This framework employs distinct pre-training tasks for both the generator and discriminator, leveraging the principles of spatial continuity and temporal periodicity in human mobility. Such an approach significantly enhances the simulation's fidelity.
In \cite{hmtrl2022}, HMTRL+ is presented as a route representation learning framework for multi-modal transportation recommendations. This model incorporates a spatiotemporal graph neural network to capture spatial and temporal autocorrelations, along with an attentive route representation module for semantic coherence in route sequences. Additionally, it features a hierarchical multi-task learning module to generate route representations for various transport modes. The authors also introduce a spatiotemporal pre-training strategy, enhancing generalization abilities via two pre-training tasks: masked attribute prediction and trajectory contrastive learning.
% trajectory representation learning
MMTEC~\cite{mmtec2023} designs a distinctive pre-training task employing maximum entropy coding to minimize biases in pre-training trajectory embeddings. This approach enables the learning of high-quality, general trajectory embeddings suitable for a variety of downstream trajectory-related tasks. The efficacy of MMTEC was tested through experiments on three specific tasks: similar trajectory search, travel time estimation, and destination prediction.
START~\cite{start2023} introduces two self-supervised tasks: span-masked trajectory recovery and trajectory contrastive learning, for pre-training a trajectory representation learning model. Following pre-training, this model exhibits robust transferability across heterogeneous road network datasets and demonstrates strong performance in three distinct downstream tasks.

\subsubsection{Adaptation-based Approaches}
Recent advancements in LLMs (\eg GPT-4~\cite{openai2023gpt4}, Llama2~\cite{touvron2023llama2}) have demonstrated exceptional zero-shot learning and generalization capabilities across various domains. In the realm of trajectory analysis, several studies have utilized LLMs for trajectory-based tasks.

A number of studies have explored the application of Large Language Models (LLMs) in addressing tasks associated with human mobility.
AuxMobLCast~\cite{auxmoblcast2022} transforms numerical temporal sequences into natural language sentences, fine-tunes pre-trained language models like BERT, RoBERTa, GPT-2, and XLNet for predicting visitor counts at points-of-interest (POIs).
LLM-Mob~\cite{llmmob2023} designs effective prompts to enhance LLMs' reasoning on mobility data, producing both accurate and interpretable predictions of individuals' subsequent locations. Experimental results indicate LLM-Mob's superior predictive performance and interpretability.
A study by \cite{zhang2023large} conducts empirical studies to evaluate the strengths and limitations of LLMs in detecting anomalous behaviors within human mobility data, comparing them with specialized anomaly detection algorithms.
LLM-MPE~\cite{llmmpe2023} aims to leverage LLMs for predicting human mobility in complex scenarios involving public events, utilizing a chain-of-thought prompting strategy to inform predictions based on historical mobility patterns and event textual descriptions.

Additionally, within the realm of autonomous driving, initiatives have been undertaken to harness LLMs for the purposes of motion planning and trajectory forecasting.
\cite{keysan2023can} presents an innovative method that integrates text-based scene descriptions with pre-trained language encoders for trajectory prediction in autonomous driving (AD). 
Similarly, GPT-Driver (referenced in \cite{gptdriver2023}) redefines motion planning as a language modeling task, converting heterogeneous planner inputs into language tokens. This process employs a GPT-3.5 model to process the input tokens and generate driving trajectory predictions.

Nevertheless, these studies predominantly convert either the entire or a portion of the input data into textual format to capitalize on the linguistic comprehension and inferential abilities of LLMs. The shift from specialized deep learning approaches to an emerging LLM-centered framework is an area that continues to be inadequately investigated.

==> sections/v2_basic_backup.tex <==
\section{Basics of Urban Foundation Models} \label{basic}

% \begin{figure*}[tb]
% \centering
% \includegraphics[width=1.95\columnwidth]{figs/basic1.pdf}
% \caption{Urban Foundation Models (UFMs) are pre-trained on multi-source, multimodal urban data and can be adapted for a variety of downstream applications.}
% \label{fig:basic}
% \end{figure*}

% \begin{figure*}[tb]
% \centering
% \includegraphics[width=1.95\columnwidth]{figs/basic3.pdf}
% \caption{Urban Foundation Models (UFMs) are pre-trained on multi-source, multi-granularity and multimodal urban data and can be adapted for a variety of downstream applications.}
% \label{fig:basic}
% \end{figure*}

\subsection{Concepts of Urban Foundation Models}

\begin{defi}[\textbf{Urban Foundation Models}]
Urban Foundation Models (UFMs) are large-scale models pre-trained on vast multi-source, multi-granularity, and multimodal urban data. It benefits significantly from its pre-training phase, exhibiting emergent capabilities and remarkable adaptability to a broader range of multiple downstream tasks and domains in urban contexts. 
\end{defi}

\subsubsection{Data Characteristics}
Urban Foundation Models (UFMs) are distinguished by their ability to process and analyze a vast array of data types, each contributing uniquely to the comprehensive understanding of urban dynamics. The data characteristics of UFMs, including multi-source, multi-granularity, and multi-modal aspects, are essential for capturing the complexities of urban environments. The following sections detail these key data characteristics.

\subsec{Multi-source.} UFMs integrate data from diverse urban sources, including sensor networks, social media, satellite imagery, mobile devices, \etc, facilitating a comprehensive understanding of urban environments.

\subsec{Multi-granularity.} UFMs handle data at different levels of granularity. At a macro level, they process city-wide patterns like traffic flow or population movement. At a micro level, they focus on specific neighborhoods or streets, analyzing local trends and behaviors.

\subsec{Multi-modal.} UFMs excel in integrating diverse data types such as textual, visual, and sensor-based inputs, enabling them to capture urban complexities more effectively than single-data-type models.

\subsubsection{Definition of Data Types}
Below are definitions and introductions to the major data types in urban contexts.

\subsec{Visual data.} This refers to any visual information captured in image or video format, including street view images, satellite imagery, and urban surveillance footage. Formally, an image can be represented as a 3-dimensional matrix $ I(x, y, c) $ where $x$ and $y$ represent the spatial dimensions (width and height) of the image, and $c$ represents the color channels. Each entry in the matrix corresponds to a pixel value. For color images, this extends to a 3D matrix to include color channels, typically RGB (Red, Green, Blue).

\subsec{Textual data.} This refers to data that is composed of written language. Examples include social media posts, geo-text data, and documents relevant to urban environments. Formally, textual data can be represented as a sequence of tokens $ T = [t_1, t_2, \ldots, t_n] $ where each token $ t_i $ corresponds to a word or character in the text. These tokens are often transformed into numerical representations (like word embeddings) for processing in UFMs.

\subsec{Geo-sensory data.} This refers to data collected from physical geospatial sensors in an urban environment. This includes GPS sensors, traffic sensors, weather stations, and other IoT devices. Formally, sensor data can be represented as a time-series collection $ S(t) = \left\{ (s_1, t_1), (s_2, t_2), \ldots, (s_n, t_n) \right\} $ where each data point $ s_i $ at time $ t_i $ corresponds to a sensor reading. These readings can vary in nature (e.g., GPS positions, traffic volumes, and air quality indices) depending on the sensor type.



\subsubsection{Key Techniques of Constructing Urban Foundation Models}

UFMs, similar to foundation models in other fields, primarily rely on two key techniques, \ie pre-training and adaptation.

\subsec{Pre-training.}
UFMs typically undergo pre-training on extensive, varied datasets comprising geo-text data, social media content, street view images, trajectories, spatiotemporal time series data, point-of-interests, \etc The primary goal of pre-training is to enable these models to obtain as much general knowledge and patterns as possible, thereby capturing the overarching characteristics and structures inherent in the data. Pre-training methods for UFMs are principally divided into four categories: supervised pre-training, generative pre-training, contrastive pre-training, and hybrid pre-training \cite{sslsurvey2021}:

\subsubsec{(1) Supervised pre-training.} This method involves training models on datasets with a substantial volume of labeled data, pairing an input with its corresponding output. This approach allows models to learn the relationship between inputs and outputs in a supervised manner. Suppose $\mathcal{D} = \{ (x_1, y_1), (x_2, y_2), \ldots, (x_N, y_N) \}$ is the training dataset, where $x_i$ represents the $i$-th sample and $y_i$ is the corresponding label. Here is an example of the most commonly used cross-entropy loss function~\cite{goodfellow2016deep}:
\begin{equation}
    L_{sup} = -\sum_{i=1}^{N} \sum_{c=1}^{C} y_{ic} \log(\hat{y}_{ic}) ,\label{l_sup}
\end{equation}
where $N$ is the number of samples, $C$ is the number of classes,  $y_{ic}$ is a binary indicator (0 or 1) if class label $c$ is the correct classification for observation $i$, $\hat{y}_{ic}$ is the predicted probability observation $i$ is of class $c$.

\subsubsec{(2) Generative pre-training.} This approach trains models to generate or reconstruct input data in the absence of labeled data. It necessitates the model's ability to autonomously discern patterns and regularities, thereby producing outputs that closely mimic real data. Here is an example of loss function in generative pre-training called Negative Log-Likelihood (NLL) loss~\cite{radford2018improving}:
\begin{equation}
    L_{gen} = -\sum_{i=1}^{N} \log P(x_i | x_{<i}, \theta) \label{l_gen},
\end{equation}
where $N$ is the number of tokens in the sequence, $x_i$ represents the $i$-th token, $x_{<i}$ represents all tokens before the $i$-th token, $P(x_i | x_{<i}, \theta)$ is the probability assigned by the model to the correct token $x_i$, given the preceding tokens $x_{<i}$ and the model parameters $\theta$.

\subsubsec{(3) Contrastive pre-training.} This method trains models to distinguish between data instances and learn robust data representations by evaluating similarities and differences among data samples, all without needing externally provided labels. A simple form of the contrastive loss for a pair of samples can be defined as follows~\cite{hadsell2006dimensionality}:
% \begin{equation}
%     L_{con} = y \times D^2 + (1 - y) \times \max(0, \epsilon - D)^2, \label{l_con}
% \end{equation}
\begin{equation}
    L_{con} = yD^2 + (1 - y)\max(0, \epsilon - D)^2, \label{l_con}
\end{equation}
where $y$ is a binary label indicating whether the pair has the same labels ($y=1$) or different labels ($y=0$), $D$ is the distance between the representations of the pair of samples, often calculated using a metric like Euclidean distance, and $\epsilon$ is a hyperparameter that defines the minimum distance between dissimilar pairs.

\subsubsec{(4) Hybrid pre-training.} This approach integrates multiple pre-training methods, including supervised, generative, and contrastive techniques. This strategy aims to tailor the training process to specific problem demands, leveraging the strengths of each method. 

Since obtaining a large amount of high-quality human-labeled data can be expensive or impractical in many domains, generative and contrastive pre-training are frequently employed to fully leverage various types of datasets. These methods optimize the model's performance and adaptability. Supervised pre-training may be used in specific application scenarios, particularly with abundant high-quality labeled data.

\subsec{Adaptation.}
After pre-training, models can be customized to specific tasks or domains through several adaptation methods. These adaptation methods enhance the flexibility and power of UFMs across diverse application contexts. Selecting suitable adaptation strategies is crucial for maximizing the performance of pre-trained models on specific tasks and datasets while reducing resource costs.

    \zhaobite{\subsubsec{(1) Model fine-tuning.} Model fine-tuning is a widely used adaptation method in UFMs. This approach involves additional training of the pre-trained model using a task-specific dataset. During fine-tuning, the model's parameters are adjusted to optimize its performance for the particular task at hand. Fine-tuning is direct and effective for task-specific adaptation, but it may demand significant amounts of training data and computational resources. This method is particularly useful when ample labeled data is available for the target task. Besides, there are also some parameter-efficient fine-tuning methods~\cite{hu2021lora} which minimize the number of parameters that require adjustment during adaptation, maintaining a balance between model adaptation performance and resource consumption.}
\subsubsec{(1) Model fine-tuning.} Model fine-tuning is a widely used adaptation method in UFMs. This approach involves additional training of the pre-trained model using a task-specific dataset. The process of fine-tuning adjusts the parameters of the model to enhance its effectiveness for the specific task. Fine-tuning is direct and effective for task-specific adaptation, but it may demand significant amounts of training data and computational resources. This method is particularly useful when sufficient labeled data is available for the target task. Besides, there are also some parameter-efficient fine-tuning methods~\cite{hu2021lora} which minimize the number of parameters that require adjustment during adaptation, maintaining a balance between model adaptation performance and resource consumption.
    \zhaobite{\subsubsec{(2) Prompt tuning.} In contrast to the conventional ``pre-train, fine-tune'' paradigm, prompt-tuning employs lightweight prompt tokens containing relevant information about the target task. In practice, such prompts are often a small number of task-specific learnable parameters~\cite{jia2022visual}. During the fine-tuning stage, the parameters of the pre-trained backbone model are frozen, and only the trainable prompts are adjusted. This method has proven effective in leveraging the inherent knowledge embedded in the pre-trained backbone. This ``Pre-train, Prompt and Predict'' paradigm~\cite{promptsurvey2023} is more efficient, as it necessitates training only a minimal set of prompt parameters, thereby avoiding the need for extensive alterations to the model's existing parameters.}

\subsubsec{(2) Prompt tuning.} Diverging from the traditional ``pre-train, fine-tune'' paradigm, prompt-tuning employs lightweight prompt tokens containing relevant information about the target task. In practice, such prompts are often a small number of task-specific learnable parameters~\cite{jia2022visual}. During the prompt-tuning stage, the parameters of the pre-trained backbone model are frozen, and only the trainable prompts are adjusted. This method has proven effective in leveraging the inherent knowledge embedded in the pre-trained backbone. This ``Pre-train, Prompt and Predict'' paradigm~\cite{promptsurvey2023} is more efficient, as it necessitates training only a minimal set of prompt parameters, thereby avoiding the need for extensive alterations to the model's existing parameters.

\subsubsec{(3) Prompt engineering.} Prompt engineering~\cite{radford2019language} is a training-free approach to directly adopt foundation models like LLMs without altering the parameters of pre-trained models. It involves designing task-specific prompts that guide the model's responses. These prompts act as instructions or hints, steering the model's attention toward relevant information within the input data.

These adaptation methods, including fine-tuning, prompt-tuning, and prompt engineering, provide UFMs with the adaptability needed to excel in different urban contexts. The choice of adaptation strategy depends on the availability of data, computational resources, and the specific requirements of the target task. Each method uniquely balances performance and resource efficiency, making UFMs versatile tools for urban applications.
% After pre-training, models can be tailored to specific tasks or domains through several methods like fine-tuning. During this phase, the model is trained on smaller, task-specific datasets to adjust and optimize its parameters, enhancing its performance for the particular task. Below are several prevalent adaptation methods.
% \subsubsec{Vanilla fine-tuning.} This approach entails additional training of the pre-trained model using a task-specific dataset. It typically involves adjusting most or all of the model's parameters. Although direct and effective for task-specific adaptation, this method may demand significant amounts of training data and computational resources.
% \subsubsec{Parameter-efficient fine-tuning.} This technique minimizes the number of parameters that require adjustment during adaptation. It involves training only a subset of the model, thereby reducing training costs. This method maintains a balance between model adaptation performance and resource consumption~\cite{hu2021lora}
% \subsubsec{Prompt-tuning.} In contrast to the conventional ``pre-train, fine-tune'' approach, prompt-tuning employs lightweight prompt tokens containing relevant information about the target task. This method has proven effective in leveraging the inherent knowledge embedded in the pre-trained backbone. This ``Pre-train, Prompt and Predict'' paradigm \cite{promptsurvey2023} is more efficient, as it necessitates training only a minimal set of prompt parameters, thereby avoiding the need for extensive alterations to the model's existing parameters.
% These adaptation methods enhance the flexibility and power of UFMs across diverse application contexts. Selecting suitable adaptation strategies is crucial for maximizing the performance of pre-trained models on specific tasks and datasets while reducing resource costs.
\subsection{Challenges of Building Urban Foundation Models}

While Urban Foundation Models (UFMs) offer significant potential for understanding and managing complex urban environments, building UFMs is a complex task that encounters several intricate challenges. These challenges stem primarily from the inherent complexities of urban data, the dynamic nature of urban environments, and the diverse range of applications UFMs are expected to address. Below, we delve into the key challenges that underscore the intricacies of building effective UFMs.

\subsec{Multi-source, multi-granularity, and multi-modal data integration.}
The integration of multi-source, multi-granularity, and multi-modal data is one of the primary challenges in building UFMs. UFMs must effectively combine data from various sources like social media, satellite imagery, urban sensors, and traffic records. Each source provides data at different levels of granularity, from broad city-wide patterns to specific local details. Moreover, the data modalities vary significantly, encompassing text, images, videos, sensor readings, \etc
Integrating these disparate data types poses significant challenges in data preprocessing, normalization, and fusion. The models must be able to discern relevant patterns across these diverse datasets and reconcile potential conflicts or discrepancies in the data.

\subsec{Spatio-temporal reasoning capability.}
Another major challenge in UFMs is mastering spatio-temporal reasoning. Urban environments are dynamic, with changes and patterns evolving over both space and time. UFMs need to understand and predict complex phenomena that are time-dependent and spatial-dependent. This involves sophisticated modeling of temporal sequences and spatial distributions, requiring advanced algorithms capable of handling high-dimensional data. This spatio-temporal reasoning skill is particularly vital in urban contexts and is often less emphasized or absent in other foundation model types.

% \subsec{Alignment with diverse urban task domains.}
\subsec{Versatility to diverse urban task domains.}
Finally, the versatility of UFMs to diverse urban task domains is a significant challenge. Urban environments encompass a wide array of domains, such as transportation, urban planning, energy management, and environmental monitoring. Each domain presents unique challenges and requirements, and UFMs need to be versatile enough to adapt to these varied contexts. This involves not only tailoring the models to specific tasks but also ensuring that they can be generalized across different urban scenarios. The challenge lies in developing models that are both specialized for particular tasks and flexible enough to accommodate the multifaceted nature of urban environments. This requires a careful balance between model complexity and applicability, ensuring that UFMs can be effectively deployed in real-world urban settings.

\TODO{\subsec{Privacy and security concerns.}
Privacy reference: The use of vast data from multiple sources raises significant privacy concerns, and UFMs should be developed with stringent adherence to privacy regulations such as the GDPR~\cite{voigt2017eu}. Balancing the utility of urban data with the privacy and security of individuals remains a complex but essential task for any data-driven urban system.

Security: \eg~robustness under attacks.
}


==> sections/v2_taxonomy.tex <==
\begin{figure*}[tb]
\centering
\includegraphics[width=2\columnwidth]{figs/taxonomy_240114.png}
\caption{A detailed taxonomy of existing UFMs-related works based on the types of urban data modalities.}
\label{fig:taxonomy}
\end{figure*}

\onecolumn
\small % 或 \footnotesize 或 \scriptsize
\begin{longtable}{m{5mm}|m{3cm}m{3cm}m{2cm}m{3cm}m{4cm}}
    \caption{Summary of existing works.} \label{table:summary} \\
    \toprule
    \textbf{} & \textbf{Study} & \textbf{Data Type} & \textbf{Pre-training} & \textbf{Adaptation} & \textbf{Application} \\
    \midrule
    \endfirsthead

    \multicolumn{6}{c}{{\bfseries Table \thetable\ Summary of existing works (continued).}} \\
    \toprule
    \textbf{} & \textbf{Study} & \textbf{Data Type} & \textbf{Pre-training} & \textbf{Adaptation} & \textbf{Application} \\
    \midrule
    \endhead

    \midrule
    \multicolumn{6}{r}{{Continued on next page}} \\ 
    \endfoot

    \bottomrule
    \endlastfoot

    \multirow{10}{*}{\rotatebox{90}{\textbf{Language-based Models}}} & ERNIE-GeoL~\cite{huang2022ernie} & POI corpus, user behavior logs & Generative & Model fine-tuning & Map services \\
    \cline{2-6}
    ~ & MGeo~\cite{ding2023mgeo} & POI corpus & Generative, contrastive & Model fine-tuning & Query-POI matching \\
    \cline{2-6}
    ~ & Ji et al.~\cite{ji2023evaluating} & Geo-text, user instructions & - & Prompt engineering & Geographic information systems \\
    \cline{2-6}
    ~ & Bhandari et al.~\cite{bhandari2023large} & Geo-text, user instructions & - & Prompt engineering & Geographic information systems \\
    \cline{2-6}
    ~ & GPT4GEO~\cite{roberts2023gpt4geo} & Geo-text, user instructions & - & Prompt engineering & Geographic information systems \\
    \cline{2-6}
    ~ & Mooney et al.~\cite{mooney2023towards} & Geo-text, user instructions & - & Prompt engineering & Geographic information systems \\
    \cline{2-6}
    ~ & Mai et al.~\cite{mai2023opportunities} & Geo-text, user instructions & - & Prompt engineering & Geographic information systems \\
    \cline{2-6}
    ~ & Fu et al.~\cite{fu2023towards} & Documents, geo-text, user instructions & - & Prompt engineering & Urban science \\
    \cline{2-6}
    ~ & Aghzal et al.~\cite{aghzal2023can} & Geo-text, user instructions & - & Prompt engineering & Path planning \\
    \cline{2-6}
    ~ & GeoLLM~\cite{manvi2023geollm} & POI corpus & - & Prompt engineering & Geospatial prediction \\
    \cline{2-6}
    ~ & Zheng et al.~\cite{zheng2023chatgpt} & Traffic documents, user instructions & - & Prompt engineering & Intelligent transportation \\
    \cline{2-6}
    ~ & SpaBERT~\cite{li2022spabert}, GeoLM~\cite{li2023geolm} & Geo-text & - & Model fine-tuning & Geographic language understanding \\
    \cline{2-6}
    ~ & QUERT~\cite{xie2023quert} & User behavior logs & - & Model fine-tuning & Travel query understanding \\
    \cline{2-6}
    ~ & GEDR~\cite{mei2023improving} & POI corpus, user behavior logs & - & Model fine-tuning & Query-POI matching \\
    \cline{2-6}
    ~ & Wang et al.~\cite{wang2023optimizing} & LLM-generated instructions & - & Model fine-tuning & Urban renewal \\
    \cline{2-6}
    ~ & K2~\cite{deng2023learning} & Geo-text, geoscience instructions & - & Model fine-tuning & Geoscience tasks \\
    \midrule[0.5pt]
    
    \multirow{10}{*}{\rotatebox{90}{\textbf{Vision-based Models}}} & Urban2vec~\cite{wang2020urban2vec} & Street-view images & Contrastive & Model fine-tuning & \tabincell{c}{Demographic prediction, socioeconomic prediction} \\
    \cline{2-6}
    ~ & Li et al.~\cite{li2022predicting} & Street-view images & Contrastive & Model fine-tuning & Socioeconomic prediction \\
    \cline{2-6}
    ~ & KnowCL~\cite{liu2023knowledge} & Street-view images & Contrastive & Model fine-tuning & Socioeconomic prediction \\
    \cline{2-6}
    ~ & Wang et al.~\cite{wang2022advancing} & Remote sensing images & Generative & Model fine-tuning & \tabincell{c}{Remote sensing image analysis} \\
    \cline{2-6}
    ~ & ScaleMAE~\cite{reed2023scale} & Remote sensing images & Generative & Model fine-tuning & \tabincell{c}{Remote sensing image analysis} \\
    \cline{2-6}
    ~ & Cha et al.~\cite{cha2023billion} & Remote sensing images & Generative & Model fine-tuning & \tabincell{c}{Remote sensing image analysis} \\
    \cline{2-6}
    ~ & RingMo~\cite{sun2022ringmo} & Remote sensing images & Generative & Model fine-tuning & \tabincell{c}{Remote sensing image analysis} \\
    \cline{2-6}
    ~ & RingMo-Sense~\cite{yao2023ringmo} & Remote sensing images & Generative & Model fine-tuning & \tabincell{c}{Remote sensing spatiotemporal prediction} \\
    \cline{2-6}
    ~ & CSP~\cite{mai2023csp} & Remote sensing images & Contrastive & Model fine-tuning & \tabincell{c}{Satellite image classification} \\
    \cline{2-6}
    ~ & \tabincell{c}{FourCastNet~\cite{pathak2022fourcastnet}, Pangu-Weather~\cite{bi2023accurate}, FengWu~\cite{chen2023fengwu}} & Grid-based meteorological data & Generative & - & \tabincell{c}{Weather forecasting, tropical cyclones tracking} \\
    \cline{2-6}
    ~ & ClimaX~\cite{nguyen2023climax} & Grid-based meteorological data & Generative & Model fine-tuning & \tabincell{c}{Weather and climate modeling} \\
    \cline{2-6}
    ~ & W-MAE~\cite{man2023w} & Grid-based meteorological data & Generative & Model fine-tuning & \tabincell{c}{Weather forecasting, precipitation forecasting} \\
    \cline{2-6}
    ~ & SAMRS~\cite{wang2023samrs}, RSPrompter~\cite{chen2023rsprompter} & Remote sensing images & - & Prompt engineering & \tabincell{c}{Remote sensing semantic segmentation} \\
    \cline{2-6}
    ~ & Roberts et al.~\cite{roberts2023charting} & Remote sensing images & - & Prompt engineering & \tabincell{c}{Remote sensing image analysis} \\
    \cline{2-6}
    ~ & GeoSAM~\cite{sultan2023geosam} & Remote sensing images & - & Model fine-tuning & \tabincell{c}{Mobility infrastructure segmentation} \\
    \cline{2-6}
    ~ & RingMo-SAM~\cite{yan2023ringmo} & Remote sensing images & - & Model fine-tuning & \tabincell{c}{Multi-source remote sensing segmentation} \\
    \cline{2-6}
    ~ & Zhang et al.~\cite{zhang2022migratable} & Street-view images & - & Model fine-tuning & \tabincell{c}{Street-view image analysis} \\
    \cline{2-6}
    ~ &  StreetCLIP~\cite{sultan2023geosam} & Street-view images & - & Model fine-tuning & \tabincell{c}{Image geolocalization} \\
    
    % Trajectory-based Models
    \midrule[0.5pt]
    ~ & t2vec~\cite{t2vec2018} & Trajectory in road networks & Generative & Model fine-tuning & \tabincell{c}{Similar trajectory search} \\
    \cline{2-6}
    ~ & traj2vec~\cite{traj2vec2017} & Trajectory in road networks & Generative & Model fine-tuning & \tabincell{c}{Trajectory cluster} \\
    \cline{2-6}
    \multirow{40}{*}{\rotatebox{90}{\textbf{Trajectory-based Models}}} & Trembr~\cite{Trembr2020} & Trajectory in road networks & Generative & Model fine-tuning & \tabincell{c}{Similar trajectory search, travel time estimation, destination prediction} \\
    \cline{2-6}
    ~ & Toast~\cite{toast2021} & Trajectory in road networks & Generative & Model fine-tuning & \tabincell{c}{Road label classification, traffic inference, trajectory similarity search, travel time estimation} \\
    \cline{2-6}
    ~ & PIM~\cite{pim2021} & Trajectory in road networks & Contrastive & Model fine-tuning & \tabincell{c}{Travel time estimation, path ranking} \\
    \cline{2-6}
    ~ & STPT~\cite{stpt2023} & Trajectory in road networks & Contrastive & Model fine-tuning & \tabincell{c}{Trajectory classification, driving activity identification} \\
    \cline{2-6}
    ~ & LightPath~\cite{lightpath2023} & Trajectory in road networks & Generative & Model fine-tuning & \tabincell{c}{Travel time estimation, path ranking} \\
    \cline{2-6}
    ~ & MMTEC~\cite{mmtec2023} & Trajectory in road networks & Maximum Entropy Coding & Prompt engineering & \tabincell{c}{Similar trajectory search, travel time estimation,  destination prediction.} \\
    \cline{2-6}
    ~ & START~\cite{start2023} & Trajectory in road networks & \tabincell{c}{Generative, contrastive} & Prompt engineering & \tabincell{c}{Travel time estimation, trajectory classification, most similar trajectory search} \\
    \cline{2-6}
    ~ & HMTRL~\cite{hmtrl2022} & Trajectory in road networks & \tabincell{c}{Generative, contrastive} & Model fine-tuning & \tabincell{c}{Route recommendation} \\
    \cline{2-6}
    ~ & Movesim~\cite{movesim2020} & Trajectory in free space & \tabincell{c}{Generative, contrastive} & - & \tabincell{c}{Human mobility simulation} \\
    \cline{2-6}
    ~ & SML~\cite{sml2021} & Trajectory in free space & Contrastive & Model fine-tuning & \tabincell{c}{Location prediction, trajectory–user linking} \\
    \cline{2-6}
    ~ &  CTLE~\cite{ctle2021} & Trajectory in free space & Generative & - & \tabincell{c}{Next location prediction} \\
    \cline{2-6}
    ~ &  CACSR~\cite{cacsr2023} & Trajectory in free space & Contrastive & Model fine-tuning & \tabincell{c}{Next location prediction, trajectory user linking} \\
    \cline{2-6}
    ~ &  CATUS~\cite{CATUS2023} & Trajectory in free space & Contrastive & Model fine-tuning & \tabincell{c}{Next location prediction} \\
    \cline{2-6}
    ~ &  AuxMobLCast~\cite{auxmoblcast2022} & \tabincell{c}{Mobility prompt, user instructions} & - & Prompt engineering & \tabincell{c}{Human mobility forecasting} \\
    \cline{2-6}
    ~ &  LLM-Mob~\cite{llmmob2023} & \tabincell{c}{Mobility prompt, user instructions} & - & Prompt engineering & \tabincell{c}{Next location prediction} \\
    \cline{2-6}
    ~ &  Zhang et al.~\cite{zhang2023large} & \tabincell{c}{Mobility prompt, user instructions} & - & Prompt engineering & \tabincell{c}{Anomalous trajectory detection} \\
    \cline{2-6}
    ~ &  LLM-MPE~\cite{llmmpe2023} & \tabincell{c}{Mobility prompt, user instructions} & - & Prompt engineering & \tabincell{c}{Human mobility forecasting} \\
    \cline{2-6}
    ~ &  Keysan et al.~\cite{keysan2023can} & \tabincell{c}{Text description of scene, user instructions} & - & Prompt engineering & \tabincell{c}{Motion planning, driving trajectory prediction} \\
    \cline{2-6}
    ~ &  GPT-Driver~\cite{gptdriver2023} & \tabincell{c}{Text description of scene, user instructions} & - & Prompt engineering & \tabincell{c}{Motion planning, driving trajectory prediction} \\
    \cline{2-6}
    ~ &  LanguageMPC~\cite{languagempc2023} & \tabincell{c}{Text description of scene, user instructions} & - & Prompt engineering & \tabincell{c}{Motion planning, driving trajectory prediction} \\
    
    % Time series-based Models
    \midrule[0.5pt]
    \multirow{33}{*}{\rotatebox{90}{\textbf{Time series-based Models}}} 
    & Oreshkin et al.~\cite{oreshkin2021meta} & Ordinary time series & Supervised & - & \tabincell{c}{Energy consumption forecasting, traffic forecasting}\\
    \cline{2-6}
    ~ & Lag-Llama~\cite{rasul2023lag} & Ordinary time series & Supervised & - & Traffic forecasting\\
    \cline{2-6}
    ~ & SASA~\cite{cai2021time} & Ordinary time series & Supervised & - & Air quality regression\\
    \cline{2-6}
    ~ & TST~\cite{zerveas2021transformer} & Ordinary time series & Generative & - & Traffic regression\\
    \cline{2-6}
    ~ & SimMTM~\cite{dong2023simmtm} & Ordinary time series & Generative & - & \tabincell{c}{Weather forecasting, energy consumption forecasting, traffic forecasting}\\
    \cline{2-6}
    ~ & PatchTST~\cite{nie2022time} & Ordinary time series & Generative & - & \tabincell{c}{Weather forecasting, energy consumption forecasting, traffic forecasting}\\
    \cline{2-6}
    ~ & TSMixer~\cite{ekambaram2023tsmixer} & Ordinary time series & Generative & - & \tabincell{c}{Weather forecasting, energy consumption forecasting, traffic forecasting}\\
    \cline{2-6}
    ~ & PT-Tuning~\cite{liu2023pt} & Ordinary time series & Generative & Prompt engineering & \tabincell{c}{Weather forecasting, energy consumption forecasting, traffic forecasting}\\
    \cline{2-6}
    ~ & T-Loss~\cite{franceschi2019unsupervised} & Ordinary time series & Contrastive & - & \tabincell{c}{Traffic forecasting, energy consumption forecasting}\\
    \cline{2-6}
    ~ & COST~\cite{woo2022cost} & Ordinary time series & Contrastive & - & \tabincell{c}{Weather forecasting, energy consumption forecasting, traffic forecasting}\\
    \cline{2-6}
    ~ & TS2Vec~\cite{yue2022ts2vec} & Ordinary time series & Contrastive & - & \tabincell{c}{Traffic classification, energy consumption classification}\\
    \cline{2-6}
    ~ & SimTS~\cite{zheng2023simts} & Ordinary time series & Contrastive & - & \tabincell{c}{Weather forecasting, traffic forecasting}\\
    \cline{2-6}
    ~ & UniTime~\cite{liu2023unitime} & Ordinary time series & Hybrid & - & \tabincell{c}{Weather forecasting, energy consumption forecasting, traffic forecasting}\\
    \cline{2-6}
    ~ & ST-GSP~\cite{zhao2022st} & Spatial time series & Generative & - & Traffic forecasting\\
    \cline{2-6}
    ~ & STGCL~\cite{liu2022contrastive} & Spatial time series & Contrastive & - & Traffic forecasting\\
    \cline{2-6}
    ~ & STEP~\cite{shao2022pre} & Spatial time series & Generative & - & Traffic forecasting\\
    \cline{2-6}
    ~ & TransGTR~\cite{jin2023transferable} & Spatial time series & Hybrid & - & Traffic forecasting\\
    \cline{2-6}
    ~ & MC-STL~\cite{zhang2023mask} & Spatial time series & Hybrid & - & Traffic forecasting\\
    \cline{2-6}
    ~ & TPB~\cite{liu2023cross} & Spatial time series & Hybrid & - & Traffic forecasting\\
    \cline{2-6}
    ~ & GPT-ST~\cite{li2023gpt} & Spatial time series & Generative & - & Traffic forecasting\\
    \cline{2-6}
    ~ & PromptST~\cite{zhang2023promptst} & Spatial time series & - & Prompt engineering & \tabincell{c}{Traffic forecasting, complaint forecasting}\\
    \cline{2-6}
    ~ & MetePFL~\cite{chen2023prompt} & Spatial time series & - & Prompt engineering & Weather forecasting\\
    \cline{2-6}
    ~ & FedWing~\cite{chen2023spatial} & Spatial time series & - & Prompt engineering & Weather forecasting\\
    \cline{2-6}
    ~ & PromptCast~\cite{xue2023promptcast} & Ordinary time series & - & Prompt engineering & \tabincell{c}{Weather forecasting, energy consumption forecasting, human mobility forecasting}\\
    \cline{2-6} 
    ~ & LLMTime~\cite{gruver2023large} & Ordinary time series & - & Prompt engineering & \tabincell{c}{Weather forecasting, energy consumption forecasting, traffic forecasting}\\
    \cline{2-6} 
    ~ & GPT(6)~\cite{zhou2023one1_nips} & Ordinary time series & - & Model fine-tuning & \tabincell{c}{Weather forecasting, energy consumption forecasting, traffic forecasting}\\
    \cline{2-6} 
    ~ & GPT(6)-adapter~\cite{zhou2023one2} & Ordinary time series & - & Model fine-tuning & \tabincell{c}{Weather forecasting, energy consumption forecasting, traffic forecasting}\\
    \cline{2-6} 
    ~ & LLM4TS~\cite{chang2023llm4ts} & Ordinary time series & - & Model fine-tuning & \tabincell{c}{Weather forecasting, energy consumption forecasting, traffic forecasting}\\
    \cline{2-6} 
    ~ & TEMPO~\cite{cao2023tempo} & Ordinary time series & - & Model fine-tuning & \tabincell{c}{Weather forecasting, energy consumption forecasting, traffic forecasting}\\
    \cline{2-6} 
    ~ & GATGPT~\cite{chen2023gatgpt} & Spatial time series & - & Model fine-tuning & \tabincell{c}{Traffic forecasting, air quality imputation}\\
    \cline{2-6} 
    ~ & V2S~\cite{yang2021voice2series} & Ordinary time series & - & Model Reprogramming & Traffic classification\\
    \cline{2-6} 
    ~ & Time-LLM~\cite{jin2023time} & Ordinary time series & - & Model reprogramming & Traffic forecasting\\
    \cline{2-6}
    ~ & TEST~\cite{sun2023test} & Ordinary time series & - & Model reprogramming & \tabincell{c}{Traffic forecasting, energy consumption forecasting, air quality forecasting}\\
    
    \midrule[0.5pt]
    \multirow{14}{*}{\rotatebox{90}{\textbf{Multimodal Models}}} &  UrbanCLIP~\cite{yan2023urban} & Satellite image, textual description	& Contrastive & Model fine-tuning & Urban region profiling \\
    \cline{2-6}
    ~ & TengYun~\cite{zhao2023parallel} & Traffic-related text and image & Generative & Prompt tuning & \tabincell{c}{Traffic prediction and control, transportation planning} \\
    \cline{2-6}
    ~ & CityFM~\cite{balsebre2023city} & Spatial, visual, and textual geo-data & Contrastive	& -	& \tabincell{c}{Traffic speed inference, building functionality classification}\\
    \cline{2-6}
    ~ & AllSpark~\cite{shao2023allspark} & Text, image, trajectory, graph, etc.	& Contrastive &	Prompt engineering & Spatiotemporal data analysis \\
    \cline{2-6}
    ~ & TrafficGPT~\cite{zhang2023trafficgpt} & Multimodal traffic data & - & Prompt engineering & Traffic management \\
    \cline{2-6}
    ~ & GeoGPT~\cite{zhang2023geogpt} & Multimodal geospatial data	& -	& Prompt tuning	& \tabincell{c}{Autonomous geospatial data collection, processing, and analysis} \\
    \cline{2-6}
    ~ & VELMA~\cite{schumann2023velma} & Street image, navigation instruction	& -	& Model fine-tuning	& Autonomous street navigation \\
    \cline{2-6}
    ~ & UGI~\cite{xu2023urban} & \tabincell{c}{Urban textual, visual, knowledge graph, human behavior data} & - & \tabincell{c}{Continue learning, model fine-tuning} & \tabincell{c}{Urban planning and simulation, location recommendation} \\
    % \bottomrule[1pt]
\end{longtable}
\normalsize
\twocolumn


\section{Overview of Urban Foundation Models} \label{overview}
As illustrated in \figref{fig:taxonomy}, we introduce a data-centric taxonomy for the UFMs-related studies to shed light on the progress and efforts made in this field. Based on the urban data modalities, we categorize the existing works on UFMs into six classes: language-based models,  vision-based models, trajectory-based models, time series-based models, multimodal models, and others. Moreover, we further categorize the studies of each class into two subclasses based on their technical approaches: pretraining-based approaches and adaptation-based approaches.

\input{sections/language-based}

\input{sections/vision-based}

\input{sections/v2_trajectory-based}

\input{sections/time-series/v2_time-series-based}

\input{sections/multimodal-based}

\input{sections/others}

==> sections/v3_taxonomy.tex <==
\begin{figure*}[tb]
\centering
\includegraphics[width=2\columnwidth]{figs/taxonomy_240114.png}
\caption{A detailed taxonomy of existing UFMs-related works based on the types of urban data modalities.}
\label{fig:taxonomy}
\end{figure*}

\onecolumn
% \small % 或 \footnotesize 或 \scriptsize
\begin{longtable}{m{5mm}|m{3cm}m{3cm}m{2cm}m{3cm}m{4cm}}
    \caption{Summary of existing works.} \label{table:summary} \\
    \toprule
    \textbf{} & \textbf{Study} & \textbf{Data Type} & \textbf{Pre-training} & \textbf{Adaptation} & \textbf{Application} \\
    \midrule
    \endfirsthead

    \multicolumn{6}{c}{{\bfseries Table \thetable\ Summary of existing works (continued).}} \\
    \toprule
    \textbf{} & \textbf{Study} & \textbf{Data Type} & \textbf{Pre-training} & \textbf{Adaptation} & \textbf{Application} \\
    \midrule
    \endhead

    \midrule
    \multicolumn{6}{r}{{Continued on next page}} \\ 
    \endfoot

    \bottomrule
    \endlastfoot

    \multirow{10}{*}{\rotatebox{90}{\textbf{Language-based Models}}} & ERNIE-GeoL~\cite{huang2022ernie} & POI corpus, user behavior logs & Generative & Model fine-tuning & Map services \\
    \cline{2-6}
    ~ & MGeo~\cite{ding2023mgeo} & POI corpus & Generative, contrastive & Model fine-tuning & Query-POI matching \\
    \cline{2-6}
    ~ & Ji et al.~\cite{ji2023evaluating} & Geo-text, user instructions & - & Prompt engineering & Geographic information systems \\
    \cline{2-6}
    ~ & Bhandari et al.~\cite{bhandari2023large} & Geo-text, user instructions & - & Prompt engineering & Geographic information systems \\
    \cline{2-6}
    ~ & GPT4GEO~\cite{roberts2023gpt4geo} & Geo-text, user instructions & - & Prompt engineering & Geographic information systems \\
    \cline{2-6}
    ~ & Mooney et al.~\cite{mooney2023towards} & Geo-text, user instructions & - & Prompt engineering & Geographic information systems \\
    \cline{2-6}
    ~ & Mai et al.~\cite{mai2023opportunities} & Geo-text, user instructions & - & Prompt engineering & Geographic information systems \\
    \cline{2-6}
    ~ & Fu et al.~\cite{fu2023towards} & Documents, geo-text, user instructions & - & Prompt engineering & Urban science \\
    \cline{2-6}
    ~ & Aghzal et al.~\cite{aghzal2023can} & Geo-text, user instructions & - & Prompt engineering & Path planning \\
    \cline{2-6}
    ~ & GeoLLM~\cite{manvi2023geollm} & POI corpus & - & Prompt engineering & Geospatial prediction \\
    \cline{2-6}
    ~ & Zheng et al.~\cite{zheng2023chatgpt} & Traffic documents, user instructions & - & Prompt engineering & Intelligent transportation \\
    \cline{2-6}
    ~ & SpaBERT~\cite{li2022spabert}, GeoLM~\cite{li2023geolm} & Geo-text & - & Model fine-tuning & Geographic language understanding \\
    \cline{2-6}
    ~ & QUERT~\cite{xie2023quert} & User behavior logs & - & Model fine-tuning & Travel query understanding \\
    \cline{2-6}
    ~ & GEDR~\cite{mei2023improving} & POI corpus, user behavior logs & - & Model fine-tuning & Query-POI matching \\
    \cline{2-6}
    ~ & Wang et al.~\cite{wang2023optimizing} & LLM-generated instructions & - & Model fine-tuning & Urban renewal \\
    \cline{2-6}
    ~ & K2~\cite{deng2023learning} & Geo-text, geoscience instructions & - & Model fine-tuning & Geoscience tasks \\
    \midrule[0.5pt]
    
    \multirow{10}{*}{\rotatebox{90}{\textbf{Vision-based Models}}} & Urban2vec~\cite{wang2020urban2vec} & Street-view images & Contrastive & Model fine-tuning & \tabincell{c}{Demographic prediction, socioeconomic prediction} \\
    \cline{2-6}
    ~ & Li et al.~\cite{li2022predicting} & Street-view images & Contrastive & Model fine-tuning & Socioeconomic prediction \\
    \cline{2-6}
    ~ & KnowCL~\cite{liu2023knowledge} & Street-view images & Contrastive & Model fine-tuning & Socioeconomic prediction \\
    \cline{2-6}
    ~ & Wang et al.~\cite{wang2022advancing} & Remote sensing images & Generative & Model fine-tuning & \tabincell{c}{Remote sensing image analysis} \\
    \cline{2-6}
    ~ & ScaleMAE~\cite{reed2023scale} & Remote sensing images & Generative & Model fine-tuning & \tabincell{c}{Remote sensing image analysis} \\
    \cline{2-6}
    ~ & Cha et al.~\cite{cha2023billion} & Remote sensing images & Generative & Model fine-tuning & \tabincell{c}{Remote sensing image analysis} \\
    \cline{2-6}
    ~ & RingMo~\cite{sun2022ringmo} & Remote sensing images & Generative & Model fine-tuning & \tabincell{c}{Remote sensing image analysis} \\
    \cline{2-6}
    ~ & RingMo-Sense~\cite{yao2023ringmo} & Remote sensing images & Generative & Model fine-tuning & \tabincell{c}{Remote sensing spatiotemporal prediction} \\
    \cline{2-6}
    ~ & CSP~\cite{mai2023csp} & Remote sensing images & Contrastive & Model fine-tuning & \tabincell{c}{Satellite image classification} \\
    \cline{2-6}
    ~ & \tabincell{c}{FourCastNet~\cite{pathak2022fourcastnet}, Pangu-Weather~\cite{bi2023accurate}, FengWu~\cite{chen2023fengwu}} & Grid-based meteorological data & Generative & - & \tabincell{c}{Weather forecasting, tropical cyclones tracking} \\
    \cline{2-6}
    ~ & ClimaX~\cite{nguyen2023climax} & Grid-based meteorological data & Generative & Model fine-tuning & \tabincell{c}{Weather and climate modeling} \\
    \cline{2-6}
    ~ & W-MAE~\cite{man2023w} & Grid-based meteorological data & Generative & Model fine-tuning & \tabincell{c}{Weather forecasting, precipitation forecasting} \\
    \cline{2-6}
    ~ & SAMRS~\cite{wang2023samrs}, RSPrompter~\cite{chen2023rsprompter} & Remote sensing images & - & Prompt engineering & \tabincell{c}{Remote sensing semantic segmentation} \\
    \cline{2-6}
    ~ & Roberts et al.~\cite{roberts2023charting} & Remote sensing images & - & Prompt engineering & \tabincell{c}{Remote sensing image analysis} \\
    \cline{2-6}
    ~ & GeoSAM~\cite{sultan2023geosam} & Remote sensing images & - & Model fine-tuning & \tabincell{c}{Mobility infrastructure segmentation} \\
    \cline{2-6}
    ~ & RingMo-SAM~\cite{yan2023ringmo} & Remote sensing images & - & Model fine-tuning & \tabincell{c}{Multi-source remote sensing segmentation} \\
    \cline{2-6}
    ~ & Zhang et al.~\cite{zhang2022migratable} & Street-view images & - & Model fine-tuning & \tabincell{c}{Street-view image analysis} \\
    \cline{2-6}
    ~ &  StreetCLIP~\cite{sultan2023geosam} & Street-view images & - & Model fine-tuning & \tabincell{c}{Image geolocalization} \\
    
    % Trajectory-based Models
    \midrule[0.5pt]
    \multirow{10}{*}{\rotatebox{90}{\textbf{Trajectory-based Models}}} & t2vec~\cite{t2vec2018} & Trajectory in road networks & Generative & Model fine-tuning & \tabincell{c}{Similar trajectory search} \\
    \cline{2-6}
    ~ & traj2vec~\cite{traj2vec2017} & Trajectory in road networks & Generative & Model fine-tuning & \tabincell{c}{Trajectory cluster} \\
    \cline{2-6}
    ~ & Trembr~\cite{Trembr2020} & Trajectory in road networks & Generative & Model fine-tuning & \tabincell{c}{Similar trajectory search, travel time estimation, destination prediction} \\
    \cline{2-6}
    ~ & Toast~\cite{toast2021} & Trajectory in road networks & Generative & Model fine-tuning & \tabincell{c}{Road label classification, traffic inference, trajectory similarity search, travel time estimation} \\
    \cline{2-6}
    ~ & PIM~\cite{pim2021} & Trajectory in road networks & Contrastive & Model fine-tuning & \tabincell{c}{Travel time estimation, path ranking} \\
    \cline{2-6}
    ~ & STPT~\cite{stpt2023} & Trajectory in road networks & Contrastive & Model fine-tuning & \tabincell{c}{Trajectory classification, driving activity identification} \\
    \cline{2-6}
    ~ & LightPath~\cite{lightpath2023} & Trajectory in road networks & Generative & Model fine-tuning & \tabincell{c}{Travel time estimation, path ranking} \\
    \cline{2-6}
    ~ & MMTEC~\cite{mmtec2023} & Trajectory in road networks & Maximum Entropy Coding & Prompt engineering & \tabincell{c}{Similar trajectory search, travel time estimation,  destination prediction.} \\
    \cline{2-6}
    ~ & START~\cite{start2023} & Trajectory in road networks & \tabincell{c}{Generative, contrastive} & Prompt engineering & \tabincell{c}{Travel time estimation, trajectory classification, most similar trajectory search} \\
    \cline{2-6}
    ~ & HMTRL~\cite{hmtrl2022} & Trajectory in road networks & \tabincell{c}{Generative, contrastive} & Model fine-tuning & \tabincell{c}{Route recommendation} \\
    \cline{2-6}
    ~ & Movesim~\cite{movesim2020} & Trajectory in free space & \tabincell{c}{Generative, contrastive} & - & \tabincell{c}{Human mobility simulation} \\
    \cline{2-6}
    ~ & SML~\cite{sml2021} & Trajectory in free space & Contrastive & Model fine-tuning & \tabincell{c}{Location prediction, trajectory–user linking} \\
    \cline{2-6}
    ~ &  CTLE~\cite{ctle2021} & Trajectory in free space & Generative & - & \tabincell{c}{Next location prediction} \\
    \cline{2-6}
    ~ &  CACSR~\cite{cacsr2023} & Trajectory in free space & Contrastive & Model fine-tuning & \tabincell{c}{Next location prediction, trajectory user linking} \\
    \cline{2-6}
    ~ &  CATUS~\cite{CATUS2023} & Trajectory in free space & Contrastive & Model fine-tuning & \tabincell{c}{Next location prediction} \\
    \cline{2-6}
    ~ &  AuxMobLCast~\cite{auxmoblcast2022} & \tabincell{c}{Mobility prompt, user instructions} & - & Prompt engineering & \tabincell{c}{Human mobility forecasting} \\
    \cline{2-6}
    ~ &  LLM-Mob~\cite{llmmob2023} & \tabincell{c}{Mobility prompt, user instructions} & - & Prompt engineering & \tabincell{c}{Next location prediction} \\
    \cline{2-6}
    ~ &  Zhang et al.~\cite{zhang2023large} & \tabincell{c}{Mobility prompt, user instructions} & - & Prompt engineering & \tabincell{c}{Anomalous trajectory detection} \\
    \cline{2-6}
    ~ &  LLM-MPE~\cite{llmmpe2023} & \tabincell{c}{Mobility prompt, user instructions} & - & Prompt engineering & \tabincell{c}{Human mobility forecasting} \\
    \cline{2-6}
    ~ &  Keysan et al.~\cite{keysan2023can} & \tabincell{c}{Text description of scene, user instructions} & - & Prompt engineering & \tabincell{c}{Motion planning, driving trajectory prediction} \\
    \cline{2-6}
    ~ &  GPT-Driver~\cite{gptdriver2023} & \tabincell{c}{Text description of scene, user instructions} & - & Prompt engineering & \tabincell{c}{Motion planning, driving trajectory prediction} \\
    \cline{2-6}
    ~ &  LanguageMPC~\cite{languagempc2023} & \tabincell{c}{Text description of scene, user instructions} & - & Prompt engineering & \tabincell{c}{Motion planning, driving trajectory prediction} \\
    
    % Time series-based Models
    \midrule[0.5pt]
    \multirow{33}{*}{\rotatebox{90}{\textbf{Time series-based Models}}} 
    & Oreshkin et al.~\cite{oreshkin2021meta} & Ordinary time series & Supervised & - & \tabincell{c}{Energy consumption forecasting, traffic forecasting}\\
    \cline{2-6}
    ~ & Lag-Llama~\cite{rasul2023lag} & Ordinary time series & Supervised & - & Traffic forecasting\\
    \cline{2-6}
    ~ & SASA~\cite{cai2021time} & Ordinary time series & Supervised & - & Air quality regression\\
    \cline{2-6}
    ~ & TST~\cite{zerveas2021transformer} & Ordinary time series & Generative & - & Traffic regression\\
    \cline{2-6}
    ~ & SimMTM~\cite{dong2023simmtm} & Ordinary time series & Generative & - & \tabincell{c}{Weather forecasting, energy consumption forecasting, traffic forecasting}\\
    \cline{2-6}
    ~ & PatchTST~\cite{nie2022time} & Ordinary time series & Generative & - & \tabincell{c}{Weather forecasting, energy consumption forecasting, traffic forecasting}\\
    \cline{2-6}
    ~ & TSMixer~\cite{ekambaram2023tsmixer} & Ordinary time series & Generative & - & \tabincell{c}{Weather forecasting, energy consumption forecasting, traffic forecasting}\\
    \cline{2-6}
    ~ & PT-Tuning~\cite{liu2023pt} & Ordinary time series & Generative & Prompt engineering & \tabincell{c}{Weather forecasting, energy consumption forecasting, traffic forecasting}\\
    \cline{2-6}
    ~ & T-Loss~\cite{franceschi2019unsupervised} & Ordinary time series & Contrastive & - & \tabincell{c}{Traffic forecasting, energy consumption forecasting}\\
    \cline{2-6}
    ~ & COST~\cite{woo2022cost} & Ordinary time series & Contrastive & - & \tabincell{c}{Weather forecasting, energy consumption forecasting, traffic forecasting}\\
    \cline{2-6}
    ~ & TS2Vec~\cite{yue2022ts2vec} & Ordinary time series & Contrastive & - & \tabincell{c}{Traffic classification, energy consumption classification}\\
    \cline{2-6}
    ~ & SimTS~\cite{zheng2023simts} & Ordinary time series & Contrastive & - & \tabincell{c}{Weather forecasting, traffic forecasting}\\
    \cline{2-6}
    ~ & UniTime~\cite{liu2023unitime} & Ordinary time series & Hybrid & - & \tabincell{c}{Weather forecasting, energy consumption forecasting, traffic forecasting}\\
    \cline{2-6}
    ~ & ST-GSP~\cite{zhao2022st} & Spatial time series & Generative & - & Traffic forecasting\\
    \cline{2-6}
    ~ & STGCL~\cite{liu2022contrastive} & Spatial time series & Contrastive & - & Traffic forecasting\\
    \cline{2-6}
    ~ & STEP~\cite{shao2022pre} & Spatial time series & Generative & - & Traffic forecasting\\
    \cline{2-6}
    ~ & TransGTR~\cite{jin2023transferable} & Spatial time series & Hybrid & - & Traffic forecasting\\
    \cline{2-6}
    ~ & MC-STL~\cite{zhang2023mask} & Spatial time series & Hybrid & - & Traffic forecasting\\
    \cline{2-6}
    ~ & TPB~\cite{liu2023cross} & Spatial time series & Hybrid & - & Traffic forecasting\\
    \cline{2-6}
    ~ & GPT-ST~\cite{li2023gpt} & Spatial time series & Generative & - & Traffic forecasting\\
    \cline{2-6}
    ~ & PromptST~\cite{zhang2023promptst} & Spatial time series & - & Prompt engineering & \tabincell{c}{Traffic forecasting, complaint forecasting}\\
    \cline{2-6}
    ~ & MetePFL~\cite{chen2023prompt} & Spatial time series & - & Prompt engineering & Weather forecasting\\
    \cline{2-6}
    ~ & FedWing~\cite{chen2023spatial} & Spatial time series & - & Prompt engineering & Weather forecasting\\
    \cline{2-6}
    ~ & PromptCast~\cite{xue2023promptcast} & Ordinary time series & - & Prompt engineering & \tabincell{c}{Weather forecasting, energy consumption forecasting, human mobility forecasting}\\
    \cline{2-6} 
    ~ & LLMTime~\cite{gruver2023large} & Ordinary time series & - & Prompt engineering & \tabincell{c}{Weather forecasting, energy consumption forecasting, traffic forecasting}\\
    \cline{2-6} 
    ~ & GPT(6)~\cite{zhou2023one1_nips} & Ordinary time series & - & Model fine-tuning & \tabincell{c}{Weather forecasting, energy consumption forecasting, traffic forecasting}\\
    \cline{2-6} 
    ~ & GPT(6)-adapter~\cite{zhou2023one2} & Ordinary time series & - & Model fine-tuning & \tabincell{c}{Weather forecasting, energy consumption forecasting, traffic forecasting}\\
    \cline{2-6} 
    ~ & LLM4TS~\cite{chang2023llm4ts} & Ordinary time series & - & Model fine-tuning & \tabincell{c}{Weather forecasting, energy consumption forecasting, traffic forecasting}\\
    \cline{2-6} 
    ~ & TEMPO~\cite{cao2023tempo} & Ordinary time series & - & Model fine-tuning & \tabincell{c}{Weather forecasting, energy consumption forecasting, traffic forecasting}\\
    \cline{2-6} 
    ~ & GATGPT~\cite{chen2023gatgpt} & Spatial time series & - & Model fine-tuning & \tabincell{c}{Traffic forecasting, air quality imputation}\\
    \cline{2-6} 
    ~ & V2S~\cite{yang2021voice2series} & Ordinary time series & - & Model Reprogramming & Traffic classification\\
    \cline{2-6} 
    ~ & Time-LLM~\cite{jin2023time} & Ordinary time series & - & Model reprogramming & Traffic forecasting\\
    \cline{2-6}
    ~ & TEST~\cite{sun2023test} & Ordinary time series & - & Model reprogramming & \tabincell{c}{Traffic forecasting, energy consumption forecasting, air quality forecasting}\\
    
    \midrule[0.5pt]
    \multirow{14}{*}{\rotatebox{90}{\textbf{Multimodal Models}}} &  UrbanCLIP~\cite{yan2023urban} & Satellite image, textual description	& Contrastive & Model fine-tuning & Urban region profiling \\
    \cline{2-6}
    ~ & TengYun~\cite{zhao2023parallel} & Traffic-related text and image & Generative & Prompt tuning & \tabincell{c}{Traffic prediction and control, transportation planning} \\
    \cline{2-6}
    ~ & CityFM~\cite{balsebre2023city} & Spatial, visual, and textual geo-data & Contrastive	& -	& \tabincell{c}{Traffic speed inference, building functionality classification}\\
    \cline{2-6}
    ~ & AllSpark~\cite{shao2023allspark} & Text, image, trajectory, graph, etc.	& Contrastive &	Prompt engineering & Spatiotemporal data analysis \\
    \cline{2-6}
    ~ & TrafficGPT~\cite{zhang2023trafficgpt} & Multimodal traffic data & - & Prompt engineering & Traffic management \\
    \cline{2-6}
    ~ & GeoGPT~\cite{zhang2023geogpt} & Multimodal geospatial data	& -	& Prompt tuning	& \tabincell{c}{Autonomous geospatial data collection, processing, and analysis} \\
    \cline{2-6}
    ~ & VELMA~\cite{schumann2023velma} & Street image, navigation instruction	& -	& Model fine-tuning	& Autonomous street navigation \\
    \cline{2-6}
    ~ & UGI~\cite{xu2023urban} & \tabincell{c}{Urban textual, visual, knowledge graph, human behavior data} & - & \tabincell{c}{Continue learning, model fine-tuning} & \tabincell{c}{Urban planning and simulation, location recommendation} \\
    % \bottomrule[1pt]
\end{longtable}
\normalsize
\twocolumn


\section{Overview of Urban Foundation Models} \label{overview}
As illustrated in \figref{fig:taxonomy}, we introduce a data-centric taxonomy for the UFMs-related studies to shed light on the progress and efforts made in this field. Based on the urban data modalities, we categorize the existing works on UFMs into six classes: language-based models,  vision-based models, trajectory-based models, time series-based models, multimodal models, and others. Moreover, we further categorize the studies of each class into two subclasses based on their technical approaches: pretraining-based approaches and adaptation-based approaches.

\input{sections/language-based}

\input{sections/vision-based}

\input{sections/v2_trajectory-based}

\input{sections/time-series/v2_time-series-based}

\input{sections/multimodal-based}

\input{sections/others}
